Neural Markov Jump Processes

Markov jump processes are continuous-time stochastic processes with a wide range of applications in both natural and social sciences. Despite their widespread use, inference in these models is highly non-trivial and typically proceeds via either Monte Carlo or expectation-maximization methods. In this work we introduce an alternative, variational inference algorithm for Markov jump processes which relies on neural ordinary differential equations, and is trainable via back-propagation. Our methodology learns neural, continuous-time representations of the observed data, that are used to approximate the initial distribution and time-dependent transition probability rates of the posterior Markov jump process. The time-independent rates of the prior process are in contrast trained akin to generative adversarial networks. We test our approach on synthetic data sampled from ground-truth Markov jump processes, experimental switching ion channel data and molecular dynamics simulations. Source code to reproduce our experiments is available online.

==> adp_extra_experiment_tables.tex <==
% 50 length time series, full covariance matrix
\begin{figure}
\centering
\begin{subfigure}
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/figures_50_length_full_cov/run_0.png}
\end{subfigure}%
\begin{subfigure}
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/figures_50_length_full_cov/run_1.png}
\end{subfigure}
\begin{subfigure}
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/figures_50_length_full_cov/run_2.png}
\end{subfigure}%
\begin{subfigure}
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/figures_50_length_full_cov/run_3.png}
\end{subfigure}
\begin{subfigure}
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/figures_50_length_full_cov/run_4.png}
\end{subfigure}
\caption{50 length time series, full covariance matrix.}
\end{figure}

\begin{table}
\centering
\caption{50 length time series, full covariance. RMSE on prediction with error bars from sampling prior.}
\begin{tabular}{llllll}
\toprule
Experiment &         RMSE Test &            Pred 5 &           Pred 10 &           Pred 20 &           Pred 30 \\
\midrule
     run 0 & $0.631 \pm 0.094$ & $0.629 \pm 0.000$ & $0.635 \pm 0.015$ & $0.769 \pm 0.004$ & $0.760 \pm 0.018$ \\
     run 1 & $0.566 \pm 0.099$ & $0.626 \pm 0.001$ & $0.645 \pm 0.007$ & $0.799 \pm 0.034$ & $0.777 \pm 0.013$ \\
     run 2 & $0.646 \pm 0.100$ & $0.611 \pm 0.005$ & $0.658 \pm 0.002$ & $0.774 \pm 0.002$ & $0.787 \pm 0.001$ \\
     run 3 & $0.608 \pm 0.080$ & $0.598 \pm 0.002$ & $0.621 \pm 0.003$ & $0.750 \pm 0.000$ & $0.729 \pm 0.003$ \\
     run 4 & $0.548 \pm 0.082$ & $0.610 \pm 0.019$ & $0.625 \pm 0.001$ & $0.760 \pm 0.005$ & $0.728 \pm 0.003$ \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}
\centering
\caption{50 length time series, full covariance. NLL on prediction with error bars from sampling prior.}
\begin{tabular}{llllll}
\toprule
Experiment &             NLL Test &             Pred 5 &            Pred 10 &            Pred 20 &            Pred 30 \\
\midrule
     run 0 & $-26.169 \pm 38.358$ & $21.202 \pm 0.001$ & $30.549 \pm 2.675$ & $77.228 \pm 2.268$ & $90.394 \pm 7.851$ \\
     run 1 & $-34.551 \pm 57.946$ & $18.898 \pm 0.254$ & $25.220 \pm 0.053$ & $59.646 \pm 1.724$ & $64.769 \pm 0.657$ \\
     run 2 & $14.021 \pm 137.691$ & $16.113 \pm 0.026$ & $22.659 \pm 0.366$ & $19.449 \pm 5.205$ & $14.030 \pm 0.029$ \\
     run 3 & $-30.502 \pm 39.907$ & $16.115 \pm 0.037$ & $22.828 \pm 0.017$ & $54.235 \pm 0.000$ & $56.824 \pm 1.357$ \\
     run 4 & $-53.971 \pm 41.491$ & $22.015 \pm 0.661$ & $31.198 \pm 0.066$ & $72.337 \pm 0.193$ & $73.693 \pm 0.131$ \\
\bottomrule
\end{tabular}
\end{table}

%\begin{figure}
%\centering
%\begin{align*}
%& \begin{pmatrix}
%0. & 51.012 & 236.635 & 97.106 & 124598.297 & 124526.086\\
%15.170 & 0. & 231.142 & 91.972 & 124594.562 & 124522.383\\
%84.667 & 115.898 & 0. & 40.102 & 124578.352 & 124506.320\\
%50.245 & 83.405 & 141.073 & 0. & 124590.625 & 124518.422\\
%4175.924 & 4202.437 & 4290.668 & 4177.841 & 0. & 2111.799\\
%4129.581 & 4156.108 & 4244.449 & 4131.288 & 1804.003 & 0.\\
%\end{pmatrix}
%&\pm
%\begin{pmatrix}
%0. & 1.172 & 11.073 & 3.490 & 47613.332 & 47511.266\\
%0.725 & 0. & 10.924 & 3.302 & 47612.969 & 47510.914\\
%2.852 & 3.795 & 0. & 1.316 & 47609.820 & 47507.820\\
%2.012 & 2.682 & 8.83 & 0. & 47611.160 & 47509.137\\
%1244.198 & 1245.028 & 1241.45 & 1245.544 & 0. & 758.796\\
%1243.249 & 1244.067 & 1240.517 & 1244.726 & 846.503 & 0.\\
%\end{pmatrix}\\
%& \begin{pmatrix}
%0. & 26.634 & 337.391 & 196.075 & 122064.414 & 121738.641\\
%29.627 & 0. & 324.529 & 183.461 & 122075.609 & 121749.695\\
%138.428 & 120.384 & 0. & 38.966 & 122122.461 & 121796.383\\
%101.657 & 83.698 & 147.101 & 0. & 122101.531 & 121775.602\\
%8302.297 & 8291.911 & 8395.814 & 8284.892 & 0. & 1473.396\\
%8181.557 & 8171.228 & 8275.674 & 8164.309 & 2771.894 & 0.\\
%\end{pmatrix}
%&\pm
%\begin{pmatrix}
%0. & 1.427 & 17.918 & 10.941 & 43566.949 & 43422.809\\
%1.126 & 0. & 17.470 & 10.505 & 43566.359 & 43422.266\\
%3.994 & 3.753 & 0. & 1.472 & 43564.230 & 43420.203\\
%3.062 & 2.841 & 8.063 & 0. & 43564.344 & 43420.289\\
%3234.726 & 3234.23 & 3240.223 & 3239.373 & 0. & 611.025\\
%3243.281 & 3242.768 & 3248.446 & 3247.894 & 1644.055 & 0.\\
%\end{pmatrix}\\
%& \begin{pmatrix}
%0. & 124.794 & 324.237 & 41.452 & 1432.835 & 450.055\\
%75.495 & 0. & 310.316 & 20.706 & 1441.323 & 458.586\\
%198.254 & 256.202 & 0. & 118.832 & 1361.875 & 378.32\\
%86.201 & 149.532 & 293.049 & 0. & 1431.043 & 448.115\\
%458.702 & 519.488 & 561.418 & 378.426 & 0. & 393.375\\
%254.464 & 316.419 & 312.612 & 174.610 & 987.67 & 0.\\
%\end{pmatrix}
%&\pm
%\begin{pmatrix}
%0. & 5.608 & 14.396 & 1.653 & 106.867 & 26.259\\
%3.083 & 0. & 13.686 & 0.588 & 106.616 & 26.042\\
%12.470 & 15.091 & 0. & 8.473 & 103.425 & 21.988\\
%4.011 & 6.631 & 13.573 & 0. & 106.639 & 26.111\\
%64.802 & 67.319 & 64.464 & 61.568 & 0. & 54.419\\
%26.614 & 29.307 & 29.449 & 23.045 & 90.819 & 0.\\
%\end{pmatrix}\\
%& \begin{pmatrix}
%0. & 94.411 & 314.246 & 195.860 & 171419.266 & 27.533\\
%34.826 & 0. & 339.734 & 221.337 & 171418.109 & 15.956\\
%111.491 & 192.941 & 0. & 28.270 & 171368.141 & 133.127\\
%87.067 & 168.648 & 120.167 & 0. & 171392.141 & 108.781\\
%783.898 & 816.136 & 1064.018 & 952.308 & 0. & 788.540\\
%30.589 & 75.712 & 339.936 & 221.562 & 171420.688 & 0.\\
%\end{pmatrix}
%&\pm
%\begin{pmatrix}
%0. & 2.483 & 13.225 & 8.6 & 65252.258 & 1.203\\
%0.528 & 0. & 13.299 & 8.722 & 65250.578 & 0.682\\
%3.250 & 5.412 & 0. & 0.955 & 65259.914 & 3.988\\
%3.002 & 5.290 & 6.308 & 0. & 65257.039 & 3.774\\
%206.045 & 199.919 & 208.096 & 207.240 & 0. & 203.661\\
%0.442 & 1.782 & 13.352 & 8.751 & 65251.938 & 0.\\
%\end{pmatrix}\\
%& \begin{pmatrix}
%0. & 14.915 & 37.442 & 216.422 & 291094.594 & 138.946\\
%22.334 & 0. & 28.702 & 225.134 & 291097.656 & 147.587\\
%29.855 & 12.472 & 0. & 221.082 & 291099.125 & 143.483\\
%89.686 & 92.452 & 102.202 & 0. & 291085.344 & 31.347\\
%543.83 & 523.326 & 550.288 & 737.745 & 0. & 661.173\\
%70.601 & 73.366 & 83.113 & 79.425 & 291087.156 & 0.\\
%\end{pmatrix}
%&\pm
%\begin{pmatrix}
%0. & 0.487 & 0.732 & 6.193 & 99388.891 & 4.14\\
%0.504 & 0. & 0.556 & 6.104 & 99388.469 & 4.079\\
%0.67 & 0.457 & 0. & 5.976 & 99388.781 & 3.999\\
%2.773 & 2.781 & 2.753 & 0. & 99388.93 & 1.132\\
%120.210 & 120.495 & 120.276 & 121.01 & 0. & 120.621\\
%2.259 & 2.304 & 2.319 & 3.208 & 99388.953 & 0.\\
%\end{pmatrix}
%\\ \end{align*}
%\caption{50 length time series, full covariance.}
%\end{figure}


% 200 length time series, full covariance matrix
\begin{figure}
\centering
\begin{subfigure}
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/figures_200_length_full_cov/run_0.png}
\end{subfigure}%
\begin{subfigure}
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/figures_200_length_full_cov/run_1.png}
\end{subfigure}
\begin{subfigure}
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/figures_200_length_full_cov/run_2.png}
\end{subfigure}%
\begin{subfigure}
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/figures_200_length_full_cov/run_3.png}
\end{subfigure}
\begin{subfigure}
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/figures_200_length_full_cov/run_4.png}
\end{subfigure}
\caption{200 length time series, full covariance.}
\end{figure}


\begin{table}
\centering
\caption{ADP 200 length time series, full covariance. RMSE on prediction with error bars from sampling prior.}
\begin{tabular}{llllll}
\toprule
Experiment &         RMSE Test &            Pred 5 &           Pred 10 &           Pred 20 &           Pred 50 \\
\midrule
     run 0 & $0.651 \pm 0.070$ & $0.660 \pm 0.005$ & $0.757 \pm 0.012$ & $0.712 \pm 0.018$ & $0.863 \pm 0.034$ \\
     run 1 & $0.659 \pm 0.063$ & $0.660 \pm 0.006$ & $0.747 \pm 0.013$ & $0.714 \pm 0.025$ & $0.858 \pm 0.057$ \\
     run 2 & $0.649 \pm 0.066$ & $0.648 \pm 0.003$ & $0.744 \pm 0.008$ & $0.698 \pm 0.009$ & $0.871 \pm 0.011$ \\
     run 3 & $0.646 \pm 0.062$ & $0.654 \pm 0.011$ & $0.742 \pm 0.015$ & $0.716 \pm 0.024$ & $0.862 \pm 0.037$ \\
     run 4 & $0.654 \pm 0.061$ & $0.675 \pm 0.002$ & $0.758 \pm 0.001$ & $0.737 \pm 0.004$ & $0.866 \pm 0.025$ \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}
\centering
\caption{200 length time series, full covariance. NLL on prediction with error bars from sampling prior.}
\begin{tabular}{llllll}
\toprule
Experiment &              NLL Test &             Pred 5 &            Pred 10 &            Pred 20 &            Pred 50 \\
\midrule
     run 0 &  $-3.403 \pm 491.229$ & $19.064 \pm 0.039$ & $23.540 \pm 0.102$ & $20.002 \pm 0.916$ & $34.439 \pm 6.458$ \\
     run 1 &  $19.346 \pm 399.468$ & $14.436 \pm 0.106$ & $17.212 \pm 0.424$ & $15.779 \pm 0.621$ & $26.765 \pm 3.406$ \\
     run 2 & $-28.910 \pm 467.885$ & $15.745 \pm 0.018$ & $19.588 \pm 0.088$ & $17.424 \pm 0.286$ & $31.637 \pm 0.635$ \\
     run 3 & $-68.863 \pm 135.424$ & $14.276 \pm 0.132$ & $18.756 \pm 0.922$ & $16.408 \pm 2.344$ & $29.121 \pm 3.937$ \\
     run 4 &  $11.124 \pm 480.913$ & $13.887 \pm 0.004$ & $17.726 \pm 0.081$ & $18.435 \pm 1.975$ & $15.674 \pm 6.874$ \\
\bottomrule
\end{tabular}
\end{table}



%\begin{figure}
%\centering
%\begin{align*}
%& \begin{pmatrix}
%0. & 87.037 & 492.389 & 294.668 & 11817.264 & 95.094\\
%215.735 & 0. & 416.151 & 217.017 & 11807.629 & 155.835\\
%309.535 & 141.594 & 0. & 46.227 & 11732.274 & 267.505\\
%280.087 & 108.997 & 205.821 & 0. & 11752.736 & 237.592\\
%652.611 & 566.371 & 902.59 & 725.168 & 0. & 587.501\\
%213.909 & 68.42 & 478.526 & 280.392 & 11825.054 & 0.\\
%\end{pmatrix}
%&\pm
%\begin{pmatrix}
%0. & 6.662 & 63.56 & 31.565 & 3828.319 & 15.852\\
%24.178 & 0. & 62.786 & 30.478 & 3827.868 & 21.148\\
%36.035 & 19.283 & 0. & 10.513 & 3829.139 & 31.867\\
%32.524 & 15.006 & 40.252 & 0. & 3826.689 & 28.402\\
%216.72 & 202.739 & 211.956 & 202.551 & 0. & 213.924\\
%21.137 & 7.552 & 64.219 & 32.727 & 3825.628 & 0.\\
%\end{pmatrix}\\
%& \begin{pmatrix}
%0. & 410.112 & 578.025 & 340.74 & 10699.526 & 118.025\\
%457.937 & 0. & 556.645 & 313.249 & 10812.534 & 84.797\\
%473.372 & 414.475 & 0. & 56.450 & 10833.542 & 130.694\\
%442.507 & 384.551 & 263.333 & 0. & 10811.965 & 98.774\\
%820.071 & 682.883 & 835.021 & 650.264 & 0. & 528.909\\
%378.184 & 298.991 & 481.702 & 236.995 & 10790.863 & 0.\\
%\end{pmatrix}
%&\pm
%\begin{pmatrix}
%0. & 55.974 & 83.153 & 45.698 & 3663.032 & 17.317\\
%64.299 & 0. & 81.877 & 42.930 & 3658.324 & 10.984\\
%66.691 & 56.953 & 0. & 12.818 & 3655.410 & 17.308\\
%66.327 & 55.056 & 54.766 & 0. & 3656.655 & 13.817\\
%174.531 & 180.257 & 181.487 & 165.626 & 0. & 156.859\\
%61.621 & 50.820 & 79.270 & 39.707 & 3659.308 & 0.\\
%\end{pmatrix}\\
%& \begin{pmatrix}
%0. & 59.766 & 543.837 & 357.517 & 18620.588 & 132.772\\
%149.507 & 0. & 516.665 & 329.626 & 18606.648 & 104.240\\
%295.642 & 225.502 & 0. & 47.316 & 18622.121 & 132.278\\
%262.582 & 192.378 & 195.634 & 0. & 18624.199 & 98.180\\
%1215.713 & 1111.705 & 1511.731 & 1341.734 & 0. & 1163.200\\
%178.740 & 107.224 & 425.287 & 237.048 & 18622.619 & 0.\\
%\end{pmatrix}
%&\pm
%\begin{pmatrix}
%0. & 7.142 & 75.844 & 41.785 & 7789.942 & 11.114\\
%15.573 & 0. & 75.847 & 41.590 & 7795.552 & 10.971\\
%31.888 & 26.63 & 0. & 8.019 & 7770.065 & 17.685\\
%29.648 & 24.286 & 42.832 & 0. & 7777.661 & 14.688\\
%435.472 & 441.137 & 421.148 & 425.339 & 0. & 433.646\\
%20.418 & 14.039 & 70.048 & 35.406 & 7785.568 & 0.\\
%\end{pmatrix}\\
%& \begin{pmatrix}
%0. & 131.596 & 530.42 & 343.392 & 15907.637 & 112.540\\
%97.176 & 0. & 540.370 & 353.979 & 15897.181 & 122.352\\
%241.192 & 279.559 & 0. & 37.889 & 15889.478 & 129.309\\
%216.260 & 254.695 & 201.942 & 0. & 15903.036 & 103.440\\
%976.052 & 1012.485 & 1195.258 & 1022.154 & 0. & 907.784\\
%129.735 & 171.985 & 431.987 & 242.489 & 15910.634 & 0.\\
%\end{pmatrix}
%&\pm
%\begin{pmatrix}
%0. & 13.664 & 74.785 & 42.843 & 6348.065 & 12.155\\
%11.87 & 0. & 74.969 & 43.318 & 6353.111 & 13.562\\
%29.861 & 30.214 & 0. & 6.499 & 6330.786 & 16.425\\
%29.028 & 29.564 & 43.234 & 0. & 6334.71 & 15.149\\
%300.359 & 297.916 & 316.933 & 307.587 & 0. & 303.489\\
%19.55 & 19.548 & 69.613 & 37.466 & 6342.761 & 0.\\
%\end{pmatrix}\\
%& \begin{pmatrix}
%0. & 497.129 & 724.731 & 435.792 & 14412.042 & 333.938\\
%789.669 & 0. & 601.481 & 309.327 & 14447.628 & 58.927\\
%828.642 & 452.916 & 0. & 79.304 & 14350.402 & 169.227\\
%787.537 & 408.375 & 303.673 & 0. & 14385.333 & 123.303\\
%1041.074 & 1025.931 & 1087.279 & 836.612 & 0. & 816.792\\
%737.875 & 311.314 & 548.979 & 255.835 & 14417.294 & 0.\\
%\end{pmatrix}
%&\pm
%\begin{pmatrix}
%0. & 93.375 & 125.59 & 82.661 & 5247.363 & 57.528\\
%83.366 & 0. & 98.715 & 42.001 & 5232.756 & 7.454\\
%90.824 & 51.881 & 0. & 13.125 & 5238.459 & 21.866\\
%90.956 & 50.192 & 74.746 & 0. & 5236.699 & 18.072\\
%307.150 & 265.281 & 290.366 & 283.196 & 0. & 264.892\\
%81.709 & 42.269 & 97.537 & 40.737 & 5233.623 & 0.\\
%\end{pmatrix}
%\\ \end{align*}
%\caption{200 length time series, full covariance.}
%\end{figure}



% 7/8 runs on standardized data
\begin{figure}
\centering
\begin{subfigure}
    \centering
    \includegraphics[width=0.4\textwidth]{figures_7_extra_runs_standardized/run_20.png}
\end{subfigure}%
\begin{subfigure}
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/figures_7_extra_runs_standardized/run_21.png}
\end{subfigure}
\begin{subfigure}
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/figures_7_extra_runs_standardized/run_23.png}
\end{subfigure}
\begin{subfigure}
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/figures_7_extra_runs_standardized/run_24.png}
\end{subfigure}%
\begin{subfigure}
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/figures_7_extra_runs_standardized/run_25.png}
\end{subfigure}
\begin{subfigure}
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/figures_7_extra_runs_standardized/run_26.png}
\end{subfigure}%
\begin{subfigure}
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/figures_7_extra_runs_standardized/run_27.png}
\end{subfigure}
\caption{Standardized data.}
\end{figure}

\begin{table}
\centering
\caption{Standardized data. Relaxation Time with error bars from sampling prior.}
\begin{tabular}{ll}
\toprule
Experiment &                                                                                     Relaxation Time \\
\midrule
    run 20 &   [$-8.427\pm0.106$, $-11.182\pm0.153$, $-11.427\pm0.159$, $-74.29\pm1.154$, $-1310.625\pm209.121$] \\
    run 21 & [$-11.081\pm0.104$, $-16.033\pm0.157$, $-16.033\pm0.157$, $-46.821\pm0.513$, $-1675.752\pm407.303$] \\
    run 23 &     [$-9.578\pm0.164$, $-11.748\pm0.281$, $-25.553\pm0.661$, $-80.274\pm1.6$, $-782.907\pm125.064$] \\
    run 24 &    [$-10.913\pm0.111$, $-15.694\pm0.136$, $-27.156\pm0.33$, $-74.836\pm1.335$, $-909.862\pm93.484$] \\
    run 25 &  [$-10.072\pm0.116$, $-13.029\pm0.169$, $-13.029\pm0.169$, $-65.755\pm0.85$, $-1157.262\pm139.493$] \\
    run 26 &      [$-5.738\pm0.082$, $-8.71\pm0.096$, $-9.615\pm0.117$, $-70.437\pm0.806$, $-1314.63\pm157.736$] \\
    run 27 &  [$-12.837\pm0.086$, $-16.605\pm0.099$, $-16.605\pm0.099$, $-42.683\pm0.344$, $-978.819\pm109.442$] \\
\bottomrule
\end{tabular}
\end{table}



% 10 new runs, normalize obs
\begin{figure}
\centering
\begin{subfigure}
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/figures_10_extra_runs_with_norm/run_10.png}
\end{subfigure}%
\begin{subfigure}
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/figures_10_extra_runs_with_norm/run_11.png}
\end{subfigure}
\begin{subfigure}
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/figures_10_extra_runs_with_norm/run_12.png}
\end{subfigure}%
\begin{subfigure}
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/figures_10_extra_runs_with_norm/run_13.png}
\end{subfigure}
\begin{subfigure}
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/figures_10_extra_runs_with_norm/run_14.png}
\end{subfigure}%
\begin{subfigure}
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/figures_10_extra_runs_with_norm/run_15.png}
\end{subfigure}
\begin{subfigure}
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/figures_10_extra_runs_with_norm/run_16.png}
\end{subfigure}%
\begin{subfigure}
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/figures_10_extra_runs_with_norm/run_17.png}
\end{subfigure}
\begin{subfigure}
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/figures_10_extra_runs_with_norm/run_18.png}
\end{subfigure}%
\begin{subfigure}
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/figures_10_extra_runs_with_norm/run_19.png}
\end{subfigure}
\caption{10 new runs, normalize observations during training.}
\end{figure}


\begin{table}
\centering
\caption{10 new runs, normalize observations. RMSE on prediction with error bars from sampling prior.}
\begin{tabular}{llllll}
\toprule
Experiment &         RMSE Test &            Pred 5 &           Pred 10 &           Pred 20 &           Pred 50 \\
\midrule
    run 10 & $0.666 \pm 0.122$ & $0.638 \pm 0.001$ & $0.688 \pm 0.000$ & $0.742 \pm 0.000$ & $0.836 \pm 0.003$ \\
    run 11 & $0.637 \pm 0.143$ & $0.591 \pm 0.002$ & $0.643 \pm 0.000$ & $0.692 \pm 0.000$ & $0.854 \pm 0.000$ \\
    run 12 & $0.656 \pm 0.122$ & $0.649 \pm 0.000$ & $0.681 \pm 0.000$ & $0.727 \pm 0.000$ & $0.856 \pm 0.000$ \\
    run 13 & $0.655 \pm 0.125$ & $0.629 \pm 0.001$ & $0.687 \pm 0.000$ & $0.765 \pm 0.000$ & $0.878 \pm 0.000$ \\
    run 14 & $0.753 \pm 0.162$ & $0.690 \pm 0.004$ & $0.767 \pm 0.000$ & $0.821 \pm 0.004$ & $0.955 \pm 0.000$ \\
    run 15 & $0.642 \pm 0.141$ & $0.632 \pm 0.000$ & $0.679 \pm 0.000$ & $0.726 \pm 0.001$ & $0.822 \pm 0.000$ \\
    run 16 & $0.646 \pm 0.146$ & $0.605 \pm 0.003$ & $0.664 \pm 0.006$ & $0.708 \pm 0.000$ & $0.825 \pm 0.000$ \\
    run 17 & $0.641 \pm 0.145$ & $0.616 \pm 0.000$ & $0.682 \pm 0.001$ & $0.730 \pm 0.004$ & $0.866 \pm 0.000$ \\
    run 18 & $0.637 \pm 0.138$ & $0.601 \pm 0.016$ & $0.656 \pm 0.002$ & $0.712 \pm 0.000$ & $0.857 \pm 0.000$ \\
    run 19 & $0.625 \pm 0.144$ & $0.617 \pm 0.000$ & $0.662 \pm 0.000$ & $0.710 \pm 0.000$ & $0.839 \pm 0.000$ \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}
\centering
\caption{10 new runs, normalize observations. NLL on prediction with error bars from sampling prior.}
\begin{tabular}{llllll}
\toprule
Experiment &              NLL Test &            Pred 5 &            Pred 10 &            Pred 20 &            Pred 50 \\
\midrule
    run 10 &  $-27.354 \pm 79.661$ & $2.169 \pm 0.011$ &  $3.979 \pm 0.000$ &  $6.869 \pm 0.000$ & $11.114 \pm 0.026$ \\
    run 11 &   $5.749 \pm 685.093$ & $8.114 \pm 0.016$ & $16.026 \pm 0.000$ & $27.813 \pm 0.000$ & $52.953 \pm 0.000$ \\
    run 12 & $-38.319 \pm 122.104$ & $9.250 \pm 0.000$ & $16.902 \pm 0.001$ & $35.181 \pm 0.000$ & $59.554 \pm 0.000$ \\
    run 13 &  $40.909 \pm 670.511$ & $5.605 \pm 0.164$ &  $8.466 \pm 0.000$ & $14.441 \pm 0.000$ & $22.640 \pm 0.000$ \\
    run 14 &  $21.263 \pm 133.033$ & $0.978 \pm 0.022$ &  $5.073 \pm 0.002$ & $11.038 \pm 0.170$ &  $1.370 \pm 0.000$ \\
    run 15 &  $-5.787 \pm 613.493$ & $8.379 \pm 0.000$ & $22.822 \pm 0.004$ & $36.476 \pm 0.008$ & $34.724 \pm 0.000$ \\
    run 16 &   $1.952 \pm 641.476$ & $7.838 \pm 0.014$ & $15.208 \pm 0.186$ & $30.744 \pm 0.000$ & $49.065 \pm 0.000$ \\
    run 17 &  $-0.666 \pm 614.002$ & $8.473 \pm 0.002$ & $14.364 \pm 0.147$ & $27.013 \pm 0.953$ & $32.751 \pm 0.000$ \\
    run 18 &   $9.037 \pm 604.849$ & $7.563 \pm 0.243$ & $14.836 \pm 0.008$ & $29.746 \pm 0.000$ & $49.332 \pm 0.000$ \\
    run 19 & $-12.197 \pm 471.019$ & $1.761 \pm 0.003$ &  $3.760 \pm 0.004$ &  $6.429 \pm 0.000$ & $12.943 \pm 0.000$ \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}
\centering
\caption{10 new runs, normalize obs during training. Equilibria with error bars from sampling prior.}
\begin{tabular}{ll}
\toprule
Experiment &                                                                                            Equilibrium \\
\midrule
    run 10 & [$0.185\pm0.003$, $0.425\pm0.005$, $0.092\pm0.002$, $0.152\pm0.003$, $0.103\pm0.006$, $0.043\pm0.002$] \\
    run 11 &   [$0.433\pm0.003$, $0.218\pm0.002$, $0.178\pm0.003$, $0.111\pm0.001$, $0.001\pm0.0$, $0.059\pm0.001$] \\
    run 12 &   [$0.408\pm0.004$, $0.242\pm0.002$, $0.164\pm0.003$, $0.116\pm0.002$, $0.001\pm0.0$, $0.069\pm0.001$] \\
    run 13 & [$0.433\pm0.076$, $0.167\pm0.029$, $0.135\pm0.024$, $0.118\pm0.021$, $0.134\pm0.136$, $0.013\pm0.013$] \\
    run 14 &  [$0.174\pm0.002$, $0.228\pm0.002$, $0.144\pm0.002$, $0.408\pm0.003$, $0.03\pm0.001$, $0.016\pm0.001$] \\
    run 15 &   [$0.367\pm0.004$, $0.294\pm0.004$, $0.122\pm0.003$, $0.131\pm0.003$, $0.001\pm0.0$, $0.085\pm0.001$] \\
    run 16 & [$0.443\pm0.006$, $0.188\pm0.002$, $0.157\pm0.005$, $0.102\pm0.002$, $0.002\pm0.001$, $0.108\pm0.002$] \\
    run 17 &  [$0.24\pm0.004$, $0.377\pm0.005$, $0.145\pm0.005$, $0.111\pm0.003$, $0.003\pm0.001$, $0.125\pm0.002$] \\
    run 18 & [$0.412\pm0.007$, $0.178\pm0.002$, $0.194\pm0.006$, $0.096\pm0.002$, $0.003\pm0.001$, $0.118\pm0.002$] \\
    run 19 & [$0.401\pm0.005$, $0.149\pm0.002$, $0.219\pm0.007$, $0.092\pm0.001$, $0.003\pm0.001$, $0.136\pm0.002$] \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}
\centering
\caption{10 new runs, normalize observations. Relaxation Time in picoseconds with error bars from sampling prior.}
\begin{tabular}{ll}
\toprule
Experiment &                                                                                        Relaxation Time \\
\midrule
    run 10 &       [$-11.069\pm0.127$, $-15.303\pm0.101$, $-33.84\pm0.576$, $-70.291\pm0.697$, $-383.868\pm16.533$] \\
    run 11 &           [$-5.41\pm0.065$, $-7.149\pm0.073$, $-9.144\pm0.089$, $-69.09\pm0.592$, $-614.699\pm37.022$] \\
    run 12 &         [$-5.753\pm0.064$, $-7.612\pm0.078$, $-9.715\pm0.078$, $-63.608\pm0.445$, $-678.751\pm74.546$] \\
    run 13 & [$-10.428\pm0.079$, $-12.141\pm0.092$, $-20.118\pm1.024$, $-68.387\pm0.986$, $-67982.633\pm22089.559$] \\
    run 14 &       [$-22.181\pm0.196$, $-24.086\pm0.107$, $-24.087\pm0.107$, $-47.954\pm0.285$, $-188.007\pm5.542$] \\
    run 15 &          [$-6.196\pm0.057$, $-9.595\pm0.078$, $-13.78\pm0.122$, $-85.384\pm1.087$, $-695.46\pm46.985$] \\
    run 16 &          [$-7.265\pm0.104$, $-8.86\pm0.144$, $-12.519\pm0.195$, $-69.496\pm1.109$, $-844.19\pm92.375$] \\
    run 17 &       [$-7.489\pm0.127$, $-12.104\pm0.171$, $-17.575\pm0.26$, $-90.725\pm1.355$, $-854.296\pm127.575$] \\
    run 18 &         [$-5.833\pm0.098$, $-8.262\pm0.146$, $-10.659\pm0.178$, $-80.88\pm1.368$, $-783.796\pm95.128$] \\
    run 19 &          [$-7.869\pm0.102$, $-9.975\pm0.143$, $-13.67\pm0.154$, $-69.551\pm0.938$, $-905.9\pm118.826$] \\
\bottomrule
\end{tabular}
\end{table}


\begin{figure}
\centering
\begin{align*}
&
\begin{pmatrix}
0. & 104.674 & 394.551 & 192.262 & 11055.858 & 8764.990\\
15.625 & 0. & 410.038 & 207.758 & 11070.794 & 8779.980\\
138.633 & 236.834 & 0. & 20.463 & 10922.346 & 8631.275\\
120.339 & 218.518 & 209.215 & 0. & 10904.019 & 8612.856\\
1608.762 & 1705.593 & 1752.636 & 1561.466 & 0. & 784.42\\
1417.272 & 1514.271 & 1547.289 & 1356.343 & 2327.735 & 0.\\
\end{pmatrix}
&\pm
\begin{pmatrix}
0. & 4.115 & 11.131 & 4.270 & 1940.174 & 1605.115\\
0.206 & 0. & 11.129 & 4.232 & 1940.089 & 1605.025\\
8.266 & 11.869 & 0. & 0.426 & 1938.952 & 1604.631\\
8.256 & 11.856 & 8.282 & 0. & 1939.156 & 1604.862\\
263.020 & 264.656 & 272.039 & 269.399 & 0. & 153.47\\
264.325 & 265.927 & 274.487 & 271.896 & 570.838 & 0.\\
\end{pmatrix}\\
\end{align*}
\caption{Un-normalized data, run  1 mean passage times}
\end{figure}





% 100 length time series, diagonal covariance
\begin{figure}
\centering
\begin{subfigure}
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/figures_diag_cov/run_0.png}
\end{subfigure}%
\begin{subfigure}
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/figures_diag_cov/run_1.png}
\end{subfigure}
\begin{subfigure}
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/figures_diag_cov/run_2.png}
\end{subfigure}%
\begin{subfigure}
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/figures_diag_cov/run_3.png}
\end{subfigure}
\begin{subfigure}
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/figures_diag_cov/run_4.png}
\end{subfigure}
\caption{100 length time series, diagonal covariance matrix.}
\end{figure}


\begin{table}
\centering
\caption{100 length time series, diagonal covariance. RMSE on prediction with error bars from sampling prior.}
\begin{tabular}{llllll}
\toprule
Experiment &         RMSE Test &            Pred 5 &           Pred 10 &           Pred 20 &           Pred 50 \\
\midrule
     run 0 & $0.654 \pm 0.161$ & $0.627 \pm 0.000$ & $0.702 \pm 0.006$ & $0.716 \pm 0.001$ & $0.898 \pm 0.005$ \\
     run 1 & $0.635 \pm 0.147$ & $0.596 \pm 0.005$ & $0.656 \pm 0.000$ & $0.699 \pm 0.007$ & $0.829 \pm 0.038$ \\
     run 2 & $0.686 \pm 0.156$ & $0.630 \pm 0.002$ & $0.691 \pm 0.002$ & $0.741 \pm 0.041$ & $0.801 \pm 0.011$ \\
     run 3 & $0.633 \pm 0.145$ & $0.615 \pm 0.002$ & $0.680 \pm 0.002$ & $0.709 \pm 0.007$ & $0.818 \pm 0.027$ \\
     run 4 & $0.638 \pm 0.146$ & $0.651 \pm 0.006$ & $0.698 \pm 0.016$ & $0.716 \pm 0.001$ & $0.825 \pm 0.000$ \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}
\centering
\caption{100 length time series, diagonal covariance. NLL on prediction with error bars from sampling prior.}
\begin{tabular}{llllll}
\toprule
Experiment &             NLL Test &            Pred 5 &           Pred 10 &           Pred 20 &            Pred 50 \\
\midrule
     run 0 & $81.876 \pm 223.075$ & $1.852 \pm 0.000$ & $4.259 \pm 0.512$ & $6.352 \pm 0.075$ & $15.010 \pm 0.508$ \\
     run 1 & $51.260 \pm 249.677$ & $1.695 \pm 0.077$ & $4.292 \pm 0.002$ & $6.215 \pm 0.255$ & $12.366 \pm 3.251$ \\
     run 2 & $73.958 \pm 166.812$ & $0.909 \pm 0.015$ & $2.395 \pm 0.127$ & $5.217 \pm 0.794$ &  $8.828 \pm 0.785$ \\
     run 3 & $52.916 \pm 313.834$ & $1.741 \pm 0.040$ & $4.474 \pm 0.024$ & $6.308 \pm 0.198$ & $13.525 \pm 1.661$ \\
     run 4 & $64.587 \pm 358.857$ & $2.373 \pm 0.057$ & $4.882 \pm 0.125$ & $6.395 \pm 0.095$ & $10.993 \pm 0.000$ \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}
\centering
\caption{100 length time series, diagonal covariance. Equilibria with error bars from sampling prior.}
\begin{tabular}{ll}
\toprule
Experiment &                                                                                            Equilibrium \\
\midrule
     run 0 &     [$0.468\pm0.018$, $0.215\pm0.006$, $0.195\pm0.012$, $0.053\pm0.005$, $0.069\pm0.006$, $0.0\pm0.0$] \\
     run 1 & [$0.119\pm0.007$, $0.164\pm0.007$, $0.126\pm0.014$, $0.153\pm0.011$, $0.024\pm0.011$, $0.414\pm0.019$] \\
     run 2 &  [$0.405\pm0.018$, $0.202\pm0.008$, $0.129\pm0.009$, $0.218\pm0.011$, $0.041\pm0.02$, $0.005\pm0.002$] \\
     run 3 & [$0.167\pm0.005$, $0.138\pm0.006$, $0.133\pm0.013$, $0.143\pm0.008$, $0.017\pm0.007$, $0.403\pm0.014$] \\
     run 4 &  [$0.158\pm0.006$, $0.153\pm0.008$, $0.09\pm0.008$, $0.187\pm0.011$, $0.017\pm0.007$, $0.395\pm0.014$] \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}
\centering
\caption{100 length time series, diagonal covariance. Relaxation Time with error bars from sampling prior.}
\begin{tabular}{ll}
\toprule
Experiment &                                                                               Relaxation Time \\
\midrule
     run 0 &      [$9.062\pm0.534$, $9.714\pm0.599$, $11.432\pm0.447$, $20.881\pm1.147$, $71.205\pm3.745$] \\
     run 1 &   [$4.953\pm0.255$, $7.164\pm0.387$, $10.165\pm0.458$, $62.272\pm2.817$, $979.009\pm285.093$] \\
     run 2 & [$14.856\pm0.376$, $17.248\pm0.483$, $31.194\pm4.999$, $64.791\pm1.995$, $2501.947\pm977.64$] \\
     run 3 &   [$7.197\pm0.298$, $9.456\pm0.417$, $12.216\pm0.558$, $68.906\pm3.794$, $771.907\pm166.991$] \\
     run 4 & [$9.991\pm0.333$, $12.468\pm0.438$, $13.852\pm0.613$, $70.553\pm2.892$, $1048.516\pm371.267$] \\
\bottomrule
\end{tabular}
\end{table}



%%% Removed Figures showing separation of states
\section{ADP, 5 selected runs, full covariance}
\begin{figure}
\centering
\begin{subfigure}
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/figures_5_selected_runs/adp_run_0.png}
\end{subfigure}%
\begin{subfigure}
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/figures_5_selected_runs/adp_run_1.png}
\end{subfigure}
\begin{subfigure}
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/figures_5_selected_runs/adp_run_2.png}
\end{subfigure}%
\begin{subfigure}
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/figures_5_selected_runs/adp_run_3.png}
\end{subfigure}
\begin{subfigure}
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/figures_5_selected_runs/adp_run_4.png}
\end{subfigure}
\caption{5 selected runs, un-normalized data.}
\end{figure}


%   \begin{figure}
%   \centering
%   {\small
%   \begin{align*}
%   & \begin{pmatrix}
%   0. & 67.744 & 297.589 & 165.45 & 22983.676 & 23038.643\\
%   18.293 & 0. & 311.991 & 179.993 & 22985.609 & 23042.131\\
%   142.796 & 201.977 & 0. & 55.318 & 22924.232 & 22994.545\\
%   95.026 & 154.153 & 133.093 & 0. & 22938.264 & 22998.178\\
%   905.505 & 930.876 & 1110.227 & 992.437 & 0. & 4506.108\\
%   769.323 & 793.731 & 973.483 & 855.855 & 4498.42 & 0.\\
%   \end{pmatrix}
%   &\pm
%   \begin{pmatrix}
%   0. & 5.137 & 23.449 & 10.963 & 5092.290 & 4808.451\\
%   1.441 & 0. & 23.768 & 11.224 & 5092.443 & 4808.09\\
%   12.519 & 15.987 & 0. & 4.274 & 5097.052 & 4809.417\\
%   10.559 & 14.208 & 16.818 & 0. & 5093.735 & 4808.850\\
%   210.482 & 214.086 & 200.797 & 202.95 & 0. & 1913.325\\
%   189.308 & 193.316 & 179.892 & 180.896 & 1565.527 & 0.\\
%   \end{pmatrix}\\
%   & \begin{pmatrix}
%   0. & 138.33 & 299.857 & 48.198 & 104006.305 & 92127.570\\
%   382.427 & 0. & 367.259 & 121.465 & 103982.828 & 92082.703\\
%   477.65 & 137.562 & 0. & 47.616 & 103994.141 & 92119.344\\
%   431.653 & 90.949 & 253.247 & 0. & 103991.711 & 92096.547\\
%   1279.398 & 1142.333 & 1297.46 & 1061.728 & 0. & 84521.789\\
%   1311.212 & 1086.158 & 1186.652 & 1031.759 & 59985.484 & 0.\\
%   \end{pmatrix}
%   &\pm
%   \begin{pmatrix}
%   0. & 7.281 & 18.706 & 3.125 & 34710.867 & 31207.381\\
%   30.293 & 0. & 20.81 & 5.385 & 34712.969 & 31209.773\\
%   30.314 & 7.413 & 0. & 2.403 & 34711.371 & 31208.961\\
%   29.753 & 5.840 & 18.596 & 0. & 34711.422 & 31209.178\\
%   280.777 & 246.294 & 242.320 & 246.63 & 0. & 29537.551\\
%   236.43 & 231.946 & 255.027 & 234.001 & 26572.143 & 0.\\
%   \end{pmatrix}\\
%   & \begin{pmatrix}
%   0. & 18.288 & 378.707 & 212.328 & 32150.783 & 29776.740\\
%   109.832 & 0. & 360.994 & 194.538 & 32145.59 & 29771.707\\
%   219.194 & 118.271 & 0. & 35.659 & 32019.322 & 29645.535\\
%   187.097 & 85.969 & 175.781 & 0. & 32066.264 & 29692.057\\
%   1698.555 & 1630.969 & 1811.363 & 1689.886 & 0. & 2741.523\\
%   1564.369 & 1499.021 & 1679.341 & 1557.217 & 3942.547 & 0.\\
%   \end{pmatrix}
%   &\pm
%   \begin{pmatrix}
%   0. & 1.139 & 31.252 & 14.752 & 8949.484 & 8489.84\\
%   7.036 & 0. & 31.182 & 14.674 & 8950.319 & 8490.606\\
%   14.936 & 10.455 & 0. & 3.750 & 8949.858 & 8490.729\\
%   12.901 & 8.178 & 19.635 & 0. & 8948.637 & 8489.407\\
%   382.785 & 380.021 & 383.709 & 378.848 & 0. & 1082.768\\
%   369.53 & 366.229 & 370.854 & 365.806 & 1449.364 & 0.\\
%   \end{pmatrix}\\
%   & \begin{pmatrix}
%   0. & 34.156 & 418.409 & 225.276 & 16547.752 & 15511.635\\
%   39.362 & 0. & 390.644 & 197.679 & 16531.77 & 15507.103\\
%   142.431 & 110.099 & 0. & 60.104 & 16398.354 & 15494.911\\
%   100.324 & 68.219 & 219.951 & 0. & 16450.869 & 15483.832\\
%   533.393 & 517.545 & 727.903 & 558.658 & 0. & 12526.279\\
%   420.342 & 403.634 & 542.133 & 450.179 & 14362.049 & 0.\\
%   \end{pmatrix}
%   &\pm
%   \begin{pmatrix}
%   0. & 2.453 & 48.054 & 21.386 & 4302.082 & 3933.452\\
%   4.798 & 0. & 48.034 & 21.298 & 4302.156 & 3932.355\\
%   12.719 & 10.373 & 0. & 5.769 & 4313.721 & 3928.432\\
%   10.557 & 8.032 & 33.474 & 0. & 4304.769 & 3927.742\\
%   76.19 & 77.176 & 97.801 & 86.907 & 0. & 3880.534\\
%   59.388 & 58.588 & 94.674 & 65.033 & 4023.051 & 0.\\
%   \end{pmatrix}\\
%   & \begin{pmatrix}
%   0. & 27.539 & 290.648 & 106.966 & 13726.715 & 15864.058\\
%   32.459 & 0. & 287.114 & 102.982 & 13728.424 & 15865.984\\
%   131.683 & 133.512 & 0. & 63.494 & 13729.080 & 15859.124\\
%   72.53 & 74.224 & 187.246 & 0. & 13706.344 & 15844.268\\
%   917.046 & 913.309 & 1054.649 & 932.254 & 0. & 3959.010\\
%   804.452 & 800.225 & 952.336 & 824.08 & 2563.419 & 0.\\
%   \end{pmatrix}
%   &\pm
%   \begin{pmatrix}
%   0. & 2.379 & 27.775 & 6.354 & 3990.165 & 4007.994\\
%   2.776 & 0. & 27.45 & 6.016 & 3989.649 & 4007.413\\
%   11.473 & 11.321 & 0. & 5.361 & 3985.953 & 4005.433\\
%   8.188 & 8.053 & 24.957 & 0. & 3988.846 & 4006.788\\
%   220.779 & 221.158 & 232.475 & 224.869 & 0. & 1118.255\\
%   207.978 & 208.572 & 211.777 & 208.569 & 1076.984 & 0.\\
%   \end{pmatrix}
%   \\ \end{align*}}
%   \caption{5 selected runs mean  passage times.}
%   \end{figure}


%%% 10 new runs

%\begin{figure}
%\centering
%\begin{subfigure}
%    \centering
%    \includegraphics[width=0.4\textwidth]{Figures/figures_10_extra_runs/run_0.png}
%\end{subfigure}%
%\begin{subfigure}
%    \centering
%    \includegraphics[width=0.4\textwidth]{Figures/figures_10_extra_runs/run_1.png}
%\end{subfigure}
%\begin{subfigure}
%    \centering
%    \includegraphics[width=0.4\textwidth]{Figures/figures_10_extra_runs/run_2.png}
%\end{subfigure}%
%\begin{subfigure}
%    \centering
%    \includegraphics[width=0.4\textwidth]{Figures/figures_10_extra_runs/run_3.png}
%\end{subfigure}
%\begin{subfigure}
%    \centering
%    \includegraphics[width=0.4\textwidth]{Figures/figures_10_extra_runs/run_4.png}
%\end{subfigure}%
%\begin{subfigure}
%    \centering
%    \includegraphics[width=0.4\textwidth]{Figures/figures_10_extra_runs/run_5.png}
%\end{subfigure}
%\begin{subfigure}
%    \centering
%    \includegraphics[width=0.4\textwidth]{Figures/figures_10_extra_runs/run_6.png}
%\end{subfigure}%
%\begin{subfigure}
%    \centering
%    \includegraphics[width=0.4\textwidth]{Figures/figures_10_extra_runs/run_7.png}
%\end{subfigure}
%\begin{subfigure}
%    \centering
%    \includegraphics[width=0.4\textwidth]{Figures/figures_10_extra_runs/run_8.png}
%\end{subfigure}%
%\begin{subfigure}
%    \centering
%    \includegraphics[width=0.4\textwidth]{Figures/figures_10_extra_runs/run_9.png}
%\end{subfigure}
%\caption{10 runs of ADP, un-normalized data during training.}
%\end{figure}
%


%\begin{table}
%\centering
%\caption{10 new runs. NLL on prediction with error bars from sampling prior.}
%\begin{tabular}{llllll}
%\toprule
%Experiment &             NLL Test &             Pred 5 &            Pred 10 &            Pred 20 &            Pred 50 \\
%\midrule
%     run 0 & $33.829 \pm 807.249$ &  $7.834 \pm 0.003$ & $14.779 \pm 0.000$ & $29.639 \pm 0.123$ & $51.050 \pm 0.186$ \\
%     run 1 & $-16.180 \pm 94.323$ &  $1.460 \pm 0.012$ &  $2.711 \pm 0.004$ &  $4.597 \pm 0.000$ &  $7.425 \pm 0.000$ \\
%     run 2 & $14.471 \pm 713.887$ &  $3.123 \pm 0.002$ & $14.712 \pm 0.497$ & $11.603 \pm 0.005$ & $21.086 \pm 0.000$ \\
%     run 3 & $19.460 \pm 413.984$ &  $1.989 \pm 0.015$ &  $3.578 \pm 0.013$ &  $6.244 \pm 0.000$ & $10.610 \pm 0.007$ \\
%     run 4 & $-9.695 \pm 529.113$ &  $7.334 \pm 0.143$ &  $5.658 \pm 0.038$ &  $9.029 \pm 0.130$ & $16.459 \pm 0.187$ \\
%     run 5 & $48.485 \pm 831.841$ &  $4.926 \pm 0.005$ & $10.750 \pm 0.012$ & $11.853 \pm 0.027$ & $17.443 \pm 0.102$ \\
%     run 6 & $44.772 \pm 849.915$ & $11.185 \pm 0.024$ & $21.577 \pm 2.062$ & $37.965 \pm 0.068$ & $64.540 \pm 0.537$ \\
%     run 7 & $34.416 \pm 944.469$ &  $7.150 \pm 0.014$ & $12.356 \pm 0.061$ & $24.884 \pm 0.000$ & $40.793 \pm 0.019$ \\
%     run 8 &  $5.817 \pm 597.914$ &  $4.474 \pm 0.001$ & $14.369 \pm 0.090$ & $25.635 \pm 0.528$ & $47.047 \pm 0.022$ \\
%     run 9 & $22.561 \pm 778.671$ &  $7.921 \pm 0.002$ & $14.828 \pm 0.664$ & $29.582 \pm 0.000$ & $47.328 \pm 0.000$ \\
%\bottomrule
%\end{tabular}
%\end{table}



%\begin{figure}
%\centering
%\begin{align*}
%& \begin{pmatrix}
%0. & 47.507 & 303.972 & 339.885 & 376.791 & 59308.266\\
%38.544 & 0. & 278.128 & 311.906 & 358. & 59313.016\\
%135.583 & 102.530 & 0. & 193.498 & 254.660 & 59304.480\\
%143.636 & 110.770 & 22.343 & 0. & 258.370 & 59295.195\\
%102.731 & 74.769 & 175.173 & 282.595 & 0. & 59319.367\\
%147.108 & 114.556 & 36.809 & 65.492 & 266.86 & 0.\\
%\end{pmatrix}
%&\pm
%\begin{pmatrix}
%0. & 2.153 & 17.822 & 20.998 & 27.891 & 22518.908\\
%2.785 & 0. & 17.313 & 20.764 & 26.821 & 22518.225\\
%8.11 & 6.995 & 0. & 10.694 & 17.347 & 22527.537\\
%8.162 & 6.994 & 2.448 & 0. & 17.083 & 22523.352\\
%6.357 & 5.263 & 11.746 & 16.080 & 0. & 22520.391\\
%8.002 & 6.806 & 3.401 & 6.189 & 17.245 & 0.\\
%\end{pmatrix}\\
%& \begin{pmatrix}
%0. & 41.996 & 335.316 & 203.282 & 45295.949 & 12.582\\
%62.99 & 0. & 320.616 & 188.668 & 45312.547 & 20.034\\
%140.213 & 105.882 & 0. & 23.582 & 45337.559 & 112.28\\
%120.206 & 85.876 & 141.466 & 0. & 45330.77 & 92.302\\
%1028.081 & 1044.001 & 1317.824 & 1191.518 & 0. & 1024.345\\
%48.074 & 34.003 & 336.776 & 204.774 & 45311.52 & 0.\\
%\end{pmatrix}
%&\pm
%\begin{pmatrix}
%0. & 2.311 & 24.139 & 13.522 & 16920.428 & 1.231\\
%3.536 & 0. & 23.913 & 13.137 & 16917.037 & 1.749\\
%6.886 & 5.832 & 0. & 1.596 & 16908.564 & 6.328\\
%6.328 & 5.248 & 15.095 & 0. & 16911.314 & 5.72\\
%304.222 & 297.930 & 294.222 & 296.008 & 0. & 300.496\\
%2.894 & 1.946 & 24.388 & 13.792 & 16917.934 & 0.\\
%\end{pmatrix}\\
%& \begin{pmatrix}
%0. & 75.793 & 343.101 & 173.782 & 61063.703 & 60474.910\\
%54.297 & 0. & 321.686 & 155.415 & 61064.305 & 60475.695\\
%152.302 & 140.779 & 0. & 29.643 & 61075.746 & 60489.523\\
%123.776 & 112.366 & 184.759 & 0. & 61077.457 & 60490.203\\
%2712.966 & 2695.992 & 2917.165 & 2770.385 & 0. & 4714.257\\
%2613.684 & 2596.155 & 2821.441 & 2673.756 & 3501. & 0.\\
%\end{pmatrix}
%&\pm
%\begin{pmatrix}
%0. & 3.782 & 18.544 & 9.629 & 23426.793 & 23031.436\\
%3.209 & 0. & 17.784 & 8.564 & 23426.508 & 23031.262\\
%6.528 & 5.825 & 0. & 1.590 & 23423.6 & 23027.857\\
%5.687 & 5.146 & 11.981 & 0. & 23425.154 & 23029.676\\
%1076.935 & 1079.370 & 1074.330 & 1072.994 & 0. & 2381.552\\
%1071.622 & 1074.442 & 1067.899 & 1066.975 & 2134.321 & 0.\\
%\end{pmatrix}\\
%& \begin{pmatrix}
%0. & 76.12 & 364.858 & 193.664 & 53489.336 & 27.485\\
%49.923 & 0. & 376.202 & 204.738 & 53492.02 & 24.966\\
%113.827 & 164.759 & 0. & 31.194 & 53423.387 & 130.488\\
%86.726 & 137.587 & 176.926 & 0. & 53436.922 & 103.380\\
%833.475 & 802.142 & 1146.613 & 979.802 & 0. & 814.569\\
%41.497 & 60.442 & 387.4 & 216.113 & 53494.320 & 0.\\
%\end{pmatrix}
%&\pm
%\begin{pmatrix}
%0. & 3.657 & 19.196 & 9.399 & 20149.371 & 2.073\\
%2.096 & 0. & 19.011 & 9.222 & 20147.795 & 1.905\\
%6.690 & 10.555 & 0. & 2.694 & 20144.072 & 8.388\\
%5.086 & 9.539 & 14.044 & 0. & 20147.045 & 6.998\\
%172.140 & 173.126 & 174.319 & 173.529 & 0. & 171.913\\
%1.660 & 2.706 & 19.179 & 9.469 & 20149.984 & 0.\\
%\end{pmatrix}\\
%& \begin{pmatrix}
%0. & 98.75 & 409.369 & 203.953 & 66603.195 & 43.434\\
%70.489 & 0. & 438.761 & 233.090 & 66614.953 & 32.421\\
%119.816 & 179.249 & 0. & 24.174 & 66560.672 & 143.732\\
%98.838 & 158.104 & 213.91 & 0. & 66576.203 & 122.717\\
%1136.811 & 1111.942 & 1462.104 & 1264.251 & 0. & 1111.482\\
%62.354 & 73.998 & 448.6 & 243.159 & 66614.320 & 0.\\
%\end{pmatrix}
%&\pm
%\begin{pmatrix}
%0. & 4.959 & 21.412 & 11.605 & 26041.811 & 3.129\\
%2.348 & 0. & 21.867 & 12.619 & 26043.434 & 2.238\\
%5.376 & 9.776 & 0. & 2.125 & 26045.699 & 7.517\\
%4.308 & 9.175 & 12.74 & 0. & 26045.035 & 6.571\\
%379.917 & 385.712 & 381.325 & 380.567 & 0. & 381.458\\
%2.265 & 3.917 & 21.719 & 12.266 & 26044.537 & 0.\\
%\end{pmatrix}
%\\ \end{align*}
%\caption{100 length time series, diagonal covariance.}
%\end{figure}






%% Ion Channel
%\begin{table}
%\centering
%\caption{Ion Channel trained on first second. NLL on prediction with error bars from sampling prior.}
%\begin{tabular}{llllll}
%\toprule
%Experiment &                 NLL Test &             Pred 5 &            Pred 10 &            Pred 20 &            Pred 50 \\
%\midrule
%     run 0 & $-1816.827 \pm 1904.679$ &  $0.837 \pm 0.045$ &  $6.827 \pm 3.866$ & $45.573 \pm 3.564$ & $18.505 \pm 1.683$ \\
%     run 1 &  $-2194.978 \pm 818.345$ & $10.011 \pm 0.000$ & $13.881 \pm 0.000$ & $36.534 \pm 4.118$ & $18.906 \pm 0.000$ \\
%     run 2 &  $-2229.142 \pm 718.582$ & $13.048 \pm 5.556$ & $25.581 \pm 0.000$ & $47.018 \pm 0.027$ & $22.215 \pm 5.407$ \\
%     run 3 & $-1552.948 \pm 2168.707$ & $10.114 \pm 0.000$ & $14.035 \pm 0.183$ & $35.543 \pm 0.860$ & $19.218 \pm 0.428$ \\
%     run 4 & $-1850.768 \pm 1825.458$ & $19.291 \pm 0.000$ & $23.056 \pm 0.061$ & $44.865 \pm 0.751$ & $31.199 \pm 0.409$ \\
%\bottomrule
%\end{tabular}
%\end{table}
%
%
%\begin{table}
%\centering
%\caption{Ion Channel trained on first second. Equilibria with error bars from sampling prior. State order: low, mid, high.}
%\begin{tabular}{ll}
%\toprule
%Experiment &                                         Equilibrium \\
%\midrule
%     run 0 & [$0.177\pm0.033$, $0.094\pm0.013$, $0.729\pm0.039$] \\
%     run 1 & [$0.184\pm0.029$, $0.087\pm0.012$, $0.729\pm0.037$] \\
%     run 2 & [$0.176\pm0.037$, $0.097\pm0.014$, $0.727\pm0.045$] \\
%     run 3 &  [$0.19\pm0.048$, $0.082\pm0.016$, $0.728\pm0.058$] \\
%     run 4 & [$0.178\pm0.043$, $0.087\pm0.011$, $0.734\pm0.048$] \\
%\bottomrule
%\end{tabular}
%\end{table}
%
%
%\begin{table}
%\centering
%\caption{Ion Channel trained on first second. Relaxation Time in seconds with error bars from sampling prior.}
%\begin{tabular}{ll}
%\toprule
%Experiment &                    Relaxation Time \\
%\midrule
%     run 0 & [$-0.003\pm0.0$, $-0.021\pm0.002$] \\
%     run 1 & [$-0.003\pm0.0$, $-0.021\pm0.002$] \\
%     run 2 & [$-0.003\pm0.0$, $-0.021\pm0.002$] \\
%     run 3 &  [$-0.003\pm0.0$, $-0.02\pm0.002$] \\
%     run 4 & [$-0.003\pm0.0$, $-0.019\pm0.002$] \\
%\bottomrule
%\end{tabular}
%\end{table}

% \begin{figure} \centering
% \begin{equation*}
% \begin{pmatrix}
% $-373.14576$ & $-48.30131$ & $-0.0$\\
% \end{pmatrix}\end{equation*}
% \caption{Eigenvalues of the Q-matrix for selected Ion Channel 1st second experiment.}
% \end{figure}
% \begin{figure} \centering
% \begin{equation*}
% \begin{pmatrix}
% -0.00268 & -0.02070\\
% \end{pmatrix}
% \end{equation*}
% \caption{Relaxation times (inverse of real parts of eigenvalues) for selected Ion Channel 1st second experiment.}
% \end{figure}
% \begin{figure}
% \centering
% \begin{align*}
% \begin{pmatrix}
% 0. & 0.01863 & 0.02977\\
% 0.07429 & 0. & 0.01349\\
% 0.11025 & 0.03829 & 0.\\
% \end{pmatrix}
% \\ \end{align*}
% \caption{Mean passage time in seconds from state in row to state in column for selected Ion Channel Experiment.}
% \end{figure}
% 





%\begin{table}
%\centering
%\caption{5 selected runs. RMSE on prediction with error bars from sampling prior.}
%\begin{tabular}{lrllll}
%\toprule
%Experiment &  RMSE Test &            Pred 5 &           Pred 10 &           Pred 20 &           Pred 50 \\
%\midrule
%     run 0 &   0.627937 & $1.185 \pm 0.628$ & $1.201 \pm 0.618$ & $1.167 \pm 0.607$ & $1.127 \pm 0.613$ \\
%     run 1 &   0.747193 & $1.168 \pm 0.598$ & $1.178 \pm 0.594$ & $1.178 \pm 0.593$ & $1.126 \pm 0.591$ \\
%     run 2 &   0.692117 & $1.180 \pm 0.611$ & $1.194 \pm 0.597$ & $1.210 \pm 0.588$ & $1.154 \pm 0.566$ \\
%     run 3 &   0.636459 & $1.161 \pm 0.599$ & $1.183 \pm 0.579$ & $1.165 \pm 0.597$ & $1.107 \pm 0.582$ \\
%     run 4 &   0.624748 & $1.191 \pm 0.629$ & $1.222 \pm 0.621$ & $1.209 \pm 0.642$ & $1.192 \pm 0.640$ \\
%\bottomrule
%\end{tabular}
%\end{table}

\begin{table}
\centering
\caption{100 length time series, full covariance. RMSE on prediction with error bars from sampling prior.}
\begin{tabular}{lllllll}
\toprule
Group & Experiment &         RMSE Test &            Pred 5 &           Pred 10 &           Pred 20 &           Pred 50 \\
\midrule
\multirow{5}*{Handpicked} 
     &\textbf{run 0} & $0.614 \pm 0.129$ & $0.633 \pm 0.004$ & $0.716 \pm 0.012$ & $0.728 \pm 0.000$ & $0.868 \pm 0.001$ \\
     &run 1 & $0.731 \pm 0.162$ & $0.643 \pm 0.000$ & $0.689 \pm 0.003$ & $0.737 \pm 0.005$ & $0.859 \pm 0.029$ \\
     &run 2 & $0.680 \pm 0.137$ & $0.594 \pm 0.001$ & $0.659 \pm 0.045$ & $0.755 \pm 0.002$ & $0.892 \pm 0.076$ \\
     &\textbf{run 3} & $0.622 \pm 0.125$ & $0.611 \pm 0.009$ & $0.687 \pm 0.004$ & $0.708 \pm 0.028$ & $0.840 \pm 0.039$ \\
     &\textbf{run 4} & $0.615 \pm 0.128$ & $0.641 \pm 0.002$ & $0.677 \pm 0.010$ & $0.767 \pm 0.053$ & $0.893 \pm 0.136$ \\
\midrule
\multirow{10}*{Additional}
    &run 0 & $0.641 \pm 0.147$ & $0.608 \pm 0.001$ & $0.667 \pm 0.000$ & $0.703 \pm 0.000$ & $0.833 \pm 0.005$ \\
    &\textbf{run 1} & $0.661 \pm 0.115$ & $0.634 \pm 0.000$ & $0.690 \pm 0.001$ & $0.734 \pm 0.000$ & $0.852 \pm 0.000$ \\
    &run 2 & $0.643 \pm 0.139$ & $0.615 \pm 0.000$ & $0.660 \pm 0.001$ & $0.709 \pm 0.001$ & $0.839 \pm 0.000$ \\
    &run 3 & $0.659 \pm 0.147$ & $0.638 \pm 0.003$ & $0.701 \pm 0.001$ & $0.739 \pm 0.000$ & $0.830 \pm 0.001$ \\
    &run 4 & $0.643 \pm 0.141$ & $0.626 \pm 0.000$ & $0.664 \pm 0.002$ & $0.704 \pm 0.004$ & $0.822 \pm 0.008$ \\
    &run 5 & $0.661 \pm 0.159$ & $0.646 \pm 0.001$ & $0.710 \pm 0.001$ & $0.758 \pm 0.000$ & $0.861 \pm 0.012$ \\
    &run 6 & $0.663 \pm 0.153$ & $0.657 \pm 0.006$ & $0.682 \pm 0.001$ & $0.719 \pm 0.001$ & $0.848 \pm 0.013$ \\
    &run 7 & $0.630 \pm 0.120$ & $0.606 \pm 0.002$ & $0.655 \pm 0.000$ & $0.709 \pm 0.000$ & $0.834 \pm 0.001$ \\
    &run 8 & $0.647 \pm 0.147$ & $0.616 \pm 0.000$ & $0.668 \pm 0.006$ & $0.710 \pm 0.011$ & $0.850 \pm 0.001$ \\
    &run 9 & $0.630 \pm 0.147$ & $0.612 \pm 0.000$ & $0.673 \pm 0.002$ & $0.704 \pm 0.000$ & $0.830 \pm 0.000$ \\
\bottomrule
\end{tabular}
\end{table}

%\begin{table}
%\centering
%\caption{5 selected runs. NLL on prediction with error bars from sampling prior.}
%\begin{tabular}{llllll}
%\toprule
%Experiment &              NLL Test &             Pred 5 &            Pred 10 &            Pred 20 &            Pred 50 \\
%\midrule
%     run 0 &  $29.371 \pm 704.960$ & $15.666 \pm 0.197$ & $24.295 \pm 0.257$ & $35.547 \pm 0.000$ & $56.732 \pm 0.148$ \\
%     run 1 & $-20.915 \pm 113.587$ &  $7.773 \pm 0.001$ & $14.390 \pm 0.017$ & $26.085 \pm 0.032$ & $50.679 \pm 1.494$ \\
%     run 2 & $-26.112 \pm 125.885$ &  $5.684 \pm 0.006$ & $11.695 \pm 0.255$ & $24.301 \pm 0.037$ & $42.475 \pm 7.681$ \\
%     run 3 & $-43.771 \pm 154.627$ &  $8.562 \pm 0.364$ & $18.072 \pm 0.263$ & $32.515 \pm 1.542$ & $60.740 \pm 6.937$ \\
%     run 4 &  $-82.793 \pm 77.203$ &  $8.942 \pm 0.061$ & $15.370 \pm 0.098$ & $29.405 \pm 1.583$ & $45.929 \pm 2.561$ \\
%\bottomrule
%\end{tabular}
%\end{table}

\begin{table}
\centering
\caption{100 length time series, full covariance. Equilibria with error bars from sampling prior.}
\begin{tabular}{lrcccccc}
\toprule
Group & Experiment & \multicolumn{6}{c}{Equilibrium Distribution} \\
       &    &                  State 1 &         State 2 &         State 3 &         State 4 &         State 5 &         State 6 \\
\midrule
& VAMPnets &              $0.30017$    & $0.23837$ & $0.1936$ & $0.14458$ & $0.10904$ & $0.01424$ \\
\midrule
\multirow{5}*{Handpicked}
    & \textbf{run 0} &          $0.433\pm0.022$ &  $0.19\pm0.015$ & $0.258\pm0.026$ & $0.082\pm0.005$ & $0.034\pm0.012$ & $0.004\pm0.001$ \\
    & run 1 &          $0.099\pm0.008$ & $0.478\pm0.021$ & $0.154\pm0.014$ & $0.253\pm0.012$ &  $0.01\pm0.004$ & $0.006\pm0.002$ \\
    & run 2 &           $0.136\pm0.01$ & $0.534\pm0.025$ & $0.139\pm0.017$ &  $0.139\pm0.01$ & $0.042\pm0.015$ &  $0.01\pm0.003$ \\
    & \textbf{run 3} &           $0.43\pm0.029$ & $0.285\pm0.017$ & $0.158\pm0.024$ &  $0.084\pm0.01$ & $0.025\pm0.007$ & $0.019\pm0.005$ \\
    & \textbf{run 4} &          $0.298\pm0.021$ &  $0.31\pm0.018$ & $0.234\pm0.028$ & $0.097\pm0.007$ & $0.053\pm0.017$ & $0.008\pm0.002$ \\
\midrule
\multirow{10}*{Additional}
    & run 0 &          $0.414\pm0.005$ & $0.264\pm0.002$ & $0.146\pm0.004$ & $0.125\pm0.002$ & $0.002\pm0.001$ &  $0.05\pm0.001$ \\
    & \textbf{run 1} &           $0.47\pm0.015$ & $0.129\pm0.004$ & $0.082\pm0.003$ & $0.185\pm0.006$ & $0.091\pm0.019$ & $0.043\pm0.008$ \\
    & run 2 &           $0.35\pm0.003$ & $0.205\pm0.002$ & $0.126\pm0.003$ & $0.121\pm0.002$ &   $0.002\pm0.0$ & $0.197\pm0.003$ \\
    & run 3 &          $0.483\pm0.004$ & $0.114\pm0.002$ & $0.108\pm0.002$ & $0.204\pm0.002$ &   $0.001\pm0.0$ & $0.091\pm0.002$ \\
    & run 4 &          $0.475\pm0.005$ & $0.187\pm0.003$ & $0.112\pm0.003$ & $0.158\pm0.004$ &   $0.001\pm0.0$ & $0.067\pm0.001$ \\
    & run 5 &          $0.334\pm0.004$ & $0.191\pm0.002$ & $0.105\pm0.004$ & $0.188\pm0.004$ &   $0.001\pm0.0$ & $0.181\pm0.002$ \\
    & run 6 &          $0.456\pm0.006$ & $0.223\pm0.003$ & $0.127\pm0.004$ & $0.124\pm0.002$ & $0.002\pm0.001$ & $0.069\pm0.002$ \\
    & run 7 &          $0.127\pm0.003$ & $0.177\pm0.002$ & $0.168\pm0.005$ & $0.114\pm0.003$ & $0.017\pm0.004$ & $0.397\pm0.006$ \\
    & run 8 &          $0.073\pm0.001$ & $0.222\pm0.002$ & $0.162\pm0.004$ & $0.127\pm0.002$ &   $0.001\pm0.0$ & $0.415\pm0.004$ \\ 
    & run 9 &          $0.423\pm0.005$ & $0.228\pm0.002$ & $0.203\pm0.005$ & $0.084\pm0.002$ &   $0.002\pm0.0$ & $0.061\pm0.001$ \\
\bottomrule
\end{tabular}
\end{table}



\begin{table}
\centering
\caption{100 length time series, full covariance. Relaxation Time with error bars from sampling prior.}
\begin{tabular}{lrccccc}
\toprule
 Group & Experiment & \multicolumn{5}{c}{Ordered Relaxation Times} \\
 &              & & & & &  \\
\midrule
 & VAMPnets & 7.7 & 9.1 & 55 & 65 & 1920 \\
 & Varolg\"une & 2.72 & 3.1 & 33 & 65 & 1430 \\
\midrule
\multirow{5}*{Handpicked}
    & \textbf{run 0} &           $7.82\pm0.393$ & $11.304\pm0.568$ &   $26.64\pm5.355$ &    $84.011\pm5.196$ &   $818.36\pm191.225$ \\
    & run 1 &         $21.477\pm0.645$ &  $47.925\pm3.79$ &  $55.457\pm3.156$ & $499.273\pm123.846$ & $1023.302\pm229.839$ \\
    & run 2 &         $11.775\pm0.479$ & $13.987\pm0.621$ &  $44.395\pm9.901$ &    $67.559\pm3.981$ &  $1511.488\pm343.45$ \\
    & \textbf{run 3} &           $9.429\pm0.48$ & $13.176\pm0.658$ &  $71.735\pm5.922$ &   $249.067\pm36.53$ &   $412.152\pm64.807$ \\
    & \textbf{run 4} &          $8.706\pm0.427$ &  $9.017\pm0.419$ & $42.836\pm11.849$ &    $69.012\pm4.302$ &  $773.558\pm205.017$ \\
\midrule
\multirow{10}*{Additional}
    & run 0 &          $6.258\pm0.114$ &  $7.928\pm0.108$ & $10.143\pm0.139$ & $58.539\pm0.679$ &   $694.46\pm121.959$ \\
    & \textbf{run 1} &          $11.637\pm0.12$ & $12.476\pm0.136$ & $62.131\pm0.773$ &  $79.76\pm4.401$ & $1282.166\pm214.316$ \\
    & run 2 &           $7.793\pm0.06$ &  $10.42\pm0.069$ & $13.284\pm0.103$ & $73.467\pm0.765$ &    $835.921\pm128.9$ \\
    & run 3 &         $10.399\pm0.091$ & $14.798\pm0.135$ & $17.125\pm0.166$ & $62.805\pm0.624$ &   $673.097\pm78.534$ \\
    & run 4 &            $5.35\pm0.08$ &  $8.757\pm0.111$ & $10.224\pm0.127$ & $77.226\pm0.691$ &   $501.076\pm45.054$ \\
    & run 5 &          $9.572\pm0.101$ & $10.705\pm0.131$ &   $17.875\pm0.1$ & $52.792\pm0.773$ &    $797.3\pm141.918$ \\
    & run 6 &           $7.26\pm0.088$ &  $8.986\pm0.149$ &  $10.91\pm0.178$ & $63.059\pm0.988$ &  $825.822\pm135.503$ \\
    & run 7 &            $7.478\pm0.1$ &  $7.862\pm0.081$ & $12.508\pm0.138$ & $60.255\pm0.653$ &  $737.398\pm103.588$ \\
    & run 8 &          $6.681\pm0.073$ &  $7.567\pm0.093$ & $10.538\pm0.122$ &  $63.08\pm0.874$ &   $608.783\pm55.453$ \\
    & run 9 &          $4.613\pm0.063$ &  $6.174\pm0.083$ &  $7.784\pm0.111$ & $69.777\pm0.777$ &   $648.549\pm59.624$ \\
\bottomrule
\end{tabular}
\end{table}





\section{ADP, 200 length time series, full covariance}

\begin{table}
\centering
\caption{200 length time series, full covariance. Equilibria with error bars from sampling prior.}
\begin{tabular}{rcccccc}
\toprule
Experiment & \multicolumn{6}{c}{Equilibrium Distribution} \\
           &                  State 1 &         State 2 &         State 3 &         State 4 &         State 5 &         State 6 \\
\midrule
VAMPnets &              $0.30017$    & $0.23837$ & $0.1936$ & $0.14458$ & $0.10904$ & $0.01424$ \\
\midrule
     run 0 &          $0.149\pm0.017$ & $0.288\pm0.024$ & $0.132\pm0.026$ & $0.143\pm0.019$ &  $0.043\pm0.02$ & $0.244\pm0.028$ \\
     run 1 &           $0.21\pm0.033$ & $0.208\pm0.033$ & $0.119\pm0.024$ & $0.144\pm0.021$ & $0.042\pm0.016$ &  $0.277\pm0.02$ \\
     run 2 &           $0.21\pm0.025$ & $0.312\pm0.032$ & $0.147\pm0.029$ & $0.112\pm0.015$ & $0.059\pm0.025$ & $0.159\pm0.015$ \\
     run 3 &           $0.278\pm0.03$ & $0.233\pm0.023$ & $0.113\pm0.022$ & $0.147\pm0.023$ & $0.055\pm0.025$ & $0.173\pm0.016$ \\
     run 4 &          $0.238\pm0.047$ & $0.149\pm0.022$ & $0.133\pm0.027$ & $0.122\pm0.018$ & $0.045\pm0.025$ & $0.313\pm0.027$ \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}
\centering
\caption{200 length time series, full covariance.. Relaxation Time with error bars from sampling prior.}
\begin{tabular}{rccccc}
\toprule
Experiment & \multicolumn{5}{c}{Ordered Relaxation Times} \\
           \\
\midrule
 VAMPnets & 7.7 & 9.1 & 55 & 65 & 1920 \\
 Varolg\"une & 2.72 & 3.1 & 33 & 65 & 1430 \\
\midrule
     run 0 &         $13.738\pm1.308$ & $27.947\pm1.905$ & $28.385\pm2.048$ &  $85.581\pm9.109$ & $467.663\pm186.041$ \\
     run 1 &          $16.23\pm1.672$ & $30.105\pm2.275$ &  $83.634\pm7.42$ &  $99.082\pm9.782$ & $420.136\pm145.537$ \\
     run 2 &         $11.071\pm0.819$ & $19.913\pm1.311$ & $26.386\pm2.069$ & $100.519\pm9.359$ &  $995.779\pm392.28$ \\
     run 3 &         $12.449\pm0.973$ &  $20.94\pm1.424$ & $28.984\pm2.084$ &  $96.167\pm9.225$ &  $786.058\pm271.17$ \\
     run 4 &         $17.573\pm1.839$ &  $34.97\pm2.552$ & $85.765\pm7.755$ & $183.282\pm31.74$ &  $571.003\pm233.88$ \\
\bottomrule
\end{tabular}
\end{table}




\section{ADP, 50 length time series, full covariance matrix}


\begin{table}
\centering
\caption{50 length time series, full covariance. Equilibria with error bars from sampling prior.}
\begin{tabular}{rcccccc}
\toprule
Experiment & \multicolumn{6}{c}{Equilibrium Distribution} \\
           &                  State 1 &         State 2 &         State 3 &         State 4 &         State 5 &         State 6 \\
\midrule
VAMPnets &              $0.30017$    & $0.23837$ & $0.1936$ & $0.14458$ & $0.10904$ & $0.01424$ \\
\midrule
     \textbf{run 0} &          $0.529\pm0.013$ & $0.122\pm0.004$ &   $0.19\pm0.01$ & $0.125\pm0.005$ &  $0.031\pm0.01$ & $0.003\pm0.001$ \\
     \textbf{run 1} &          $0.357\pm0.012$ & $0.288\pm0.009$ &  $0.196\pm0.01$ & $0.093\pm0.004$ & $0.056\pm0.022$ & $0.011\pm0.004$ \\
     \textbf{run 2} &          $0.204\pm0.009$ & $0.066\pm0.003$ & $0.176\pm0.008$ &  $0.32\pm0.012$ & $0.185\pm0.028$ & $0.049\pm0.003$ \\
     run 3 &          $0.187\pm0.004$ & $0.097\pm0.003$ &  $0.17\pm0.008$ & $0.123\pm0.005$ & $0.005\pm0.002$ &  $0.417\pm0.01$ \\
     run 4 &          $0.184\pm0.003$ & $0.356\pm0.007$ &  $0.16\pm0.003$ & $0.205\pm0.008$ & $0.002\pm0.001$ & $0.093\pm0.002$ \\
\bottomrule
\end{tabular}

\end{table}

\begin{table}
\centering
\caption{50 length time series, full covariance. Relaxation Time with error bars from sampling prior.}
\begin{tabular}{rccccc}
\toprule
Experiment & \multicolumn{5}{c}{Ordered Relaxation Times} \\
           \\
VAMPnets & 7.7 & 9.1 & 55 & 65 & 1920 \\
 Varolg\"une & 2.72 & 3.1 & 33 & 65 & 1430 \\
\midrule
\midrule
     \textbf{run 0} &          $6.487\pm0.197$ &  $8.539\pm0.236$ & $10.391\pm1.138$ & $48.347\pm1.216$ & $3987.362\pm1194.609$ \\
     \textbf{run 1} &          $8.006\pm0.104$ &   $9.416\pm0.14$ & $32.721\pm3.164$ &  $72.885\pm1.87$ &  $7604.07\pm2878.833$ \\
     \textbf{run 2} &           $9.232\pm0.14$ & $14.948\pm0.202$ & $19.578\pm0.741$ & $58.735\pm2.173$ &    $262.676\pm37.344$ \\
     run 3 &          $6.384\pm0.123$ &  $7.728\pm0.154$ &   $9.477\pm0.21$ &  $74.77\pm1.998$ &   $755.092\pm202.717$ \\
     run 4 &          $3.773\pm0.072$ &  $5.614\pm0.112$ &  $5.908\pm0.116$ & $53.324\pm1.408$ &   $518.498\pm119.612$ \\
\bottomrule
\end{tabular}
\end{table}







\begin{table}
\centering
\caption{Prior transition rates of handpicked ADP models.}
\begin{tabular}{rccccc}
\toprule
       Experiment & \multicolumn{5}{c}{Transition Rates} \\
                  &                 run 0 &                 run 1 &                 run 2 &                 run 3 &                 run 4 \\
\midrule
$1 \rightarrow 2$ & $0.02617 \pm 0.00120$ & $0.00008 \pm 0.00004$ & $0.05732 \pm 0.00352$ & $0.03108 \pm 0.00214$ & $0.05294 \pm 0.00379$ \\
$1 \rightarrow 3$ & $0.00002 \pm 0.00001$ & $0.00011 \pm 0.00003$ & $0.00002 \pm 0.00001$ & $0.00003 \pm 0.00001$ & $0.00019 \pm 0.00006$ \\
$1 \rightarrow 4$ & $0.00849 \pm 0.00059$ & $0.02111 \pm 0.00126$ & $0.00007 \pm 0.00003$ & $0.00072 \pm 0.00016$ & $0.00793 \pm 0.00088$ \\
$1 \rightarrow 5$ & $0.00001 \pm 0.00000$ & $0.00001 \pm 0.00000$ & $0.00000 \pm 0.00000$ & $0.00002 \pm 0.00001$ & $0.00006 \pm 0.00003$ \\
$1 \rightarrow 6$ & $0.00003 \pm 0.00001$ & $0.00000 \pm 0.00000$ & $0.00002 \pm 0.00001$ & $0.00005 \pm 0.00002$ & $0.00002 \pm 0.00001$ \\
\midrule
$2 \rightarrow 1$ & $0.06101 \pm 0.00446$ & $0.00354 \pm 0.00030$ & $0.01415 \pm 0.00062$ & $0.04681 \pm 0.00401$ & $0.04728 \pm 0.00321$ \\
$2 \rightarrow 3$ & $0.00005 \pm 0.00002$ & $0.00022 \pm 0.00005$ & $0.00028 \pm 0.00009$ & $0.00117 \pm 0.00027$ & $0.00005 \pm 0.00003$ \\
$2 \rightarrow 4$ & $0.00081 \pm 0.00015$ & $0.00611 \pm 0.00040$ & $0.00638 \pm 0.00051$ & $0.01105 \pm 0.00112$ & $0.01198 \pm 0.00090$ \\
$2 \rightarrow 5$ & $0.00003 \pm 0.00001$ & $0.00001 \pm 0.00000$ & $0.00001 \pm 0.00000$ & $0.00004 \pm 0.00001$ & $0.00004 \pm 0.00002$ \\
$2 \rightarrow 6$ & $0.00001 \pm 0.00000$ & $0.00001 \pm 0.00001$ & $0.00001 \pm 0.00001$ & $0.00006 \pm 0.00002$ & $0.00001 \pm 0.00001$ \\
\midrule
$3 \rightarrow 1$ & $0.00054 \pm 0.00017$ & $0.00003 \pm 0.00001$ & $0.00005 \pm 0.00003$ & $0.00004 \pm 0.00002$ & $0.00028 \pm 0.00009$ \\
$3 \rightarrow 2$ & $0.00002 \pm 0.00001$ & $0.00010 \pm 0.00005$ & $0.00030 \pm 0.00012$ & $0.00149 \pm 0.00025$ & $0.00013 \pm 0.00005$ \\
$3 \rightarrow 4$ & $0.02035 \pm 0.00152$ & $0.02152 \pm 0.00105$ & $0.03408 \pm 0.00272$ & $0.02167 \pm 0.00205$ & $0.01678 \pm 0.00144$ \\
$3 \rightarrow 5$ & $0.00006 \pm 0.00002$ & $0.00001 \pm 0.00000$ & $0.00002 \pm 0.00002$ & $0.00016 \pm 0.00008$ & $0.00002 \pm 0.00001$ \\
$3 \rightarrow 6$ & $0.00000 \pm 0.00000$ & $0.00001 \pm 0.00000$ & $0.00007 \pm 0.00004$ & $0.00002 \pm 0.00001$ & $0.00004 \pm 0.00002$ \\
\midrule
$4 \rightarrow 1$ & $0.04081 \pm 0.00287$ & $0.00159 \pm 0.00014$ & $0.00167 \pm 0.00031$ & $0.00425 \pm 0.00062$ & $0.03553 \pm 0.00308$ \\
$4 \rightarrow 2$ & $0.00446 \pm 0.00049$ & $0.01857 \pm 0.00098$ & $0.02378 \pm 0.00177$ & $0.03856 \pm 0.00447$ & $0.02690 \pm 0.00270$ \\
$4 \rightarrow 3$ & $0.06591 \pm 0.00585$ & $0.01268 \pm 0.00090$ & $0.03333 \pm 0.00199$ & $0.03906 \pm 0.00343$ & $0.04051 \pm 0.00436$ \\
$4 \rightarrow 5$ & $0.00001 \pm 0.00000$ & $0.00000 \pm 0.00000$ & $0.00001 \pm 0.00000$ & $0.00014 \pm 0.00005$ & $0.00025 \pm 0.00011$ \\
$4 \rightarrow 6$ & $0.00011 \pm 0.00004$ & $0.00001 \pm 0.00001$ & $0.00005 \pm 0.00003$ & $0.00014 \pm 0.00007$ & $0.00001 \pm 0.00001$ \\
\midrule
$5 \rightarrow 1$ & $0.00021 \pm 0.00011$ & $0.00047 \pm 0.00023$ & $0.00004 \pm 0.00002$ & $0.00053 \pm 0.00022$ & $0.00017 \pm 0.00006$ \\
$5 \rightarrow 2$ & $0.00028 \pm 0.00012$ & $0.00003 \pm 0.00002$ & $0.00015 \pm 0.00007$ & $0.00030 \pm 0.00016$ & $0.00022 \pm 0.00011$ \\
$5 \rightarrow 3$ & $0.00005 \pm 0.00002$ & $0.00002 \pm 0.00002$ & $0.00008 \pm 0.00005$ & $0.00012 \pm 0.00008$ & $0.00032 \pm 0.00022$ \\
$5 \rightarrow 4$ & $0.00015 \pm 0.00007$ & $0.00048 \pm 0.00014$ & $0.00006 \pm 0.00004$ & $0.00110 \pm 0.00037$ & $0.00020 \pm 0.00015$ \\
$5 \rightarrow 6$ & $0.00333 \pm 0.00118$ & $0.00010 \pm 0.00005$ & $0.00384 \pm 0.00104$ & $0.00061 \pm 0.00026$ & $0.00301 \pm 0.00108$ \\
\midrule
$6 \rightarrow 1$ & $0.00115 \pm 0.00058$ & $0.00014 \pm 0.00009$ & $0.00103 \pm 0.00045$ & $0.00083 \pm 0.00035$ & $0.00115 \pm 0.00064$ \\
$6 \rightarrow 2$ & $0.00374 \pm 0.00166$ & $0.00028 \pm 0.00010$ & $0.00012 \pm 0.00006$ & $0.00051 \pm 0.00014$ & $0.00175 \pm 0.00075$ \\
$6 \rightarrow 3$ & $0.00055 \pm 0.00021$ & $0.00061 \pm 0.00033$ & $0.00047 \pm 0.00030$ & $0.00154 \pm 0.00059$ & $0.00046 \pm 0.00022$ \\
$6 \rightarrow 4$ & $0.00147 \pm 0.00064$ & $0.00009 \pm 0.00004$ & $0.00072 \pm 0.00041$ & $0.00040 \pm 0.00016$ & $0.00065 \pm 0.00037$ \\
$6 \rightarrow 5$ & $0.02942 \pm 0.00784$ & $0.00091 \pm 0.00040$ & $0.01787 \pm 0.00537$ & $0.00054 \pm 0.00027$ & $0.01870 \pm 0.00754$ \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}
\centering
\caption{Mean First-Passage Times of handpicked ADP models.}
\begin{tabular}{rccccc}
\toprule
       Experiment & \multicolumn{5}{c}{Mean First-Passage Times} \\
                  &                    run 0 &                    run 1 &                  run 2 &                  run 3 &                  run 4 \\
\midrule
$1 \rightarrow 2$ &           $67.7 \pm 5.0$ &          $138.3 \pm 7.3$ &         $18.3 \pm 1.2$ &         $34.2 \pm 2.4$ &         $27.6 \pm 2.4$ \\
$1 \rightarrow 3$ &         $296.5 \pm 22.1$ &         $301.5 \pm 19.1$ &       $378.4 \pm 31.4$ &       $417.9 \pm 49.2$ &       $291.3 \pm 26.6$ \\
$1 \rightarrow 4$ &         $165.7 \pm 11.4$ &           $48.3 \pm 3.0$ &       $212.3 \pm 15.3$ &       $224.7 \pm 21.8$ &        $106.6 \pm 6.2$ \\
$1 \rightarrow 5$ &   $23,622.4 \pm 4,958.8$ & $105,104.4 \pm 36,135.0$ & $32,596.9 \pm 9,185.9$ & $16,461.3 \pm 4,302.6$ & $13,689.3 \pm 4,112.6$ \\
$1 \rightarrow 6$ &   $23,611.8 \pm 4,707.3$ &  $93,687.7 \pm 28,995.4$ & $30,200.1 \pm 8,745.3$ & $15,393.9 \pm 3,993.9$ & $15,830.7 \pm 4,143.4$ \\
\midrule
$2 \rightarrow 1$ &           $18.2 \pm 1.4$ &         $381.0 \pm 29.4$ &        $110.2 \pm 6.9$ &         $39.6 \pm 4.8$ &         $32.4 \pm 2.8$ \\
$2 \rightarrow 3$ &         $310.8 \pm 22.3$ &         $369.2 \pm 21.5$ &       $360.7 \pm 31.3$ &       $390.1 \pm 49.2$ &       $287.8 \pm 26.3$ \\
$2 \rightarrow 4$ &         $180.2 \pm 11.6$ &          $121.9 \pm 5.6$ &       $194.5 \pm 15.2$ &       $197.1 \pm 21.6$ &        $102.7 \pm 5.9$ \\
$2 \rightarrow 5$ &   $23,624.4 \pm 4,958.7$ & $105,081.0 \pm 36,137.2$ & $32,591.8 \pm 9,186.6$ & $16,445.3 \pm 4,302.6$ & $13,691.0 \pm 4,112.1$ \\
$2 \rightarrow 6$ &   $23,615.4 \pm 4,706.7$ &  $93,642.7 \pm 28,997.5$ & $30,195.2 \pm 8,746.0$ & $15,389.2 \pm 3,993.0$ & $15,832.6 \pm 4,142.8$ \\
\midrule
$3 \rightarrow 1$ &         $143.2 \pm 13.0$ &         $476.2 \pm 29.5$ &       $220.4 \pm 14.8$ &       $143.0 \pm 13.2$ &       $131.2 \pm 11.3$ \\
$3 \rightarrow 2$ &         $202.5 \pm 16.3$ &          $137.3 \pm 7.3$ &       $119.2 \pm 10.3$ &       $110.5 \pm 10.9$ &       $133.2 \pm 11.0$ \\
$3 \rightarrow 4$ &           $55.2 \pm 4.2$ &           $47.5 \pm 2.4$ &         $35.8 \pm 3.7$ &         $60.3 \pm 5.8$ &         $63.6 \pm 5.5$ \\
$3 \rightarrow 5$ &   $23,564.4 \pm 4,964.4$ & $105,093.4 \pm 36,135.4$ & $32,462.5 \pm 9,186.3$ & $16,308.7 \pm 4,314.3$ & $13,691.3 \pm 4,108.4$ \\
$3 \rightarrow 6$ &   $23,569.2 \pm 4,708.2$ &  $93,679.3 \pm 28,996.9$ & $30,066.1 \pm 8,745.9$ & $15,376.4 \pm 3,990.4$ & $15,825.1 \pm 4,141.1$ \\
\midrule
$4 \rightarrow 1$ &          $95.5 \pm 10.9$ &         $430.3 \pm 28.9$ &       $188.1 \pm 12.8$ &       $100.7 \pm 11.0$ &         $72.0 \pm 7.9$ \\
$4 \rightarrow 2$ &         $154.7 \pm 14.3$ &           $90.8 \pm 5.9$ &         $86.7 \pm 8.1$ &         $68.4 \pm 8.5$ &         $73.8 \pm 7.7$ \\
$4 \rightarrow 3$ &         $131.7 \pm 15.4$ &         $254.8 \pm 19.1$ &       $175.5 \pm 19.5$ &       $219.8 \pm 34.3$ &       $188.3 \pm 24.1$ \\
$4 \rightarrow 5$ &   $23,577.8 \pm 4,960.4$ & $105,090.4 \pm 36,136.0$ & $32,510.4 \pm 9,185.4$ & $16,363.3 \pm 4,305.9$ & $13,668.9 \pm 4,111.7$ \\
$4 \rightarrow 6$ &   $23,572.3 \pm 4,707.2$ &  $93,656.7 \pm 28,996.9$ & $30,113.5 \pm 8,745.0$ & $15,365.5 \pm 3,989.6$ & $15,810.8 \pm 4,142.7$ \\
\midrule
$5 \rightarrow 1$ &        $904.8 \pm 210.0$ &      $1,283.0 \pm 276.3$ &    $1,741.9 \pm 378.2$ &       $535.7 \pm 73.7$ &      $897.7 \pm 222.8$ \\
$5 \rightarrow 2$ &        $930.2 \pm 213.8$ &      $1,148.9 \pm 242.4$ &    $1,674.2 \pm 376.4$ &       $519.7 \pm 74.7$ &      $894.2 \pm 223.0$ \\
$5 \rightarrow 3$ &      $1,108.6 \pm 200.2$ &      $1,306.1 \pm 240.9$ &    $1,854.6 \pm 382.7$ &       $729.4 \pm 95.6$ &    $1,034.9 \pm 234.7$ \\
$5 \rightarrow 4$ &        $991.8 \pm 202.2$ &      $1,068.5 \pm 243.6$ &    $1,732.3 \pm 377.0$ &       $560.3 \pm 84.5$ &      $912.2 \pm 226.5$ \\
$5 \rightarrow 6$ &    $4,587.7 \pm 1,895.2$ &  $85,954.8 \pm 27,283.8$ &  $2,718.7 \pm 1,151.3$ & $12,392.7 \pm 3,933.4$ &  $3,968.4 \pm 1,139.8$ \\
\midrule
$6 \rightarrow 1$ &        $768.5 \pm 188.8$ &      $1,318.3 \pm 233.3$ &    $1,604.6 \pm 365.3$ &       $419.9 \pm 60.0$ &      $787.1 \pm 208.8$ \\
$6 \rightarrow 2$ &        $792.8 \pm 193.1$ &      $1,097.3 \pm 227.3$ &    $1,539.1 \pm 363.0$ &       $403.2 \pm 59.0$ &      $783.2 \pm 209.2$ \\
$6 \rightarrow 3$ &        $971.9 \pm 178.8$ &      $1,198.5 \pm 249.7$ &    $1,719.4 \pm 370.6$ &       $541.6 \pm 91.6$ &      $935.4 \pm 212.6$ \\
$6 \rightarrow 4$ &        $855.2 \pm 179.9$ &      $1,042.0 \pm 229.9$ &    $1,596.4 \pm 364.6$ &       $449.7 \pm 64.3$ &      $806.6 \pm 209.1$ \\
$6 \rightarrow 5$ &    $4,649.1 \pm 1,584.4$ &  $60,313.6 \pm 28,321.1$ &  $3,966.7 \pm 1,520.9$ & $14,320.1 \pm 3,990.9$ &  $2,587.5 \pm 1,088.4$ \\
\bottomrule
\end{tabular}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Relaxation Times Plots}

\begin{figure}
    \centering
    \includegraphics[scale=0.7]{Figures/relax_times_handpicked.png}
    \caption{5 handpicked experiments. Relaxation times means and standard deviations as gaussians. Colors indicate run the relaxation times belong to. Dots on the x-axis indicate mean of largest relaxation time, which usually has very large standard deviation and is thus not visible.}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[scale=0.7]{Figures/relax_times_5+10.png}
    \caption{5 handpicked experiments and 10 further experiments (not handpicked). Relaxation times means and standard deviations as gaussians. Colors indicate run the relaxation times belong to. Dots on the x-axis indicate mean of largest relaxation time, which usually has very large standard deviation and is thus not visible.}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[scale=0.7]{Figures/relax_times_all_100.png}
    \caption{All 100 length time series experiments, including normalizing data and diagonal covariance matrix. Relaxation times means and standard deviations as gaussians. Colors indicate run the relaxation times belong to. Dots on the x-axis indicate mean of largest relaxation time, which usually has very large standard deviation and is thus not visible.}
\end{figure}




\begin{table}
\begin{tabular}{lrccccc}
\toprule
 Group & Experiment & \multicolumn{5}{c}{Ordered Relaxation Times} \\
 &              & & & & &  \\
\midrule
 VAMPnets & & 7.7 & 9.1 & 55 & 65 & 1920 \\
 Varolg\"une & & 2.72 & 3.1 & 33 & 65 & 1430 \\
\midrule
& run 4 &          $8.706\pm0.427$ &  $9.017\pm0.419$ & $42.836\pm11.849$ &    $69.012\pm4.302$ &  $773.558\pm205.017$ \\
\midrule
\end{tabular}
    \label{table:adp_selected_run_results}
\end{table}

\begin{figure}

   \centering
   \begin{align*}
   \begin{pmatrix}
    0. & 0.05294 & 0.00019 & 0.00793 & 0.00006 & 0.00002\\
    0.04728 & 0. & 0.00005 & 0.01198 & 0.00004 & 0.00001\\
    0.00028 & 0.00013 & 0. & 0.01678 & 0.00002 & 0.00004\\
    0.03553 & 0.0269 & 0.04051 & 0. & 0.00025 & 0.00001\\
    0.00017 & 0.00022 & 0.00032 & 0.00020 & 0. & 0.00301\\
    0.00115 & 0.00175 & 0.00046 & 0.00065 & 0.0187 & 0.\\
    \end{pmatrix}
    &\pm
\begin{pmatrix}
0. & 0.00379 & 0.00006 & 0.00088 & 0.00003 & 0.00001\\
0.00321 & 0. & 0.00003 & 0.00090 & 0.00002 & 0.00001\\
0.00009 & 0.00005 & 0. & 0.00144 & 0.00001 & 0.00002\\
0.00308 & 0.00270 & 0.00436 & 0. & 0.00011 & 0.00001\\
0.00006 & 0.00011 & 0.00022 & 0.00015 & 0. & 0.00108\\
0.00064 & 0.00075 & 0.00022 & 0.00037 & 0.00754 & 0.\\
\end{pmatrix}
    \\
    \begin{pmatrix}
   0. & 27.539 & 290.648 & 106.966 & 13726.715 & 15864.058\\
   32.459 & 0. & 287.114 & 102.982 & 13728.424 & 15865.984\\
   131.683 & 133.512 & 0. & 63.494 & 13729.080 & 15859.124\\
   72.53 & 74.224 & 187.246 & 0. & 13706.344 & 15844.268\\
   917.046 & 913.309 & 1054.649 & 932.254 & 0. & 3959.010\\
   804.452 & 800.225 & 952.336 & 824.08 & 2563.419 & 0.\\
   \end{pmatrix}
   &\pm
\begin{pmatrix}
0. & 2.387 & 26.618 & 6.218 & 4112.59 & 4143.375\\
2.76 & 0. & 26.342 & 5.890 & 4112.066 & 4142.836\\
11.292 & 11.033 & 0. & 5.459 & 4108.395 & 4141.139\\
7.91 & 7.714 & 24.109 & 0. & 4111.708 & 4142.651\\
222.806 & 222.997 & 234.733 & 226.489 & 0. & 1139.761\\
208.79 & 209.223 & 212.628 & 209.061 & 1088.398 & 0.\\
\end{pmatrix}
   \end{align*}
    \caption{Transition rates and Mean First-Passage Time for handpicked run 4.}
\label{figure:adp_selected_run_trans_rates}
\end{figure}

==> tables_and_matrices_dec_22.tex <==
\section{All Tables}

\subsection{Discrete Flashing Ratchet}
\begin{table}
\centering
\caption{Discrete Flashing Ratchet, selected experiments: learned prior parameters with internal standard deviation.}
\begin{tabular}{rccccc}
\toprule
            Experiment &     KL &   NLL &               $V$ &               $r$ &               $b$ \\
\midrule
          Ground Truth &      - &     - &   $1.000  $ &   $1.000  $ &   $1.000  $ \\
\midrule
   Irregular Grid Data & 20.580 & 0.197 & $1.061 \pm 0.021$ & $1.165 \pm 0.016$ & $1.141 \pm 0.021$ \\
      Shared Grid Data & 19.022 & 0.138 & $0.966 \pm 0.017$ & $1.166 \pm 0.016$ & $1.172 \pm 0.013$ \\
     Regular Grid Data & 21.952 & 0.173 & $0.984 \pm 0.050$ & $1.366 \pm 0.042$ & $1.390 \pm 0.039$ \\
Masked Posterior Rates & 16.766 & 0.238 & $1.010 \pm 0.021$ & $1.145 \pm 0.019$ & $1.165 \pm 0.019$ \\
Non-parametrized Prior & 18.174 & 0.218 &     - &     - &     - \\
\bottomrule
\end{tabular}
\end{table}



\begin{figure}
\centering
\begin{align*}
\begin{pmatrix}
0. & 0.607 & 0.368 & 1. & 0. & 0.\\
1.649 & 0. & 0.607 & 0. & 1. & 0.\\
2.718 & 1.649 & 0. & 0. & 0. & 1.\\
1. & 0. & 0. & 0. & 1. & 1.\\
0. & 1. & 0. & 1. & 0. & 1.\\
0. & 0. & 1. & 1. & 1. & 0.\\
\end{pmatrix}\\
& \begin{pmatrix}
0. & 0.710 & 0.448 & 1.169 & 0.044 & 0.038\\
1.878 & 0. & 0.772 & 0.073 & 1.119 & 0.032\\
3.105 & 1.844 & 0. & 0.115 & 0.065 & 1.263\\
1.349 & 0.071 & 0.047 & 0. & 1.020 & 1.029\\
0.095 & 1.083 & 0.042 & 1.124 & 0. & 1.098\\
0.123 & 0.074 & 0.969 & 1.366 & 1.157 & 0.\\
\end{pmatrix}
&\pm
\begin{pmatrix}
0. & 0.01 & 0.006 & 0.020 & 0.001 & 0.002\\
0.032 & 0. & 0.013 & 0.002 & 0.017 & 0.001\\
0.072 & 0.049 & 0. & 0.003 & 0.002 & 0.024\\
0.018 & 0.002 & 0.001 & 0. & 0.014 & 0.016\\
0.002 & 0.017 & 0.001 & 0.019 & 0. & 0.018\\
0.002 & 0.002 & 0.018 & 0.02 & 0.015 & 0.\\
\end{pmatrix}
\\ \end{align*}
\caption{Discrete flashing ratchet, selected experiment with no explicit prior. Top: true transition rates. Bottom: Learned prior transition rates with internal standard deviation.}
\end{figure}



\begin{table}
\centering
\caption{Discrete Flashing Ratchet, selected experiments: Accuracy on test set and at observations in prediction set.}
\begin{tabular}{rcccc}
\toprule
            Experiment &  Accuracy & \multicolumn{3}{c}{Accuracy prediction} \\
                       &   &                   1 &       5 &      10 \\
\midrule
   Irregular Grid Data &   $0.930$ &             $0.660$ & $0.510$ & $0.390$ \\
      Shared Grid Data &   $0.958$ &             $0.710$ & $0.520$ & $0.370$ \\
     Regular Grid Data &   $0.934$ &             $0.700$ & $0.470$ & $0.380$ \\
Masked Posterior Rates &   $0.919$ &             $0.660$ & $0.510$ & $0.380$ \\
Non-parametrized Prior &   $0.928$ &             $0.650$ & $0.500$ & $0.380$ \\
\bottomrule
\end{tabular}
\end{table}




\begin{table}
\centering
\caption{Discrete Flashing Ratchet, all experiments: learned prior parameters with mean and standard deviation of 5 runs.}
\begin{tabular}{rccccc}
\toprule
            Experiment &                 KL &               NLL &               $V$ &               $r$ &               $b$ \\
\midrule
          Ground Truth &                  - &                 - &           $1.000$ &           $1.000$ &           $1.000$ \\
\midrule
   Irregular Grid Data & $20.095 \pm 1.211$ & $0.215 \pm 0.012$ & $0.983 \pm 0.046$ & $1.106 \pm 0.056$ & $1.127 \pm 0.039$ \\
      Shared Grid Data & $18.650 \pm 0.233$ & $0.145 \pm 0.005$ & $0.954 \pm 0.026$ & $1.180 \pm 0.035$ & $1.137 \pm 0.057$ \\
     Regular Grid Data & $21.693 \pm 0.710$ & $0.179 \pm 0.018$ & $0.995 \pm 0.051$ & $1.371 \pm 0.047$ & $1.360 \pm 0.047$ \\
Masked Posterior Rates & $17.111 \pm 0.396$ & $0.221 \pm 0.015$ & $0.990 \pm 0.017$ & $1.175 \pm 0.042$ & $1.163 \pm 0.032$ \\
Non-parametrized Prior & $17.618 \pm 0.583$ & $0.217 \pm 0.010$ &                 - &                 - &                 - \\
\bottomrule
\end{tabular}
\end{table}



\begin{figure}
\centering
\begin{align*}
\begin{pmatrix}
0. & 0.607 & 0.368 & 1. & 0. & 0.\\
1.649 & 0. & 0.607 & 0. & 1. & 0.\\
2.718 & 1.649 & 0. & 0. & 0. & 1.\\
1. & 0. & 0. & 0. & 1. & 1.\\
0. & 1. & 0. & 1. & 0. & 1.\\
0. & 0. & 1. & 1. & 1. & 0.\\
\end{pmatrix}\\
& \begin{pmatrix}
0. & 0.672 & 0.433 & 1.118 & 0.048 & 0.042\\
1.769 & 0. & 0.714 & 0.101 & 1.121 & 0.048\\
2.872 & 1.738 & 0. & 0.114 & 0.079 & 1.15\\
1.320 & 0.069 & 0.050 & 0. & 1.054 & 1.041\\
0.103 & 1.091 & 0.045 & 1.147 & 0. & 1.154\\
0.134 & 0.066 & 0.903 & 1.277 & 1.211 & 0.\\
\end{pmatrix}
&\pm
\begin{pmatrix}
0. & 0.038 & 0.012 & 0.030 & 0.002 & 0.002\\
0.093 & 0. & 0.034 & 0.016 & 0.043 & 0.01\\
0.167 & 0.085 & 0. & 0.015 & 0.015 & 0.12\\
0.025 & 0.006 & 0.004 & 0. & 0.024 & 0.065\\
0.011 & 0.028 & 0.003 & 0.056 & 0. & 0.087\\
0.015 & 0.006 & 0.078 & 0.116 & 0.051 & 0.\\
\end{pmatrix}
\\ \end{align*}
\caption{Discrete flashing ratchet, all experiments. Top: true transition rates. Bottom: Learned prior transition rates with mean and standard deviation of 5 runs.}
\end{figure}



\begin{table}
\centering
\caption{Discrete Flashing Ratchet, all experiments: Accuracy on test set and at observations in prediction set with mean and standard deviation for 5 runs}
\begin{tabular}{rcccc}
\toprule
            Experiment &          Accuracy & \multicolumn{3}{c}{Accuracy prediction} \\
                       &           &                   1 &                 5 &                10 \\
\midrule
   Irregular Grid Data & $0.927 \pm 0.003$ &   $0.644 \pm 0.013$ & $0.514 \pm 0.011$ & $0.390 \pm 0.007$ \\
      Shared Grid Data & $0.950 \pm 0.005$ &   $0.706 \pm 0.017$ & $0.508 \pm 0.028$ & $0.348 \pm 0.016$ \\
     Regular Grid Data & $0.932 \pm 0.010$ &   $0.708 \pm 0.008$ & $0.470 \pm 0.014$ & $0.370 \pm 0.010$ \\
Masked Posterior Rates & $0.924 \pm 0.005$ &   $0.664 \pm 0.011$ & $0.516 \pm 0.009$ & $0.390 \pm 0.010$ \\
Non-parametrized Prior & $0.925 \pm 0.005$ &   $0.646 \pm 0.017$ & $0.512 \pm 0.018$ & $0.388 \pm 0.004$ \\
\bottomrule
\end{tabular}
\end{table}

\subsection{Lotka-Volterra}
\begin{table}
\centering
\caption{Lotka-Volterra, selected experiments: learned prior parameters with internal standard deviation.}
\begin{tabular}{rcccccc}
\toprule
                          Experiment &     KL &    NLL &                $\alpha$ &                 $\beta$ &                $\delta$ &                $\gamma$ \\
\midrule
                        Ground Truth &      - &      - &      $\num{5.00e-04}  $ &      $\num{1.00e-04}  $ &      $\num{1.00e-04}  $ &      $\num{5.00e-04}  $ \\
  Oppers Results, Mean as Prediction &      - &      - &      $\num{1.35e-03}  $ &      $\num{2.32e-04}  $ &      $\num{1.78e-04}  $ &      $\num{1.57e-03}  $ \\
Oppers Results, Prior for Prediction &      - &      - &      $\num{1.35e-03}  $ &      $\num{2.32e-04}  $ &      $\num{1.78e-04}  $ &      $\num{1.57e-03}  $ \\
\midrule
                 Irregular Grid Data &  24.51 & 164.78 & $\num{4.50e-04} \pm \num{2.67e-05}$ & $\num{9.98e-05} \pm \num{7.55e-06}$ & $\num{7.62e-05} \pm \num{8.37e-06}$ & $\num{3.56e-04} \pm \num{2.23e-05}$ \\
                    Shared Grid Data &  31.31 & 153.28 & $\num{5.52e-04} \pm \num{1.02e-05}$ & $\num{1.13e-04} \pm \num{3.85e-06}$ & $\num{9.79e-05} \pm \num{4.35e-06}$ & $\num{4.93e-04} \pm \num{8.81e-06}$ \\
                   Regular Grid Data &  25.53 & 158.97 & $\num{4.37e-04} \pm \num{1.40e-05}$ & $\num{9.51e-05} \pm \num{5.96e-06}$ & $\num{9.81e-05} \pm \num{7.26e-06}$ & $\num{4.91e-04} \pm \num{1.05e-05}$ \\
             Opper Data, our Results & 108.57 & -10.58 & $\num{2.53e-04} \pm \num{1.05e-05}$ & $\num{6.41e-05} \pm \num{4.41e-06}$ & $\num{1.02e-04} \pm \num{6.53e-06}$ & $\num{4.15e-04} \pm \num{1.59e-05}$ \\
\bottomrule
\end{tabular}
\end{table}



\begin{table}
\centering
\caption{Lotka-Volterra, selected experiments: Accuracy on test set and at observations in prediction set. Prediction set for opper contains non-noisy observations of trajectory after the test set.}
\begin{tabular}{rcccc}
\toprule
                          Experiment & RMSE test & \multicolumn{3}{c}{RMSE prediction} \\
                                     &   &               1 &       5 &       10 \\
\midrule
  Oppers Results, Mean as Prediction &   $2.672$ &         $2.549$ & $6.524$ &  $8.024$ \\
Oppers Results, Prior for Prediction &   $2.672$ &         $3.000$ & $9.487$ & $11.402$ \\
\midrule
                 Irregular Grid Data &   $1.871$ &         $2.270$ & $2.676$ &  $2.973$ \\
                    Shared Grid Data &   $1.635$ &         $2.305$ & $2.802$ &  $3.253$ \\
                   Regular Grid Data &   $1.740$ &         $1.896$ & $2.293$ &  $2.678$ \\
             Opper Data, our Results &   $2.070$ &         $5.099$ & $3.000$ &  $1.414$ \\
\bottomrule
\end{tabular}
\end{table}



\begin{table}
\centering
\caption{Lotka-Volterra, all experiments: learned prior parameters with mean and standard deviation of 5 runs.}
\begin{tabular}{rcccccc}
\toprule
                          Experiment &                        KL &                       NLL &                  $\alpha$ &                   $\beta$ &                  $\delta$ &                  $\gamma$ \\
\midrule
                        Ground Truth &                         - &                         - &               $\num{5.000e-04}$ &               $\num{1.000e-04}$ &               $\num{1.000e-04}$ &               $\num{5.000e-04}$ \\
  Oppers Results, Mean as Prediction &                         - &                         - &               $\num{1.350e-03}$ &               $\num{2.320e-04}$ &               $\num{1.780e-04}$ &               $\num{1.570e-03}$ \\
Oppers Results, Prior for Prediction &                         - &                         - &               $\num{1.350e-03}$ &               $\num{2.320e-04}$ &               $\num{1.780e-04}$ &               $\num{1.570e-03}$ \\
\midrule
                 Irregular Grid Data & $\num{2.519e+01} \pm \num{1.342e+00}$ & $\num{1.628e+02} \pm \num{1.490e+00}$ & $\num{4.275e-04} \pm \num{6.178e-05}$ & $\num{9.408e-05} \pm \num{7.386e-06}$ & $\num{8.315e-05} \pm \num{8.595e-06}$ & $\num{4.059e-04} \pm \num{4.265e-05}$ \\
                    Shared Grid Data & $\num{3.596e+01} \pm \num{4.400e+00}$ & $\num{1.552e+02} \pm \num{2.038e+00}$ & $\num{5.495e-04} \pm \num{5.736e-05}$ & $\num{1.102e-04} \pm \num{7.342e-06}$ & $\num{1.002e-04} \pm \num{5.670e-06}$ & $\num{4.939e-04} \pm \num{4.364e-05}$ \\
                   Regular Grid Data & $\num{2.793e+01} \pm \num{4.849e+00}$ & $\num{1.627e+02} \pm \num{3.915e+00}$ & $\num{4.511e-04} \pm \num{6.368e-05}$ & $\num{9.736e-05} \pm \num{2.680e-06}$ & $\num{8.919e-05} \pm \num{8.398e-06}$ & $\num{4.308e-04} \pm \num{5.625e-05}$ \\
             Opper Data, our Results & $\num{1.921e+02} \pm \num{1.211e+02}$ & $\num{1.355e+01} \pm \num{2.471e+01}$ & $\num{2.084e-04} \pm \num{6.452e-05}$ & $\num{6.707e-05} \pm \num{5.880e-06}$ & $\num{1.048e-04} \pm \num{3.198e-05}$ & $\num{9.279e-04} \pm \num{8.181e-04}$ \\
\bottomrule
\end{tabular}
\end{table}



\begin{table}
\centering
\caption{Lotka-Volterra, all experiments: RMSE on test set and at observations in prediction set. Prediction set for opper contains non-noisy observations of trajectory after the test set.}
\begin{tabular}{rcccc}
\toprule
                          Experiment &                 RMSE test & \multicolumn{3}{c}{RMSE prediction} \\
                                     &                   &                         1 &                         5 &                        10 \\
\midrule
  Oppers Results, Mean as Prediction &               $\num{2.672e+00}$ &               $\num{2.549e+00}$ &               $\num{6.524e+00}$ &               $\num{8.024e+00}$ \\
Oppers Results, Prior for Prediction &               $\num{2.672e+00}$ &               $\num{3.000e+00}$ &               $\num{9.487e+00}$ &               $\num{1.140e+01}$ \\
\midrule
                 Irregular Grid Data & $\num{1.835e+00} \pm \num{3.233e-02}$ & $\num{2.282e+00} \pm \num{6.169e-02}$ & $\num{2.555e+00} \pm \num{7.736e-02}$ & $\num{2.926e+00} \pm \num{6.273e-02}$ \\
                    Shared Grid Data & $\num{1.671e+00} \pm \num{3.501e-02}$ & $\num{2.384e+00} \pm \num{5.204e-02}$ & $\num{2.828e+00} \pm \num{4.128e-02}$ & $\num{3.281e+00} \pm \num{3.272e-02}$ \\
                   Regular Grid Data & $\num{1.819e+00} \pm \num{8.380e-02}$ & $\num{1.993e+00} \pm \num{1.419e-01}$ & $\num{2.361e+00} \pm \num{1.141e-01}$ & $\num{2.760e+00} \pm \num{8.612e-02}$ \\
             Opper Data, our Results & $\num{2.031e+00} \pm \num{5.881e-02}$ & $\num{6.505e+00} \pm \num{3.295e+00}$ & $\num{8.081e+00} \pm \num{4.887e+00}$ & $\num{8.052e+00} \pm \num{5.451e+00}$ \\
\bottomrule
\end{tabular}
\end{table}
\subsection{Brownian Dynamics / Toy Protein Folding}



\begin{table}
\centering
\caption{Toy Protein Folding, selected experiment: NLL and KL on test set}
\begin{tabular}{rcc}
\toprule
Experiment &      KL &       NLL \\
\midrule
      Ours & $1.614$ & $542.230$ \\
\bottomrule
\end{tabular}
\end{table}




\begin{table}
\centering
\caption{Toy Protein Folding, selected experiment: RMSE on test set and at observations in prediction set.}
\begin{tabular}{rcccc}
\toprule
Experiment & RMSE test & \multicolumn{3}{c}{RMSE prediction} \\
           &   &               1 &      25 &      50 \\
\midrule
      Ours &   $2.438$ &         $2.439$ & $2.419$ & $2.481$ \\
\bottomrule
\end{tabular}
\end{table}




\begin{table}
\centering
\caption{Toy Protein Folding, selected experiment: Equilibrium distribution.}
\begin{tabular}{rc}
\toprule
Experiment &            Equilibrium \\
\midrule
  VAMPnets & [$0.72727$, $0.27273$] \\
\midrule
      Ours & [$0.75959$, $0.24041$] \\
\bottomrule
\end{tabular}
\end{table}



\begin{figure}
\centering
\begin{align*}
\begin{pmatrix}
0. & 0.03\\
0.093 & 0.\\
\end{pmatrix}
\pm
\begin{pmatrix}
0. & 0.02\\
0.054 & 0.\\
\end{pmatrix}
\\ \end{align*}
\caption{Toy Protein Folding, selected experiment: Learned prior transition rates with internal standard deviation.}
\end{figure}



\begin{table}
\centering
\caption{Toy Protein Folding, all experiments: NLL and KL on test set with mean and standard deviation of 5 runs.}
\begin{tabular}{rcc}
\toprule
Experiment &                KL &                 NLL \\
\midrule
      Ours & $1.408 \pm 0.168$ & $542.815 \pm 0.692$ \\
\bottomrule
\end{tabular}
\end{table}




\begin{table}
\centering
\caption{Toy Protein Folding, all experiment: RMSE on test set and at observations in prediction set with mean and standard deviation of 5 runs.}
\begin{tabular}{rcccc}
\toprule
Experiment &         RMSE test & \multicolumn{3}{c}{RMSE prediction} \\
           &           &                 1 &                25 &                50 \\
\midrule
      Ours & $2.437 \pm 0.002$ & $2.437 \pm 0.003$ & $2.418 \pm 0.001$ & $2.478 \pm 0.002$ \\
\bottomrule
\end{tabular}
\end{table}




\begin{table}
\centering
\caption{Toy Protein Folding, all experiments: Equilibrium distribution with mean and standard deviation of 5 runs.}
\begin{tabular}{rc}
\toprule
Experiment &                                    Equilibrium \\
\midrule
  VAMPnets &                         [$0.72727$, $0.27273$] \\
\midrule
      Ours & [$0.75489 \pm 0.01687$, $0.24511 \pm 0.01687$] \\
\bottomrule
\end{tabular}
\end{table}



\begin{figure}
\centering
\begin{align*}
\begin{pmatrix}
0. & 0.028\\
0.086 & 0.\\
\end{pmatrix}
\pm
\begin{pmatrix}
0. & 0.005\\
0.009 & 0.\\
\end{pmatrix}
\\ \end{align*}
\caption{Toy Protein Folding, all experiments: Learned transition rates with mean and standard deviation of 5 runs.}
\end{figure}
\subsection{Alanine Dipeptide}



\begin{table}
\centering
\caption{Alanine Dipeptide, selected experiment: NLL and KL on test set.}
\begin{tabular}{rcc}
\toprule
            Experiment &        KL &         NLL \\
\midrule
              VAMPnets &         - &           - \\
\midrule
$2$ States, Left-Right & $0.00061$ & $262.01837$ \\
$2$ States, Top-Bottom & $0.00011$ & $581.10406$ \\
            $3$ States & $1.51055$ & $110.85298$ \\
            $6$ States & $9.75118$ & $-69.10447$ \\
\bottomrule
\end{tabular}
\end{table}



\begin{table}
\centering
\caption{Alanine Dipeptide, selected experiment: RMSE on test set and at observations in prediction set.}
\begin{tabular}{rcccccccc}
\toprule
            Experiment & RMSE test & \multicolumn{7}{c}{RMSE prediction} \\
                       &   &               1 &       2 &       3 &       4 &       5 &      10 &      20 \\
\midrule
$2$ States, Left-Right &   $1.018$ &         $0.983$ & $0.976$ & $0.993$ & $1.005$ & $1.009$ & $1.022$ & $1.025$ \\
$2$ States, Top-Bottom &   $1.004$ &         $0.837$ & $0.829$ & $0.848$ & $0.868$ & $0.876$ & $0.914$ & $0.951$ \\
            $3$ States &   $0.669$ &         $0.725$ & $0.711$ & $0.736$ & $0.756$ & $0.770$ & $0.852$ & $0.915$ \\
            $6$ States &   $0.628$ &         $0.691$ & $0.711$ & $0.721$ & $0.703$ & $0.758$ & $0.841$ & $0.928$ \\
\bottomrule
\end{tabular}
\end{table}




\begin{table}
\centering
\caption{Alanine Dipeptide, selected experiment: Equilibrium distribution.}
\begin{tabular}{rc}
\toprule
            Experiment &                                                       Equilibrium \\
\midrule
              VAMPnets & [$0.30017$, $0.23837$, $0.1936$, $0.14458$, $0.10904$, $0.01424$] \\
\midrule
$2$ States, Left-Right &                                              [$0.0172$, $0.9828$] \\
$2$ States, Top-Bottom &                                            [$0.53817$, $0.46183$] \\
            $3$ States &                                  [$0.68751$, $0.19979$, $0.1127$] \\
            $6$ States &  [$0.36016$, $0.30057$, $0.23869$, $0.10041$, $0.00015$, $2e-05$] \\
\bottomrule
\end{tabular}
\end{table}



\begin{figure}
\centering
\begin{align*}
\begin{pmatrix}
\num{0.e+00} & \num{5.17e-07}\\
\num{6.03e-07} & \num{0.e+00}\\
\end{pmatrix}\\
\begin{pmatrix}
\num{0.e+00} & \num{1.39e-06}\\
\num{2.44e-08} & \num{0.e+00}\\
\end{pmatrix}\\
\begin{pmatrix}
\num{0.e+00} & \num{2.89e-03} & \num{8.64e-04}\\
\num{9.71e-03} & \num{0.e+00} & \num{2.68e-04}\\
\num{5.72e-03} & \num{2.82e-05} & \num{0.e+00}\\
\end{pmatrix}\\
\begin{pmatrix}
\num{0.e+00} & \num{5.08e-02} & \num{1.57e-04} & \num{6.99e-03} & \num{4.36e-08} & \num{5.10e-08}\\
\num{5.64e-02} & \num{0.e+00} & \num{4.41e-05} & \num{1.43e-02} & \num{3.37e-08} & \num{2.18e-08}\\
\num{2.66e-04} & \num{1.49e-04} & \num{0.e+00} & \num{1.80e-02} & \num{3.27e-08} & \num{8.39e-08}\\
\num{3.84e-02} & \num{2.90e-02} & \num{4.31e-02} & \num{0.e+00} & \num{8.45e-08} & \num{8.73e-08}\\
\num{4.57e-05} & \num{3.55e-06} & \num{7.73e-07} & \num{1.25e-04} & \num{0.e+00} & \num{2.54e-03}\\
\num{4.62e-04} & \num{2.22e-03} & \num{3.25e-04} & \num{5.46e-04} & \num{1.88e-02} & \num{0.e+00}\\
\end{pmatrix}
\\ \end{align*}
\caption{Alanine Dipeptide, selected experiment: Learned prior transition rates with internal standard deviation. Order: 2 states top-bottom, 2 states left-right, 3 states, 6 states.}
\end{figure}



\begin{table}
\centering
\caption{Alanine Dipeptide, all experiment: NLL and KL on test set with mean and standard deviation of all runs.}
\begin{tabular}{rcc}
\toprule
            Experiment &                KL &                   NLL \\
\midrule
              VAMPnets &                 - &                     - \\
\midrule
$2$ States, Left-Right & $0.005 \pm 0.006$ &  $219.988 \pm 59.439$ \\
$2$ States, Top-Bottom & $0.862 \pm 0.875$ & $463.860 \pm 132.803$ \\
            $3$ States & $1.535 \pm 0.083$ &   $83.419 \pm 15.404$ \\
            $6$ States & $6.053 \pm 3.039$ &  $-31.134 \pm 25.835$ \\
\bottomrule
\end{tabular}
\end{table}



\begin{table}
\centering
\caption{Alanine Dipeptide, all experiments: RMSE on test set and at observations in prediction with mean and standard deviation of all runs.}
\begin{tabular}{rcccccccc}
\toprule
            Experiment &         RMSE test & \multicolumn{7}{c}{RMSE prediction} \\
                       &           &                 1 &                 2 &                 3 &                 4 &                 5 &                10 &                20 \\
\midrule
$2$ States, Left-Right & $1.015 \pm 0.003$ & $0.981 \pm 0.003$ & $0.972 \pm 0.005$ & $0.991 \pm 0.003$ & $1.003 \pm 0.003$ & $1.007 \pm 0.003$ & $1.020 \pm 0.003$ & $1.020 \pm 0.007$ \\
$2$ States, Top-Bottom & $0.912 \pm 0.121$ & $0.895 \pm 0.073$ & $0.891 \pm 0.075$ & $0.910 \pm 0.077$ & $0.929 \pm 0.078$ & $0.940 \pm 0.083$ & $0.987 \pm 0.080$ & $1.029 \pm 0.084$ \\
            $3$ States & $0.680 \pm 0.012$ & $0.735 \pm 0.022$ & $0.722 \pm 0.021$ & $0.744 \pm 0.020$ & $0.757 \pm 0.023$ & $0.770 \pm 0.022$ & $0.852 \pm 0.021$ & $0.909 \pm 0.017$ \\
            $6$ States & $0.670 \pm 0.066$ & $0.674 \pm 0.036$ & $0.674 \pm 0.035$ & $0.706 \pm 0.042$ & $0.702 \pm 0.032$ & $0.735 \pm 0.025$ & $0.819 \pm 0.032$ & $0.893 \pm 0.026$ \\
\bottomrule
\end{tabular}
\end{table}




\begin{table}
\centering
\caption{Alanine Dipeptide, all experiments: Equilibrium distribution.}
\begin{tabular}{rcccccccc}
\toprule
            Experiment &                                                                                                                               Equilibrium \\
\midrule
              VAMPnets &                                                                         [$0.30017$, $0.23837$, $0.1936$, $0.14458$, $0.10904$, $0.01424$] \\
\midrule
$2$ States, Left-Right &                                                                                            [$0.02673 \pm 0.00953$, $0.97327 \pm 0.00953$] \\
$2$ States, Top-Bottom &                                                                                            [$0.65445 \pm 0.09161$, $0.34555 \pm 0.09161$] \\
            $3$ States &                                                                       [$0.7166 \pm 0.01919$, $0.25549 \pm 0.03036$, $0.0279 \pm 0.04303$] \\
            $6$ States & [$0.27193 \pm 0.16729$, $0.39141 \pm 0.14505$, $0.18802 \pm 0.03993$, $0.14108 \pm 0.07145$, $0.0068 \pm 0.00814$, $0.00076 \pm 0.00091$] \\
\bottomrule
\end{tabular}
\end{table}



\begin{figure}
\centering
\begin{align*}
& \begin{pmatrix}
\num{0.e+00} & \num{2.21e-03}\\
\num{5.32e-03} & \num{0.e+00}\\
\end{pmatrix}
&\pm
\begin{pmatrix}
\num{0.e+00} & \num{1.75e-03}\\
\num{3.78e-03} & \num{0.e+00}\\
\end{pmatrix}\\
& \begin{pmatrix}
\num{0.e+00} & \num{4.46e-05}\\
\num{1.66e-06} & \num{0.e+00}\\
\end{pmatrix}
&\pm
\begin{pmatrix}
\num{0.e+00} & \num{4.32e-05}\\
\num{1.64e-06} & \num{0.e+00}\\
\end{pmatrix}\\
& \begin{pmatrix}
\num{0.e+00} & \num{3.69e-03} & \num{1.77e-04}\\
\num{1.03e-02} & \num{0.e+00} & \num{5.54e-05}\\
\num{1.74e-03} & \num{1.92e-05} & \num{0.e+00}\\
\end{pmatrix}
&\pm
\begin{pmatrix}
\num{0.e+00} & \num{4.54e-04} & \num{3.43e-04}\\
\num{4.2e-04} & \num{0.e+00} & \num{1.06e-04}\\
\num{1.99e-03} & \num{9.65e-06} & \num{0.e+00}\\
\end{pmatrix}
\\ \end{align*}
\caption{Alanine Dipeptide, selected experiment: Learned prior transition rates with internal standard deviation. Order: 2 states top-bottom, 2 states left-right, 3 states, 6 states.}
\end{figure}
\subsection{One-Dimensional, Two Mode Hybrid System}



\begin{table}
\centering
\caption{u1D synthetic SSDE, selected experiment: NLL and KL on test set.}
\begin{tabular}{rcc}
\toprule
   Experiment &         KL &         NLL \\
\midrule
 Ground Truth &          - &           - \\
Koehs Results &          - &           - \\
\midrule
         Ours & $11.75765$ & $168.45613$ \\
\bottomrule
\end{tabular}
\end{table}



\begin{table}
\centering
\caption{1D synthetic SSDE, selected experiment: Equilibrium distribution.}
\begin{tabular}{rc}
\toprule
   Experiment &            Equilibrium \\
\midrule
 Ground Truth &         [$0.5$, $0.5$] \\
Koehs Results & [$0.49606$, $0.50394$] \\
\midrule
         ours & [$0.51625$, $0.48375$] \\
\bottomrule
\end{tabular}
\end{table}



\begin{figure}
\centering
\begin{align*}
\begin{pmatrix}
-0.2 & 0.2\\
0.2 & -0.2\\
\end{pmatrix}\\
\begin{pmatrix}
-0.64 & 0.64\\
0.63 & -0.63\\
\end{pmatrix}\\
\begin{pmatrix}
0. & 0.208\\
0.222 & 0.\\
\end{pmatrix}
\\ \end{align*}
\caption{1D synthetic SSDE, selected experiment: Learned prior transition rates with internal standard deviation. }
\end{figure}



\begin{table}
\centering
\caption{1D synthetic SSDE, all experiments: NLL and KL on test set with mean and standard deviation.}
\begin{tabular}{rcc}
\toprule
   Experiment &                      KL &                      NLL \\
\midrule
 Ground Truth &                       - &                        - \\
Koehs Results &                       - &                        - \\
\midrule
         Ours & $50.22557 \pm 65.90845$ & $155.64621 \pm 28.65718$ \\
\bottomrule
\end{tabular}
\end{table}



\begin{table}
\centering
\caption{1D synthetic SSDE, all experiments: Equilibrium distribution with mean and standard deviation.}
\begin{tabular}{rc}
\toprule
   Experiment &                                    Equilibrium \\
\midrule
 Ground Truth &                                 [$0.5$, $0.5$] \\
Koehs Results &                         [$0.49606$, $0.50394$] \\
\midrule
         Ours & [$0.64747 \pm 0.16666$, $0.35253 \pm 0.16666$] \\
\bottomrule
\end{tabular}
\end{table}



\begin{figure}
\centering
\begin{align*}
\begin{pmatrix}
-0.2 & 0.2\\
0.2 & -0.2\\
\end{pmatrix}\\
\begin{pmatrix}
-0.64 & 0.64\\
0.63 & -0.63\\
\end{pmatrix}\\
& \begin{pmatrix}
-0.120 & 0.230\\
0.736 & -0.119\\
\end{pmatrix}
&\pm
\begin{pmatrix}
0.223 & 0.179\\
0.895 & 0.22\\
\end{pmatrix}
\\ \end{align*}
\caption{1D synthetic SSDE, all experiment: Learned prior transition rates with mean and standard deviation. Order from top to bottom: True transition rates, Koehs result, all of our runs and our runs with 1 outlier dropped. }
\end{figure}
\subsection{Switching Ion Channel Data}



\begin{table}
\centering
\caption{Ion Channel, selected experiment: NLL and KL on various test sets.}
\begin{tabular}{rcc}
\toprule
                                Experiment &         KL &            NLL \\
\midrule
      Koehs Result, Prediction after Train &          - &              - \\
         Koehs Result, Prediction on Train &          - &              - \\
\midrule
Train on $1$st sec, Prediction after Train & $19.26165$ & $-2,709.69348$ \\
   Train on $1$st sec, Prediction on Train &  $3.91216$ & $-2,707.44351$ \\
                     Train on $1$st second &  $4.83199$ & $-1,853.32846$ \\
                     Train on $2$nd second & $18.03612$ & $-2,605.92021$ \\
                     Train on full dataset &  $7.25939$ & $-2,695.86691$ \\
\bottomrule
\end{tabular}
\end{table}



\begin{table}
\centering
\caption{Ion Channel, selected experiment: RMSE on test set and at observations in various prediction sets.}
\begin{tabular}{rccccccccc}
\toprule
                                Experiment &  RMSE test & \multicolumn{8}{c}{RMSE prediction} \\
                                           &    &               1 &          2 &          3 &          4 &          5 &         10 &         50 &         90 \\
\midrule
      Koehs Result, Prediction after Train &      - &      $\num{9.31e-16}$ & $\num{3.11e-13}$ & $\num{3.93e-13}$ & $\num{1.61e-13}$ & $\num{2.68e-13}$ & $\num{3.58e-13}$ & $\num{6.56e-12}$ & $\num{6.62e-12}$ \\
         Koehs Result, Prediction on Train &      - &      $\num{2.61e-13}$ & $\num{2.26e-13}$ & $\num{2.26e-13}$ & $\num{2.58e-13}$ & $\num{2.89e-13}$ & $\num{2.75e-13}$ & $\num{1.90e-12}$ & $\num{2.47e-12}$ \\
\midrule
   Train on $1$st sec, Prediction on Train & $\num{4.23e-13}$ &      $\num{2.73e-13}$ & $\num{2.33e-13}$ & $\num{2.25e-13}$ & $\num{2.50e-13}$ & $\num{2.74e-13}$ & $\num{2.83e-13}$ & $\num{1.91e-12}$ & $\num{2.76e-12}$ \\
Train on $1$st sec, Prediction after Train & $\num{5.06e-13}$ &      $\num{2.94e-13}$ & $\num{5.98e-14}$ & $\num{3.72e-13}$ & $\num{4.54e-13}$ & $\num{2.22e-13}$ & $\num{2.60e-13}$ & $\num{6.68e-12}$ & $\num{6.31e-12}$ \\
                     Train on $1$st second & $\num{1.58e-12}$ &      $\num{2.08e-12}$ & $\num{2.07e-12}$ & $\num{2.08e-12}$ & $\num{2.08e-12}$ & $\num{2.21e-12}$ & $\num{2.35e-12}$ & $\num{2.63e-12}$ & $\num{1.82e-12}$ \\
                     Train on $2$nd second & $\num{1.86e-12}$ &      $\num{2.03e-12}$ & $\num{2.00e-12}$ & $\num{1.95e-12}$ & $\num{1.90e-12}$ & $\num{1.90e-12}$ & $\num{2.01e-12}$ & $\num{1.74e-12}$ & $\num{2.56e-12}$ \\
                     Train on full dataset & $\num{4.67e-13}$ &      $\num{2.99e-13}$ & $\num{2.62e-13}$ & $\num{2.89e-13}$ & $\num{5.27e-13}$ & $\num{1.00e-12}$ & $\num{2.04e-12}$ & $\num{2.78e-12}$ & $\num{1.05e-12}$ \\
\bottomrule
\end{tabular}
\end{table}



\begin{table}
\centering
\caption{Ion Channel, selected experiment: Equilibrium distribution.}
\begin{tabular}{rc}
\toprule
                                Experiment &                       Equilibrium \\
\midrule
      Koehs Result, Prediction after Train & [$0.17961$, $0.14987$, $0.67052$] \\
         Koehs Result, Prediction on Train & [$0.17961$, $0.14987$, $0.67052$] \\
\midrule
   Train on $1$st sec, Prediction on Train & [$0.18197$, $0.08677$, $0.73126$] \\
Train on $1$st sec, Prediction after Train &   [$0.17705$, $0.08795$, $0.735$] \\
                     Train on $1$st second & [$0.17491$, $0.09381$, $0.73128$] \\
                     Train on $2$nd second & [$0.67787$, $0.00346$, $0.31867$] \\
                     Train on full dataset & [$0.19588$, $0.07105$, $0.73307$] \\
\bottomrule
\end{tabular}
\end{table}



\begin{figure}
\centering
\begin{align*}
\begin{pmatrix}
-30.16 & 18.58 & 11.58\\
23.35 & -67.68 & 44.33\\
2.86 & 10.15 & -13.01\\
\end{pmatrix}\\
\begin{pmatrix}
0. & 56.523 & 2.689\\
118.59 & 0. & 217.204\\
0.662 & 25.78 & 0.\\
\end{pmatrix}\\
\begin{pmatrix}
0. & 16.842 & 23.025\\
5703.653 & 0. & 408.565\\
22.894 & 30.518 & 0.\\
\end{pmatrix}\\
\begin{pmatrix}
0. & 130.055 & 2.504\\
357.462 & 0. & 576.027\\
0.774 & 55.727 & 0.\\
\end{pmatrix}
\\ \end{align*}
\caption{Ion Channel, selected experiment: Learned prior transition rates with internal standard deviation. Order from top to bottom: Koehs result, our result trained on 1st second, our result trained on 2nd second and our result trained on full dataset.}
\end{figure}



\begin{table}
\centering
\caption{Ion Channel, all experiment: NLL and KL on various test sets with mean and standard deviation.}
\begin{tabular}{rcc}
\toprule
                                Experiment &                     KL &                          NLL \\
\midrule
      Koehs Result, Prediction after Train &                      - &                            - \\
         Koehs Result, Prediction on Train &                      - &                            - \\
\midrule
Train on $1$st sec, Prediction after Train & $18.89487 \pm 0.45741$ &  $-2,698.67572 \pm 12.25620$ \\
   Train on $1$st sec, Prediction on Train &  $3.97099 \pm 0.28104$ &   $-2,703.92097 \pm 2.81778$ \\
                     Train on $1$st second &  $4.57278 \pm 0.41961$ & $-1,924.61675 \pm 277.93282$ \\
                     Train on $2$nd second & $10.90745 \pm 8.74437$ &  $-2,559.11558 \pm 35.52976$ \\
                     Train on full dataset &  $7.11452 \pm 0.37399$ &   $-2,684.78082 \pm 8.28680$ \\
\bottomrule
\end{tabular}
\end{table}



\begin{table}
\centering
\caption{Ion Channel, all experiment: RMSE on test set and at observations in various prediction sets.}
\begin{tabular}{rccccccccc}
\toprule
                                Experiment &               RMSE test & \multicolumn{8}{c}{RMSE prediction} \\
                                           &                 &                       1 &                       2 &                       3 &                       4 &                       5 &                      10 &                      50 &                      90 \\
\midrule
      Koehs Result, Prediction after Train &                       - &              $\num{9.31e-16}$ &              $\num{3.11e-13}$ &              $\num{3.93e-13}$ &              $\num{1.61e-13}$ &              $\num{2.68e-13}$ &              $\num{3.58e-13}$ &              $\num{6.56e-12}$ &              $\num{6.62e-12}$ \\
         Koehs Result, Prediction on Train &                       - &              $\num{2.61e-13}$ &              $\num{2.26e-13}$ &              $\num{2.26e-13}$ &              $\num{2.58e-13}$ &              $\num{2.89e-13}$ &              $\num{2.75e-13}$ &              $\num{1.90e-12}$ &              $\num{2.47e-12}$ \\
\midrule
Train on $1$st sec, Prediction after Train & $\num{6.65e-13} \pm \num{1.31e-13}$ & $\num{2.91e-13} \pm \num{8.96e-15}$ & $\num{6.30e-14} \pm \num{8.96e-15}$ & $\num{3.75e-13} \pm \num{8.96e-15}$ & $\num{4.57e-13} \pm \num{8.96e-15}$ & $\num{2.25e-13} \pm \num{8.96e-15}$ & $\num{2.63e-13} \pm \num{8.96e-15}$ & $\num{6.69e-12} \pm \num{8.96e-15}$ & $\num{6.31e-12} \pm \num{8.96e-15}$ \\
   Train on $1$st sec, Prediction on Train & $\num{4.70e-13} \pm \num{5.88e-14}$ & $\num{4.07e-13} \pm \num{2.95e-13}$ & $\num{3.68e-13} \pm \num{2.96e-13}$ & $\num{3.48e-13} \pm \num{2.76e-13}$ & $\num{3.59e-13} \pm \num{2.51e-13}$ & $\num{3.76e-13} \pm \num{2.44e-13}$ & $\num{3.86e-13} \pm \num{2.20e-13}$ & $\num{1.82e-12} \pm \num{2.09e-13}$ & $\num{2.82e-12} \pm \num{1.16e-13}$ \\
                     Train on $1$st second & $\num{1.49e-12} \pm \num{7.33e-14}$ & $\num{2.33e-12} \pm \num{2.08e-13}$ & $\num{2.32e-12} \pm \num{2.13e-13}$ & $\num{2.32e-12} \pm \num{2.18e-13}$ & $\num{2.37e-12} \pm \num{2.36e-13}$ & $\num{2.48e-12} \pm \num{2.22e-13}$ & $\num{2.65e-12} \pm \num{2.18e-13}$ & $\num{2.76e-12} \pm \num{1.76e-13}$ & $\num{1.75e-12} \pm \num{1.56e-13}$ \\
                     Train on $2$nd second & $\num{1.54e-12} \pm \num{4.45e-13}$ & $\num{2.12e-12} \pm \num{2.34e-13}$ & $\num{2.12e-12} \pm \num{2.48e-13}$ & $\num{2.13e-12} \pm \num{2.92e-13}$ & $\num{2.14e-12} \pm \num{3.40e-13}$ & $\num{2.15e-12} \pm \num{3.58e-13}$ & $\num{2.28e-12} \pm \num{5.28e-13}$ & $\num{2.31e-12} \pm \num{3.25e-13}$ & $\num{2.70e-12} \pm \num{1.92e-13}$ \\
                     Train on full dataset & $\num{4.61e-13} \pm \num{2.03e-14}$ & $\num{3.08e-13} \pm \num{8.93e-15}$ & $\num{2.67e-13} \pm \num{4.96e-15}$ & $\num{2.90e-13} \pm \num{7.22e-16}$ & $\num{5.30e-13} \pm \num{1.71e-15}$ & $\num{1.01e-12} \pm \num{3.29e-15}$ & $\num{2.04e-12} \pm \num{5.58e-15}$ & $\num{2.61e-12} \pm \num{3.92e-13}$ & $\num{1.06e-12} \pm \num{9.61e-15}$ \\
\bottomrule
\end{tabular}
\end{table}



\begin{table}
\centering
\caption{Ion Channel, all experiments: Equilibrium distribution with mean and standard deviation.}
\begin{tabular}{rc}
\toprule
                                Experiment &                                                           Equilibrium \\
\midrule
      Koehs Result, Prediction after Train &                                     [$0.17961$, $0.14987$, $0.67052$] \\
         Koehs Result, Prediction on Train &                                     [$0.17961$, $0.14987$, $0.67052$] \\
\midrule
   Train on $1$st sec, Prediction on Train &  [$0.17947 \pm 0.0048$, $0.08899 \pm 0.00546$, $0.73154 \pm 0.00192$] \\
Train on $1$st sec, Prediction after Train & [$0.17882 \pm 0.00483$, $0.08897 \pm 0.00551$, $0.73222 \pm 0.00167$] \\
                     Train on $1$st second & [$0.17952 \pm 0.00477$, $0.08909 \pm 0.00545$, $0.73138 \pm 0.00219$] \\
                                2nd second &  [$0.33599 \pm 0.2844$, $0.10276 \pm 0.07074$, $0.56124 \pm 0.24105$] \\
                     Train on full dataset & [$0.19206 \pm 0.00478$, $0.08018 \pm 0.00856$, $0.72776 \pm 0.00649$] \\
\bottomrule
\end{tabular}
\end{table}
\begin{figure}
\centering
\begin{align*}
\begin{pmatrix}
-30.16 & 18.58 & 11.58\\
23.35 & -67.68 & 44.33\\
2.86 & 10.15 & -13.01\\
\end{pmatrix}\\
& \begin{pmatrix}
0. & 57.192 & 3.536\\
117.324 & 0. & 212.426\\
0.724 & 25.911 & 0.\\
\end{pmatrix}
&\pm
\begin{pmatrix}
0. & 2.331 & 1.256\\
13.489 & 0. & 10.795\\
0.124 & 0.254 & 0.\\
\end{pmatrix}\\
& \begin{pmatrix}
0. & 92.519 & 86.688\\
1287.002 & 0. & 184.682\\
13.97 & 40.143 & 0.\\
\end{pmatrix}
&\pm
\begin{pmatrix}
0. & 97.198 & 119.861\\
2208.612 & 0. & 119.488\\
11.187 & 14.213 & 0.\\
\end{pmatrix}\\
& \begin{pmatrix}
0. & 125.545 & 2.645\\
304.044 & 0. & 520.222\\
0.789 & 56.796 & 0.\\
\end{pmatrix}
&\pm
\begin{pmatrix}
0. & 2.414 & 0.402\\
39.952 & 0. & 39.652\\
0.088 & 2.638 & 0.\\
\end{pmatrix}
\\ \end{align*}
\caption{Ion Channel, all experiment: Learned prior transition rates with mean and standard deviation. Order from top to bottom: Koehs result, our result trained on 1st second, our result trained on 2nd second and our result trained on full dataset.}
\end{figure}



==> tables_and_matrices_jan_23.tex <==
\section{All Tables}

\subsection{Discrete Flashing Ratchet}
\begin{table}
\centering
\caption{Discrete Flashing Ratchet, selected experiments: learned prior parameters with internal standard deviation.}
\begin{tabular}{rccccc}
\toprule
            Experiment &                 KL &               NLL &               $V$ &               $r$ &               $b$ \\
\midrule
          Ground Truth &      - &     - &   $1.000  $ &   $1.000  $ &   $1.000  $ \\
\midrule
   Irregular Grid Data & $20.239 \pm 6.358$ & $0.196 \pm 0.766$ & $1.061 \pm 0.020$ & $1.166 \pm 0.015$ & $1.141 \pm 0.019$ \\
      Shared Grid Data & $19.154 \pm 7.720$ & $0.136 \pm 0.659$ & $0.966 \pm 0.017$ & $1.166 \pm 0.016$ & $1.172 \pm 0.012$ \\
     Regular Grid Data & $22.274 \pm 5.808$ & $0.175 \pm 0.701$ & $0.985 \pm 0.052$ & $1.367 \pm 0.043$ & $1.388 \pm 0.040$ \\
Masked Posterior Rates & $16.762 \pm 3.901$ & $0.237 \pm 0.828$ & $1.011 \pm 0.022$ & $1.144 \pm 0.018$ & $1.164 \pm 0.018$ \\
Non-parametrized Prior & $18.087 \pm 4.302$ & $0.218 \pm 0.838$ &     - &     - &     - \\
\bottomrule
\end{tabular}
\end{table}



\begin{figure}
\centering
\begin{align*}
\begin{pmatrix}
0. & 0.607 & 0.368 & 1. & 0. & 0.\\
1.649 & 0. & 0.607 & 0. & 1. & 0.\\
2.718 & 1.649 & 0. & 0. & 0. & 1.\\
1. & 0. & 0. & 0. & 1. & 1.\\
0. & 1. & 0. & 1. & 0. & 1.\\
0. & 0. & 1. & 1. & 1. & 0.\\
\end{pmatrix}\\
& \begin{pmatrix}
0. & 0.710 & 0.448 & 1.17 & 0.044 & 0.038\\
1.878 & 0. & 0.771 & 0.073 & 1.119 & 0.032\\
3.105 & 1.844 & 0. & 0.115 & 0.065 & 1.264\\
1.349 & 0.071 & 0.047 & 0. & 1.02 & 1.029\\
0.095 & 1.083 & 0.042 & 1.124 & 0. & 1.098\\
0.123 & 0.074 & 0.969 & 1.367 & 1.157 & 0.\\
\end{pmatrix}
&\pm
\begin{pmatrix}
0. & 0.010 & 0.006 & 0.020 & 0.001 & 0.001\\
0.032 & 0. & 0.013 & 0.002 & 0.016 & 0.001\\
0.072 & 0.048 & 0. & 0.003 & 0.002 & 0.024\\
0.018 & 0.002 & 0.002 & 0. & 0.014 & 0.016\\
0.002 & 0.017 & 0.001 & 0.019 & 0. & 0.018\\
0.003 & 0.002 & 0.018 & 0.02 & 0.015 & 0.\\
\end{pmatrix}
\\ \end{align*}
\caption{Discrete flashing ratchet, selected experiment with no explicit prior. Top: true transition rates. Bottom: Learned prior transition rates with internal standard deviation.}
\end{figure}



\begin{table}
\centering
\caption{Discrete Flashing Ratchet, selected experiments: Accuracy on test set and at observations in prediction set.}
\begin{tabular}{rcccc}
\toprule
            Experiment &          Accuracy & \multicolumn{3}{c}{Accuracy prediction} \\
                       &           &                   1 &                 5 &                10 \\
\midrule
   Irregular Grid Data & $0.934 \pm 0.058$ &   $0.670 \pm 0.000$ & $0.501 \pm 0.002$ & $0.402 \pm 0.006$ \\
      Shared Grid Data & $0.958 \pm 0.045$ &   $0.710 \pm 0.000$ & $0.520 \pm 0.001$ & $0.340 \pm 0.004$ \\
     Regular Grid Data & $0.933 \pm 0.053$ &   $0.720 \pm 0.000$ & $0.468 \pm 0.010$ & $0.380 \pm 0.007$ \\
Masked Posterior Rates & $0.916 \pm 0.076$ &   $0.670 \pm 0.000$ & $0.500 \pm 0.001$ & $0.396 \pm 0.011$ \\
Non-parametrized Prior & $0.930 \pm 0.071$ &   $0.670 \pm 0.000$ & $0.505 \pm 0.006$ & $0.410 \pm 0.002$ \\
\bottomrule
\end{tabular}
\end{table}




\begin{table}
\centering
\caption{Discrete Flashing Ratchet, all experiments: learned prior parameters with mean and standard deviation of 5 runs.}
\begin{tabular}{rccccc}
\toprule
            Experiment &                 KL &               NLL &               $V$ &               $r$ &               $b$ \\
\midrule
          Ground Truth &                  - &                 - &           $1.000$ &           $1.000$ &           $1.000$ \\
\midrule
   Irregular Grid Data & $19.988 \pm 1.148$ & $0.214 \pm 0.012$ & $0.983 \pm 0.047$ & $1.106 \pm 0.056$ & $1.127 \pm 0.039$ \\
      Shared Grid Data & $18.743 \pm 0.460$ & $0.144 \pm 0.006$ & $0.954 \pm 0.026$ & $1.180 \pm 0.036$ & $1.137 \pm 0.057$ \\
     Regular Grid Data & $21.755 \pm 0.728$ & $0.181 \pm 0.018$ & $0.995 \pm 0.051$ & $1.371 \pm 0.048$ & $1.361 \pm 0.048$ \\
Masked Posterior Rates & $17.090 \pm 0.376$ & $0.221 \pm 0.014$ & $0.990 \pm 0.018$ & $1.176 \pm 0.042$ & $1.163 \pm 0.032$ \\
Non-parametrized Prior & $17.630 \pm 0.600$ & $0.216 \pm 0.008$ &                 - &                 - &                 - \\
\bottomrule
\end{tabular}
\end{table}



\begin{figure}
\centering
\begin{align*}
\begin{pmatrix}
0. & 0.607 & 0.368 & 1. & 0. & 0.\\
1.649 & 0. & 0.607 & 0. & 1. & 0.\\
2.718 & 1.649 & 0. & 0. & 0. & 1.\\
1. & 0. & 0. & 0. & 1. & 1.\\
0. & 1. & 0. & 1. & 0. & 1.\\
0. & 0. & 1. & 1. & 1. & 0.\\
\end{pmatrix}\\
& \begin{pmatrix}
0. & 0.672 & 0.433 & 1.118 & 0.048 & 0.042\\
1.769 & 0. & 0.714 & 0.101 & 1.121 & 0.048\\
2.872 & 1.738 & 0. & 0.114 & 0.079 & 1.150\\
1.320 & 0.069 & 0.050 & 0. & 1.054 & 1.042\\
0.103 & 1.091 & 0.045 & 1.147 & 0. & 1.155\\
0.134 & 0.066 & 0.903 & 1.277 & 1.211 & 0.\\
\end{pmatrix}
&\pm
\begin{pmatrix}
0. & 0.038 & 0.013 & 0.030 & 0.002 & 0.002\\
0.093 & 0. & 0.034 & 0.016 & 0.043 & 0.01\\
0.167 & 0.085 & 0. & 0.015 & 0.015 & 0.12\\
0.025 & 0.006 & 0.004 & 0. & 0.024 & 0.065\\
0.011 & 0.029 & 0.003 & 0.056 & 0. & 0.087\\
0.015 & 0.006 & 0.078 & 0.116 & 0.051 & 0.\\
\end{pmatrix}
\\ \end{align*}
\caption{Discrete flashing ratchet, all experiments. Top: true transition rates. Bottom: Learned prior transition rates with mean and standard deviation of 5 runs.}
\end{figure}



\begin{table}
\centering
\caption{Discrete Flashing Ratchet, all experiments: Accuracy on test set and at observations in prediction set with mean and standard deviation for 5 runs}
\begin{tabular}{rcccc}
\toprule
            Experiment &          Accuracy & \multicolumn{3}{c}{Accuracy prediction} \\
                       &           &                   1 &                 5 &                10 \\
\midrule
   Irregular Grid Data & $0.928 \pm 0.004$ &   $0.648 \pm 0.015$ & $0.496 \pm 0.011$ & $0.396 \pm 0.005$ \\
      Shared Grid Data & $0.951 \pm 0.005$ &   $0.710 \pm 0.016$ & $0.509 \pm 0.022$ & $0.331 \pm 0.013$ \\
     Regular Grid Data & $0.932 \pm 0.010$ &   $0.714 \pm 0.011$ & $0.468 \pm 0.015$ & $0.370 \pm 0.010$ \\
Masked Posterior Rates & $0.924 \pm 0.007$ &   $0.661 \pm 0.015$ & $0.496 \pm 0.005$ & $0.397 \pm 0.009$ \\
Non-parametrized Prior & $0.926 \pm 0.003$ &   $0.648 \pm 0.019$ & $0.499 \pm 0.019$ & $0.396 \pm 0.008$ \\
\bottomrule
\end{tabular}
\end{table}

\subsection{Lotka-Volterra}
\begin{table}
\centering
\caption{Lotka-Volterra, selected experiments: KL and NLL.}
\begin{tabular}{rcc}
\toprule
                          Experiment &                KL &                NLL \\
\midrule
                        Ground Truth &     - &      - \\
  Oppers Results, Mean as Prediction &     - &      - \\
Oppers Results, Prior for Prediction &     - &      - \\
\midrule
                 Irregular Grid Data & $31.37 \pm 27.36$ & $167.93 \pm 20.29$ \\
                    Shared Grid Data & $31.28 \pm 15.72$ &  $153.22 \pm 8.80$ \\
                   Regular Grid Data &  $25.62 \pm 7.07$ &  $158.84 \pm 9.25$ \\
             Opper Data, our Results &   $97.65  $ &   $-10.58  $ \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}
\centering
\caption{Lotka-Volterra, selected experiments: learned prior parameters with internal standard deviation.}
\begin{tabular}{rcccc}
\toprule
                          Experiment &                $\alpha$ &                 $\beta$ &                $\delta$ &                $\gamma$ \\
\midrule
                        Ground Truth &      $\num{5.00e-04}  $ &      $\num{1.00e-04}  $ &      $\num{1.00e-04}  $ &      $\num{5.00e-04}  $ \\
  Oppers Results, Mean as Prediction &      $\num{1.35e-03}  $ &      $\num{2.32e-04}  $ &      $\num{1.78e-04}  $ &      $\num{1.57e-03}  $ \\
Oppers Results, Prior for Prediction &      $\num{1.35e-03}  $ &      $\num{2.32e-04}  $ &      $\num{1.78e-04}  $ &      $\num{1.57e-03}  $ \\
\midrule
                 Irregular Grid Data & $\num{4.48e-04} \pm \num{2.59e-05}$ & $\num{9.98e-05} \pm \num{7.74e-06}$ & $\num{7.56e-05} \pm \num{7.96e-06}$ & $\num{3.55e-04} \pm \num{2.23e-05}$ \\
                    Shared Grid Data & $\num{5.52e-04} \pm \num{1.03e-05}$ & $\num{1.13e-04} \pm \num{3.88e-06}$ & $\num{9.83e-05} \pm \num{4.46e-06}$ & $\num{4.93e-04} \pm \num{8.54e-06}$ \\
                   Regular Grid Data & $\num{4.37e-04} \pm \num{1.42e-05}$ & $\num{9.51e-05} \pm \num{5.67e-06}$ & $\num{9.83e-05} \pm \num{7.13e-06}$ & $\num{4.91e-04} \pm \num{1.04e-05}$ \\
             Opper Data, our Results & $\num{2.53e-04} \pm \num{1.01e-05}$ & $\num{6.42e-05} \pm \num{4.35e-06}$ & $\num{1.03e-04} \pm \num{6.43e-06}$ & $\num{4.15e-04} \pm \num{1.67e-05}$ \\
\bottomrule
\end{tabular}
\end{table}



\begin{table}
\centering
\caption{Lotka-Volterra, selected experiments: Accuracy on test set and at observations in prediction set. Prediction set for opper contains non-noisy observations of trajectory after the test set.}
\begin{tabular}{rcccc}
\toprule
                          Experiment &         RMSE Test & \multicolumn{3}{c}{RMSE Prediction} \\
                                     &           &                 1 &                  5 &                 10 \\
\midrule
  Oppers Results, Mean as Prediction &   $2.672  $ &   $2.549  $ &    $6.524  $ &    $8.024  $ \\
Oppers Results, Prior for Prediction &   $2.672  $ &   $3.000  $ &    $9.487  $ &   $11.402  $ \\
\midrule
                 Irregular Grid Data & $1.915 \pm 0.460$ & $2.935 \pm 0.588$ &  $3.272 \pm 0.986$ &  $3.389 \pm 1.686$ \\
                    Shared Grid Data & $1.627 \pm 0.162$ & $2.267 \pm 0.440$ &  $2.700 \pm 0.467$ &  $3.041 \pm 0.577$ \\
                   Regular Grid Data & $1.727 \pm 0.191$ & $1.667 \pm 0.011$ &  $2.198 \pm 0.295$ &  $2.518 \pm 0.354$ \\
             Opper Data, our Results &   $2.070  $ & $6.000 \pm 0.000$ & $5.600 \pm 11.530$ & $6.730 \pm 17.437$ \\
\bottomrule
\end{tabular}
\end{table}



\begin{table}
\centering
\caption{Lotka-Volterra, all experiments:KL and NLL.}
\begin{tabular}{rcc}
\toprule
                          Experiment &                    KL &                 NLL \\
\midrule
                        Ground Truth &                     - &                   - \\
  Oppers Results, Mean as Prediction &                     - &                   - \\
Oppers Results, Prior for Prediction &                     - &                   - \\
\midrule
                 Irregular Grid Data &    $30.615 \pm 2.253$ & $165.979 \pm 1.765$ \\
                    Shared Grid Data &    $35.904 \pm 4.407$ & $155.338 \pm 2.180$ \\
                   Regular Grid Data &    $28.054 \pm 5.020$ & $162.607 \pm 3.933$ \\
             Opper Data, our Results & $192.218 \pm 114.124$ & $12.556 \pm 23.797$ \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}
\centering
\caption{Lotka-Volterra, all experiments: learned prior parameters with mean and standard deviation of 5 runs.}
\begin{tabular}{rcccc}
\toprule
                          Experiment &                  $\alpha$ &                   $\beta$ &                  $\delta$ &                  $\gamma$ \\
\midrule
                        Ground Truth &               $\num{5.000e-04}$ &               $\num{1.000e-04}$ &               $\num{1.000e-04}$ &               $\num{5.000e-04}$ \\
  Oppers Results, Mean as Prediction &               $\num{1.350e-03}$ &               $\num{2.320e-04}$ &               $\num{1.780e-04}$ &               $\num{1.570e-03}$ \\
Oppers Results, Prior for Prediction &               $\num{1.350e-03}$ &               $\num{2.320e-04}$ &               $\num{1.780e-04}$ &               $\num{1.570e-03}$ \\
\midrule
                 Irregular Grid Data & $\num{4.269e-04} \pm \num{6.224e-05}$ & $\num{9.414e-05} \pm \num{7.350e-06}$ & $\num{8.303e-05} \pm \num{8.690e-06}$ & $\num{4.060e-04} \pm \num{4.262e-05}$ \\
                    Shared Grid Data & $\num{5.495e-04} \pm \num{5.718e-05}$ & $\num{1.103e-04} \pm \num{7.393e-06}$ & $\num{1.003e-04} \pm \num{5.519e-06}$ & $\num{4.939e-04} \pm \num{4.348e-05}$ \\
                   Regular Grid Data & $\num{4.511e-04} \pm \num{6.351e-05}$ & $\num{9.749e-05} \pm \num{2.695e-06}$ & $\num{8.923e-05} \pm \num{8.425e-06}$ & $\num{4.309e-04} \pm \num{5.627e-05}$ \\
             Opper Data, our Results & $\num{2.088e-04} \pm \num{6.485e-05}$ & $\num{6.722e-05} \pm \num{6.028e-06}$ & $\num{1.052e-04} \pm \num{3.237e-05}$ & $\num{9.262e-04} \pm \num{8.149e-04}$ \\
\bottomrule
\end{tabular}
\end{table}



\begin{table}
\centering
\caption{Lotka-Volterra, all experiments: RMSE on test set and at observations in prediction set. Prediction set for opper contains non-noisy observations of trajectory after the test set.}
\begin{tabular}{rcccc}
\toprule
                          Experiment &         RMSE Test & \multicolumn{3}{c}{RMSE Prediction} \\
                                     &           &                 1 &                 5 &                 10 \\
\midrule
  Oppers Results, Mean as Prediction &   $2.672  $ &   $2.549  $ &   $6.524  $ &    $8.024  $ \\
Oppers Results, Prior for Prediction &   $2.672  $ &   $3.000  $ &   $9.487  $ &   $11.402  $ \\
\midrule
                 Irregular Grid Data & $1.868 \pm 0.036$ & $2.666 \pm 0.171$ & $3.127 \pm 0.105$ &  $3.269 \pm 0.110$ \\
                    Shared Grid Data & $1.665 \pm 0.036$ & $2.325 \pm 0.076$ & $2.810 \pm 0.178$ &  $3.120 \pm 0.185$ \\
                   Regular Grid Data & $1.801 \pm 0.075$ & $1.752 \pm 0.141$ & $2.346 \pm 0.184$ &  $2.684 \pm 0.234$ \\
             Opper Data, our Results & $2.017 \pm 0.043$ & $5.692 \pm 2.656$ & $9.192 \pm 3.618$ & $10.582 \pm 4.294$ \\
\bottomrule
\end{tabular}
\end{table}



\subsection{Brownian Dynamics / Toy Protein Folding}



\begin{table}
\centering
\caption{Toy Protein Folding, selected experiment: NLL and KL on test set}
\begin{tabular}{rcc}
\toprule
Experiment &                KL &                   NLL \\
\midrule
      Ours & $1.593 \pm 2.161$ & $542.374 \pm 271.273$ \\
\bottomrule
\end{tabular}
\end{table}




\begin{table}
\centering
\caption{Toy Protein Folding, selected experiment: RMSE on test set and at observations in prediction set.}
\begin{tabular}{rcccc}
\toprule
Experiment &         RMSE Test & \multicolumn{3}{c}{RMSE Prediction} \\
           &           &                 1 &                25 &                50 \\
\midrule
      Ours & $2.021 \pm 1.370$ & $1.951 \pm 0.000$ & $1.914 \pm 0.003$ & $1.911 \pm 0.006$ \\
\bottomrule
\end{tabular}
\end{table}




\begin{table}
\centering
\caption{Toy Protein Folding, selected experiment: Equilibrium distribution.}
\begin{tabular}{rcc}
\toprule
Experiment & \multicolumn{2}{c}{Equilibrium Distribution} \\
           &            Low STD State &        High STD State \\
\midrule
  VAMPnets &        $0.72727  $ &     $0.27273  $ \\
\midrule
      Ours &    $0.73169 \pm 0.14493$ & $0.26831 \pm 0.14493$ \\
\bottomrule
\end{tabular}
\end{table}



\begin{figure}
\centering
\begin{align*}
\begin{pmatrix}
0. & 0.029\\
0.089 & 0.\\
\end{pmatrix}
\pm
\begin{pmatrix}
0. & 0.025\\
0.051 & 0.\\
\end{pmatrix}
\\ \end{align*}
\caption{Toy Protein Folding, selected experiment: Learned prior transition rates with internal standard deviation.}
\end{figure}



\begin{table}
\centering
\caption{Toy Protein Folding, all experiments: NLL and KL on test set with mean and standard deviation of 5 runs.}
\begin{tabular}{rcc}
\toprule
Experiment &                KL &                 NLL \\
\midrule
      Ours & $1.405 \pm 0.173$ & $542.658 \pm 0.513$ \\
\bottomrule
\end{tabular}
\end{table}




\begin{table}
\centering
\caption{Toy Protein Folding, all experiment: RMSE on test set and at observations in prediction set with mean and standard deviation of 5 runs.}
\begin{tabular}{rcccc}
\toprule
Experiment &         RMSE Test & \multicolumn{3}{c}{RMSE Prediction} \\
           &           &                 1 &                25 &                50 \\
\midrule
      Ours & $2.021 \pm 0.001$ & $1.950 \pm 0.002$ & $1.913 \pm 0.001$ & $1.910 \pm 0.002$ \\
\bottomrule
\end{tabular}
\end{table}




\begin{table}
\centering
\caption{Toy Protein Folding, all experiments: Equilibrium distribution with mean and standard deviation of 5 runs.}
\begin{tabular}{rcc}
\toprule
Experiment & \multicolumn{2}{c}{Equilibrium Distribution} \\
           &            Low STD State &       High STD State \\
\midrule
  VAMPnets &                $0.72727$ &            $0.27273$ \\
\midrule
      Ours &     $0.74129 \pm 0.0211$ & $0.25871 \pm 0.0211$ \\
\bottomrule
\end{tabular}
\end{table}



\begin{figure}
\centering
\begin{align*}
\begin{pmatrix}
0. & 0.028\\
0.085 & 0.\\
\end{pmatrix}
\pm
\begin{pmatrix}
0. & 0.007\\
0.011 & 0.\\
\end{pmatrix}
\\ \end{align*}
\caption{Toy Protein Folding, all experiments: Learned transition rates with mean and standard deviation of 5 runs.}
\end{figure}


\subsection{Alanine Dipeptide}



\begin{table}
\centering
\caption{Alanine Dipeptide, selected experiment: NLL and KL on test set.}
\begin{tabular}{rcc}
\toprule
            Experiment &                    KL &                        NLL \\
\midrule
              VAMPnets &         - &              - \\
\midrule
$2$ States, Top-Bottom & $0.00010 \pm 0.00026$ & $579.48688 \pm 2028.74731$ \\
$2$ States, Left-Right & $0.00054 \pm 0.00410$ &  $262.01837 \pm 828.91785$ \\
            $3$ States & $1.53461 \pm 1.64815$ &  $101.69016 \pm 372.33661$ \\
            $6$ States & $9.55489 \pm 3.65148$ &   $-81.97252 \pm 76.50587$ \\
\bottomrule
\end{tabular}
\end{table}



\begin{table}
\centering
\caption{Alanine Dipeptide, selected experiment: RMSE on test set and at observations in prediction set.}
\begin{tabular}{rccccc}
\toprule
            Experiment &         RMSE Test & \multicolumn{4}{c}{RMSE Prediction} \\
                       &           &                 5 &                10 &                20 &                50 \\
\midrule
$2$ States, Left-Right & $0.981 \pm 0.273$ & $0.945 \pm 0.000$ & $0.962 \pm 0.000$ & $0.957 \pm 0.000$ & $0.928 \pm 0.000$ \\
$2$ States, Top-Bottom & $0.934 \pm 0.354$ & $0.785 \pm 0.000$ & $0.813 \pm 0.000$ & $0.843 \pm 0.000$ & $0.898 \pm 0.000$ \\
            $3$ States & $0.655 \pm 0.134$ & $0.650 \pm 0.000$ & $0.709 \pm 0.000$ & $0.752 \pm 0.000$ & $0.869 \pm 0.000$ \\
            $6$ States & $0.613 \pm 0.126$ & $0.643 \pm 0.000$ & $0.696 \pm 0.006$ & $0.783 \pm 0.057$ & $0.903 \pm 0.137$ \\
\bottomrule
\end{tabular}
\end{table}




\begin{table}
\centering
\caption{Alanine Dipeptide, selected experiment: Equilibrium distribution.}
\begin{tabular}{rcccccc}
\toprule
            Experiment & \multicolumn{6}{c}{Equilibrium Distribution} \\
                       &                  State 1 &           State 2 &           State 3 &           State 4 &           State 5 &           State 6 \\
\midrule
              VAMPnets &            $0.3  $ &   $0.238  $ &   $0.194  $ &   $0.145  $ &   $0.109  $ &   $0.014  $ \\
\midrule
$2$ States, Left-Right &        $0.713 \pm 0.005$ & $0.287 \pm 0.005$ &    - &    - &    - &    - \\
$2$ States, Top-Bottom &        $0.458 \pm 0.376$ & $0.542 \pm 0.376$ &    - &    - &    - &    - \\
            $3$ States &        $0.687 \pm 0.014$ & $0.199 \pm 0.011$ & $0.113 \pm 0.012$ &    - &    - &    - \\
            $6$ States &        $0.298 \pm 0.021$ &  $0.31 \pm 0.018$ & $0.234 \pm 0.028$ & $0.097 \pm 0.007$ & $0.053 \pm 0.017$ & $0.008 \pm 0.002$ \\
\bottomrule
\end{tabular}
\end{table}



\begin{figure}
\centering
\begin{align*}
& \begin{pmatrix}
0. & 0.00000\\
0.00000 & 0.\\
\end{pmatrix}
&\pm
\begin{pmatrix}
0. & 0.00000\\
0.00000 & 0.\\
\end{pmatrix}\\
& \begin{pmatrix}
0. & 0.00000\\
0.00000 & 0.\\
\end{pmatrix}
&\pm
\begin{pmatrix}
0. & 0.00000\\
0.00000 & 0.\\
\end{pmatrix}\\
& \begin{pmatrix}
0. & 0.00289 & 0.00087\\
0.00971 & 0. & 0.00027\\
0.00572 & 0.00003 & 0.\\
\end{pmatrix}
&\pm
\begin{pmatrix}
0. & 0.00019 & 0.00009\\
0.00024 & 0. & 0.00004\\
0.00043 & 0.00001 & 0.\\
\end{pmatrix}\\
& \begin{pmatrix}
0. & 0.05294 & 0.00019 & 0.00793 & 0.00006 & 0.00002\\
0.04728 & 0. & 0.00005 & 0.01198 & 0.00004 & 0.00001\\
0.00028 & 0.00013 & 0. & 0.01678 & 0.00002 & 0.00004\\
0.03553 & 0.0269 & 0.04051 & 0. & 0.00025 & 0.00001\\
0.00017 & 0.00022 & 0.00032 & 0.00020 & 0. & 0.00301\\
0.00115 & 0.00175 & 0.00046 & 0.00065 & 0.0187 & 0.\\
\end{pmatrix}
&\pm
\begin{pmatrix}
0. & 0.00379 & 0.00006 & 0.00088 & 0.00003 & 0.00001\\
0.00321 & 0. & 0.00003 & 0.00090 & 0.00002 & 0.00001\\
0.00009 & 0.00005 & 0. & 0.00144 & 0.00001 & 0.00002\\
0.00308 & 0.00270 & 0.00436 & 0. & 0.00011 & 0.00001\\
0.00006 & 0.00011 & 0.00022 & 0.00015 & 0. & 0.00108\\
0.00064 & 0.00075 & 0.00022 & 0.00037 & 0.00754 & 0.\\
\end{pmatrix}
\\ \end{align*}
\caption{Alanine Dipeptide, selected experiment: Learned prior transition rates with internal standard deviation. Order: 2 states top-bottom, 2 states left-right, 3 states, 6 states.}
\end{figure}



\begin{table}
\centering
\caption{Alanine Dipeptide, selected experiment: Absolute Values of Eigenvalues of Q-Matrix.}
\begin{tabular}{rcccccc}
\toprule
            Experiment & \multicolumn{6}{c}{Absolute Eigenvalues} \\
                       &          $\lambda_0$ &         $\lambda_1$ &         $\lambda_2$ &         $\lambda_3$ &         $\lambda_4$ &         $\lambda_5$ \\
\midrule
$2$ States, Top-Bottom &        $0.0 \pm 0.0$ &       $0.0 \pm 0.0$ &      - &      - &      - &      - \\
$2$ States, Left-Right &        $0.0 \pm 0.0$ &       $0.0 \pm 0.0$ &      - &      - &      - &      - \\
            $3$ States &        $0.0 \pm 0.0$ & $0.0064 \pm 0.0004$ & $0.0131 \pm 0.0003$ &      - &      - &      - \\
            $6$ States &        $0.0 \pm 0.0$ & $0.0014 \pm 0.0004$ & $0.0145 \pm 0.0009$ & $0.0254 \pm 0.0079$ & $0.1112 \pm 0.0051$ & $0.1152 \pm 0.0057$ \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}
\centering
\caption{Alanine Dipeptide, selected experiment: Relaxation Times.}
\begin{tabular}{rccccc}
\toprule
            Experiment & \multicolumn{5}{c}{Ordered Relaxation Times} \\
                       \\
\midrule
$2$ States, Top-Bottom &    $1288418.75 \pm 777470.25$ &         - &        - &       - &          - \\
$2$ States, Left-Right & $773440.9375 \pm 256286.9531$ &         - &        - &       - &          - \\
            $3$ States &          $76.1845 \pm 1.9796$ & $158.1308 \pm 10.4805$ &        - &       - &          - \\
            $6$ States &           $8.7064 \pm 0.4275$ &    $9.0174 \pm 0.4186$ & $42.8364 \pm 11.8488$ & $69.0118 \pm 4.3018$ & $773.5579 \pm 205.0169$ \\
\bottomrule
\end{tabular}
\end{table}




\begin{figure}
\centering
\begin{align*}
& \begin{pmatrix}
0. & 788217.875\\
73984008. & 0.\\
\end{pmatrix}
&\pm
\begin{pmatrix}
0. & 263568.719\\
58886680. & 0.\\
\end{pmatrix}\\
& \begin{pmatrix}
0. & 27.566 & 291.316 & 106.63 & 13689.327 & 15830.701\\
32.37 & 0. & 287.816 & 102.67 & 13690.997 & 15832.566\\
131.240 & 133.18 & 0. & 63.555 & 13691.293 & 15825.118\\
72.025 & 73.828 & 188.313 & 0. & 13668.916 & 15810.806\\
897.66 & 894.216 & 1034.88 & 912.237 & 0. & 3968.429\\
787.110 & 783.166 & 935.371 & 806.551 & 2587.450 & 0.\\
\end{pmatrix}
&\pm
\begin{pmatrix}
0. & 2.387 & 26.618 & 6.218 & 4112.59 & 4143.375\\
2.76 & 0. & 26.342 & 5.890 & 4112.066 & 4142.836\\
11.292 & 11.033 & 0. & 5.459 & 4108.395 & 4141.139\\
7.91 & 7.714 & 24.109 & 0. & 4111.708 & 4142.651\\
222.806 & 222.997 & 234.733 & 226.489 & 0. & 1139.761\\
208.79 & 209.223 & 212.628 & 209.061 & 1088.398 & 0.\\
\end{pmatrix}
\\ \end{align*}
\caption{Alanine Dipeptide, selected experiments. Mean First-Passage Times for 2 states, separating left and right regions of Ramachandran plane, and 6 states}
\end{figure}



\begin{table}
\centering
\caption{Alanine Dipeptide, all experiment: nll_mean and KL on test set with mean and standard deviation of all runs.}
\begin{tabular}{rcc}
\toprule
            Experiment &                    KL &                       NLL \\
\midrule
              VAMPnets &                     - &                         - \\
\midrule
$2$ States, Left-Right & $0.00439 \pm 0.00545$ &  $224.48798 \pm 53.07599$ \\
$2$ States, Top-Bottom & $0.87299 \pm 0.88886$ & $463.37313 \pm 136.61439$ \\
            $3$ States & $1.53688 \pm 0.09337$ &   $81.94286 \pm 15.55570$ \\
            $6$ States & $6.06125 \pm 2.82497$ &  $-26.74495 \pm 38.78156$ \\
\bottomrule
\end{tabular}
\end{table}



\begin{table}
\centering
\caption{Alanine Dipeptide, all experiments: RMSE on test set and at observations in prediction with mean and standard deviation of all runs.}
\begin{tabular}{rccccc}
\toprule
            Experiment &         RMSE Test & \multicolumn{4}{c}{RMSE Prediction} \\
                       &           &                 5 &                10 &                20 &                50 \\
\midrule
$2$ States, Left-Right & $0.977 \pm 0.006$ & $0.947 \pm 0.003$ & $0.963 \pm 0.002$ & $0.960 \pm 0.004$ & $0.924 \pm 0.006$ \\
$2$ States, Top-Bottom & $0.849 \pm 0.113$ & $0.801 \pm 0.075$ & $0.840 \pm 0.072$ & $0.878 \pm 0.066$ & $0.960 \pm 0.059$ \\
            $3$ States & $0.663 \pm 0.009$ & $0.649 \pm 0.019$ & $0.714 \pm 0.024$ & $0.752 \pm 0.017$ & $0.859 \pm 0.010$ \\
            $6$ States & $0.652 \pm 0.052$ & $0.627 \pm 0.022$ & $0.689 \pm 0.019$ & $0.745 \pm 0.026$ & $0.874 \pm 0.023$ \\
\bottomrule
\end{tabular}
\end{table}




\begin{table}
\centering
\caption{Alanine Dipeptide, all experiments: Equilibrium distribution.}
\begin{tabular}{rcccccc}
\toprule
            Experiment & \multicolumn{6}{c}{Equilibrium Distribution} \\
                       &                  State 1 &           State 2 &           State 3 &           State 4 &           State 5 &           State 6 \\
\midrule
              VAMPnets &                    $0.3$ &           $0.238$ &           $0.194$ &           $0.145$ &           $0.109$ &           $0.014$ \\
\midrule
$2$ States, Left-Right &        $0.375 \pm 0.338$ & $0.625 \pm 0.338$ &    - &    - &    - &    - \\
$2$ States, Top-Bottom &        $0.628 \pm 0.127$ & $0.372 \pm 0.127$ &    - &    - &    - &    - \\
            $3$ States &        $0.716 \pm 0.019$ & $0.256 \pm 0.031$ & $0.028 \pm 0.043$ &    - &    - &    - \\
            $6$ States &        $0.279 \pm 0.141$ & $0.359 \pm 0.128$ & $0.189 \pm 0.048$ & $0.131 \pm 0.064$ & $0.033 \pm 0.015$ & $0.009 \pm 0.005$ \\
\bottomrule
\end{tabular}
\end{table}



\begin{figure}
\centering
\begin{align*}
& \begin{pmatrix}
\num{0.e+00} & \num{2.21e-03}\\
\num{5.32e-03} & \num{0.e+00}\\
\end{pmatrix}
&\pm
\begin{pmatrix}
\num{0.e+00} & \num{6.69e-05}\\
\num{1.44e-04} & \num{0.e+00}\\
\end{pmatrix}\\
& \begin{pmatrix}
\num{0.e+00} & \num{4.44e-05}\\
\num{1.65e-06} & \num{0.e+00}\\
\end{pmatrix}
&\pm
\begin{pmatrix}
\num{0.e+00} & \num{1.09e-05}\\
\num{5.97e-07} & \num{0.e+00}\\
\end{pmatrix}\\
& \begin{pmatrix}
\num{0.e+00} & \num{3.69e-03} & \num{1.78e-04}\\
\num{1.03e-02} & \num{0.e+00} & \num{5.58e-05}\\
\num{1.74e-03} & \num{1.93e-05} & \num{0.e+00}\\
\end{pmatrix}
&\pm
\begin{pmatrix}
\num{0.e+00} & \num{1.49e-04} & \num{3.67e-05}\\
\num{1.31e-04} & \num{0.e+00} & \num{1.59e-05}\\
\num{1.07e-04} & \num{7.13e-06} & \num{0.e+00}\\
\end{pmatrix}
\\ \end{align*}
\caption{Alanine Dipeptide, selected experiment: Learned prior transition rates with internal standard deviation. Order: 2 states top-bottom, 2 states left-right, 3 states, 6 states.}
\end{figure}



\begin{table}
\centering
\caption{Alanine Dipeptide, all experiments: Absolute Values of Eigenvalues of Q-Matrix.}
\begin{tabular}{rcccccc}
\toprule
            Experiment & \multicolumn{6}{c}{Absolute Eigenvalues} \\
                       &          $\lambda_0$ &         $\lambda_1$ &         $\lambda_2$ &         $\lambda_3$ &         $\lambda_4$ &         $\lambda_5$ \\
\midrule
$2$ States, Top-Bottom &        $0.0 \pm 0.0$ & $0.0075 \pm 0.0054$ &      - &      - &      - &      - \\
$2$ States, Left-Right &        $0.0 \pm 0.0$ &       $0.0 \pm 0.0$ &      - &      - &      - &      - \\
            $3$ States &        $0.0 \pm 0.0$ & $0.0019 \pm 0.0022$ & $0.0141 \pm 0.0006$ &      - &      - &      - \\
            $6$ States &        $0.0 \pm 0.0$ & $0.0014 \pm 0.0006$ & $0.0095 \pm 0.0054$ & $0.0241 \pm 0.0085$ & $0.0737 \pm 0.0297$ & $0.0963 \pm 0.0285$ \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}
\centering
\caption{Alanine Dipeptide, all experiments: Relaxation Times.}
\begin{tabular}{rccccc}
\toprule
            Experiment & \multicolumn{5}{c}{Ordered Relaxation Times} \\
                       \\
\midrule
$2$ States, Top-Bottom & $429532.8943 \pm 607324.0129$ &          - &        - &          - &          - \\
$2$ States, Left-Right & $392571.8364 \pm 380869.1011$ &          - &        - &          - &          - \\
            $3$ States &          $71.1794 \pm 3.2147$ & $1154.807 \pm 514.8208$ &        - &          - &          - \\
            $6$ States &          $11.8414 \pm 4.9935$ &   $19.0817 \pm 14.5228$ & $48.2127 \pm 14.9308$ & $193.7844 \pm 167.2905$ & $907.7719 \pm 360.4073$ \\
\bottomrule
\end{tabular}
\end{table}




\begin{figure}
\centering
\begin{align*}
& \begin{pmatrix}
0. & 400193.345\\
37163995.469 & 0.\\
\end{pmatrix}
&\pm
\begin{pmatrix}
0. & 388024.530\\
36820012.531 & 0.\\
\end{pmatrix}\\
& \begin{pmatrix}
0. & 57.203 & 337.123 & 151.514 & 38294.870 & 35744.848\\
116.271 & 0. & 343.747 & 159.255 & 38286.707 & 35735.011\\
222.819 & 140.524 & 0. & 52.488 & 38224.052 & 35703.214\\
177.333 & 94.889 & 194.027 & 0. & 38242.158 & 35703.750\\
1072.619 & 1033.431 & 1206.721 & 1053.016 & 0. & 21924.452\\
979.686 & 923.127 & 1073.344 & 949.977 & 17167.395 & 0.\\
\end{pmatrix}
&\pm
\begin{pmatrix}
0. & 43.832 & 51.481 & 66.219 & 34039.39 & 29482.429\\
136.144 & 0. & 38.216 & 39.269 & 34031.991 & 29465.01\\
130.628 & 32.433 & 0. & 9.939 & 34063.901 & 29490.88\\
132.485 & 31.007 & 41.495 & 0. & 34056.170 & 29483.342\\
409.675 & 378.924 & 373.268 & 381.570 & 0. & 32194.971\\
424.312 & 378.584 & 386.046 & 375.804 & 21969.287 & 0.\\
\end{pmatrix}
\\ \end{align*}
\caption{Alanine Dipeptide, all experiments. Mean First-Passage Times for 2 States, separating left and right region of Ramachandran plane, and 6 States.}
\end{figure}
\subsection{One-Dimensional, Two Mode Hybrid System}



\begin{table}
\centering
\caption{1D synthetic SSDE, selected experiment: NLL and KL on test set.}
\begin{tabular}{rcc}
\toprule
   Experiment &                 KL &                 NLL \\
\midrule
 Ground Truth &      - &       - \\
Koehs Results &      - &       - \\
\midrule
         Ours & $11.54202  $ & $168.45613  $ \\
\bottomrule
\end{tabular}
\end{table}



\begin{table}
\centering
\caption{1D synthetic SSDE, selected experiment: Equilibrium distribution.}
\begin{tabular}{rcc}
\toprule
   Experiment & \multicolumn{2}{c}{Equilibrium Distribution} \\
              &             Bottom State &            Top State \\
\midrule
 Ground Truth &            $0.5  $ &        $0.5  $ \\
Koehs Results &        $0.49606  $ &    $0.50394  $ \\
\midrule
         ours &     $0.5164 \pm 0.01192$ & $0.4836 \pm 0.01192$ \\
\bottomrule
\end{tabular}
\end{table}



\begin{figure}
\centering
\begin{align*}
& \begin{pmatrix}
-0.2 & 0.2\\
0.2 & -0.2\\
\end{pmatrix}
&\pm
\begin{pmatrix}
nan\\
\end{pmatrix}\\
& \begin{pmatrix}
-0.64 & 0.64\\
0.63 & -0.63\\
\end{pmatrix}
&\pm
\begin{pmatrix}
nan\\
\end{pmatrix}\\
& \begin{pmatrix}
0. & 0.208\\
0.222 & 0.\\
\end{pmatrix}
&\pm
\begin{pmatrix}
0. & 0.008\\
0.013 & 0.\\
\end{pmatrix}
\\ \end{align*}
\caption{1D synthetic SSDE, selected experiment:Learned prior transition rates with mean and standard deviation. Order from top to bottom: True transition rates, Koehs result, all of our runs and our runs with 1 outlier dropped. }
\end{figure}



\begin{table}
\centering
\caption{1D synthetic SSDE, all experiments: NLL and KL on test set with mean and standard deviation.}
\begin{tabular}{rcc}
\toprule
   Experiment &                      KL &                      NLL \\
\midrule
 Ground Truth &                       - &                        - \\
Koehs Results &                       - &                        - \\
\midrule
         Ours & $48.69639 \pm 48.86893$ & $155.64621 \pm 28.65718$ \\
\bottomrule
\end{tabular}
\end{table}



\begin{table}
\centering
\caption{1D synthetic SSDE, all experiments: Equilibrium distribution with mean and standard deviation.}
\begin{tabular}{rcc}
\toprule
   Experiment & \multicolumn{2}{c}{Equilibrium Distribution} \\
              &             Bottom State &             Top State \\
\midrule
 Ground Truth &                    $0.5$ &                 $0.5$ \\
Koehs Results &                $0.49606$ &             $0.50394$ \\
\midrule
         Ours &    $0.70377 \pm 0.16139$ & $0.29623 \pm 0.16139$ \\
\bottomrule
\end{tabular}
\end{table}



\begin{figure}
\centering
\begin{align*}
\begin{pmatrix}
-0.2 & 0.2\\
0.2 & -0.2\\
\end{pmatrix}\\
\begin{pmatrix}
-0.64 & 0.64\\
0.63 & -0.63\\
\end{pmatrix}\\
& \begin{pmatrix}
0. & 0.155\\
0.885 & 0.\\
\end{pmatrix}
&\pm
\begin{pmatrix}
0. & 0.016\\
0.891 & 0.\\
\end{pmatrix}
\\ \end{align*}
\caption{1D synthetic SSDE, all experiment: Learned prior transition rates with mean and standard deviation. Order from top to bottom: True transition rates, Koehs result, all of our results, including one model that does not find the dynamics. }
\end{figure}
\subsection{Switching Ion Channel Data}



\begin{table}
\centering
\caption{Ion Channel, selected experiment: NLL and KL on various test sets.}
\begin{tabular}{rcc}
\toprule
                                Experiment &                      KL &                          NLL \\
\midrule
      Koehs Result, Prediction after Train &           - &                - \\
         Koehs Result, Prediction on Train &           - &                - \\
\midrule
   Train on $1$st sec, Prediction on Train &   $3.91659 \pm 4.83258$ &   $-2706.45040 \pm 27.78618$ \\
Train on $1$st sec, Prediction after Train &      $19.48157  $ &        $-2709.69348  $ \\
                     Train on $1$st second &   $4.75509 \pm 4.09270$ & $-1805.56500 \pm 1806.28715$ \\
                     Train on $2$nd second & $12.07092 \pm 36.10958$ &  $-2605.37450 \pm 118.08720$ \\
                     Train on full dataset &   $7.27852 \pm 3.03052$ &   $-2693.05612 \pm 35.21390$ \\
\bottomrule
\end{tabular}
\end{table}



\begin{table}
\centering
\caption{Ion Channel, selected experiment: RMSE on test set and at observations in various prediction sets.}
\begin{tabular}{rccccccccc}
\toprule
                                Experiment &               RMSE Test & \multicolumn{8}{c}{RMSE Prediction} \\
                                           &                 &                       1 &                       2 &                       3 &                       4 &                       5 &                      10 &                      50 &                      90 \\
\midrule
      Koehs Result, Prediction after Train &           - &           - &           - &           - &           - &           - &           - &           - &           - \\
         Koehs Result, Prediction on Train &           - &           - &           - &           - &           - &           - &           - &           - &           - \\
\midrule
   Train on $1$st sec, Prediction on Train & $\num{4.08e-13} \pm \num{1.94e-13}$ & $\num{2.37e-13} \pm \num{0.00e+00}$ & $\num{1.91e-13} \pm \num{0.00e+00}$ & $\num{1.67e-13} \pm \num{0.00e+00}$ & $\num{2.09e-13} \pm \num{0.00e+00}$ & $\num{2.23e-13} \pm \num{0.00e+00}$ & $\num{2.04e-13} \pm \num{0.00e+00}$ & $\num{8.51e-13} \pm \num{0.00e+00}$ & $\num{1.59e-12} \pm \num{3.05e-13}$ \\
Train on $1$st sec, Prediction after Train &      $\num{5.06e-13}  $ & $\num{2.94e-13} \pm \num{0.00e+00}$ & $\num{5.98e-14} \pm \num{0.00e+00}$ & $\num{3.72e-13} \pm \num{0.00e+00}$ & $\num{4.54e-13} \pm \num{0.00e+00}$ & $\num{2.22e-13} \pm \num{0.00e+00}$ & $\num{2.60e-13} \pm \num{0.00e+00}$ & $\num{6.68e-12} \pm \num{0.00e+00}$ & $\num{4.82e-12} \pm \num{2.67e-12}$ \\
                     Train on $1$st second & $\num{1.20e-12} \pm \num{1.07e-12}$ & $\num{1.07e-12} \pm \num{0.00e+00}$ & $\num{1.05e-12} \pm \num{0.00e+00}$ & $\num{1.09e-12} \pm \num{0.00e+00}$ & $\num{1.16e-12} \pm \num{0.00e+00}$ & $\num{1.25e-12} \pm \num{0.00e+00}$ & $\num{1.39e-12} \pm \num{0.00e+00}$ & $\num{1.61e-12} \pm \num{3.52e-14}$ & $\num{8.25e-13} \pm \num{1.96e-13}$ \\
                     Train on $2$nd second & $\num{1.34e-12} \pm \num{1.31e-12}$ & $\num{1.20e-12} \pm \num{0.00e+00}$ & $\num{1.17e-12} \pm \num{0.00e+00}$ & $\num{1.17e-12} \pm \num{0.00e+00}$ & $\num{1.18e-12} \pm \num{0.00e+00}$ & $\num{1.18e-12} \pm \num{0.00e+00}$ & $\num{1.20e-12} \pm \num{0.00e+00}$ & $\num{1.37e-12} \pm \num{6.42e-13}$ & $\num{1.89e-12} \pm \num{8.41e-13}$ \\
                     Train on full dataset & $\num{4.42e-13} \pm \num{2.05e-13}$ & $\num{1.97e-13} \pm \num{0.00e+00}$ & $\num{2.14e-13} \pm \num{0.00e+00}$ & $\num{2.26e-13} \pm \num{0.00e+00}$ & $\num{3.44e-13} \pm \num{0.00e+00}$ & $\num{4.86e-13} \pm \num{0.00e+00}$ & $\num{7.77e-13} \pm \num{0.00e+00}$ & $\num{1.44e-12} \pm \num{5.93e-13}$ & $\num{5.65e-13} \pm \num{0.00e+00}$ \\
\bottomrule
\end{tabular}
\end{table}



\begin{table}
\centering
\caption{Ion Channel, selected experiment: Equilibrium distribution.}
\begin{tabular}{rccc}
\toprule
                                Experiment & \multicolumn{3}{c}{Equilibrium Distribution} \\
                                           &             Bottom State &          Middle State &             Top State \\
\midrule
      Koehs Result, Prediction after Train &        $0.17961  $ &     $0.14987  $ &     $0.67052  $ \\
         Koehs Result, Prediction on Train &        $0.17961  $ &     $0.14987  $ &     $0.67052  $ \\
\midrule
   Train on $1$st sec, Prediction on Train &    $0.18487 \pm 0.02819$ & $0.08702 \pm 0.01139$ & $0.72811 \pm 0.03569$ \\
Train on $1$st sec, Prediction after Train &     $0.18137 \pm 0.0424$ &  $0.0885 \pm 0.01223$ & $0.73013 \pm 0.04687$ \\
                     Train on $1$st second &    $0.17582 \pm 0.03241$ & $0.09535 \pm 0.01464$ & $0.72883 \pm 0.04015$ \\
                     Train on $2$nd second &    $0.65818 \pm 0.18368$ & $0.00564 \pm 0.00674$ & $0.33618 \pm 0.18304$ \\
                     Train on full dataset &     $0.1963 \pm 0.01735$ & $0.07153 \pm 0.00592$ & $0.73217 \pm 0.02039$ \\
\bottomrule
\end{tabular}
\end{table}



\begin{figure}
\centering
\begin{align*}
& \begin{pmatrix}
-30.16 & 18.58 & 11.58\\
23.35 & -67.68 & 44.33\\
2.86 & 10.15 & -13.01\\
\end{pmatrix}
&\pm
\begin{pmatrix}
nan\\
\end{pmatrix}\\
& \begin{pmatrix}
0. & 56.150 & 2.648\\
118.839 & 0. & 216.052\\
0.656 & 25.704 & 0.\\
\end{pmatrix}
&\pm
\begin{pmatrix}
0. & 6.878 & 0.953\\
12.62 & 0. & 22.745\\
0.291 & 3.249 & 0.\\
\end{pmatrix}\\
& \begin{pmatrix}
0. & 16.172 & 22.991\\
5767.15 & 0. & 414.751\\
21.327 & 32.555 & 0.\\
\end{pmatrix}
&\pm
\begin{pmatrix}
0. & 13.586 & 18.826\\
5055.155 & 0. & 350.098\\
17.844 & 30.800 & 0.\\
\end{pmatrix}\\
& \begin{pmatrix}
0. & 130.131 & 2.495\\
356.236 & 0. & 575.229\\
0.78 & 55.725 & 0.\\
\end{pmatrix}
&\pm
\begin{pmatrix}
0. & 8.911 & 0.833\\
29.704 & 0. & 53.231\\
0.237 & 2.296 & 0.\\
\end{pmatrix}
\\ \end{align*}
\caption{Ion Channel, selected experiment: Learned prior transition rates with internal standard deviation. Order from top to bottom: Koehs result, our result trained on 1st second, our result trained on 2nd second and our result trained on full dataset.}
\end{figure}



\begin{table}
\centering
\caption{Ion Channel, selected experiment: Absolute Values of Eigenvalues of Q-Matrix.}
\begin{tabular}{rccc}
\toprule
                                Experiment & \multicolumn{3}{c}{Absolute Eigenvalues} \\
                                           &          $\lambda_0$ &         $\lambda_1$ &             $\lambda_2$ \\
\midrule
      Koehs Result, Prediction after Train &        - &      - &          - \\
         Koehs Result, Prediction on Train &        - &      - &          - \\
\midrule
   Train on $1$st sec, Prediction on Train &        $0.0 \pm 0.0$ &  $47.901 \pm 4.726$ &    $372.148 \pm 30.072$ \\
Train on $1$st sec, Prediction after Train &        $0.0 \pm 0.0$ &  $52.268 \pm 6.244$ &    $379.336 \pm 41.223$ \\
                     Train on $1$st second &        $0.0 \pm 0.0$ &  $47.831 \pm 4.125$ &    $341.809 \pm 36.563$ \\
                     Train on $2$nd second &        $0.0 \pm 0.0$ &  $75.28 \pm 37.063$ & $6199.663 \pm 5089.133$ \\
                     Train on full dataset &        $0.0 \pm 0.0$ & $103.458 \pm 5.828$ &   $1017.138 \pm 75.209$ \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}
\centering
\caption{Ion Channel, selected experiment: Relaxation Times.}
\begin{tabular}{rcc}
\toprule
                                Experiment & \multicolumn{2}{c}{Ordered Relaxation Times} \\
                                           \\
\midrule
      Koehs Result, Prediction after Train &            - &    - \\
         Koehs Result, Prediction on Train &            - &    - \\
\midrule
   Train on $1$st sec, Prediction on Train &          $0.003 \pm 0.0$ & $0.021 \pm 0.002$ \\
Train on $1$st sec, Prediction after Train &          $0.003 \pm 0.0$ & $0.019 \pm 0.002$ \\
                     Train on $1$st second &          $0.003 \pm 0.0$ & $0.021 \pm 0.002$ \\
                     Train on $2$nd second &            $0.0 \pm 0.0$ & $0.016 \pm 0.007$ \\
                     Train on full dataset &          $0.001 \pm 0.0$ &  $0.01 \pm 0.001$ \\
\bottomrule
\end{tabular}
\end{table}



\begin{figure}
\centering
\begin{align*}
& \begin{pmatrix}
0. & 0.019 & 0.031\\
0.084 & 0. & 0.014\\
0.119 & 0.038 & 0.\\
\end{pmatrix}
&\pm
\begin{pmatrix}
0. & 0.002 & 0.003\\
0.017 & 0. & 0.002\\
0.02 & 0.005 & 0.\\
\end{pmatrix}\\
& \begin{pmatrix}
0. & 0.008 & 0.014\\
0.031 & 0. & 0.006\\
0.048 & 0.018 & 0.\\
\end{pmatrix}
&\pm
\begin{pmatrix}
0. & 0.001 & 0.001\\
0.003 & 0. & 0.001\\
0.003 & 0.001 & 0.\\
\end{pmatrix}
\\ \end{align*}
\caption{Ion Channel, selected experiments trained on first second and on complete dataset: Mean passage time in seconds from state in row to state in column. States are ordered from lowest to highest state.}
\end{figure}



\begin{table}
\centering
\caption{Ion Channel, all experiment: NLL and KL on various test sets with mean and standard deviation.}
\begin{tabular}{rcc}
\toprule
                                Experiment &                     KL &                          NLL \\
\midrule
      Koehs Result, Prediction after Train &                      - &                            - \\
         Koehs Result, Prediction on Train &                      - &                            - \\
\midrule
Train on $1$st sec, Prediction after Train & $18.92818 \pm 0.68893$ &  $-2,694.21624 \pm 24.62892$ \\
   Train on $1$st sec, Prediction on Train &  $3.94384 \pm 0.25928$ &   $-2,703.86109 \pm 2.67986$ \\
                     Train on $1$st second &  $4.54390 \pm 0.33989$ & $-1,911.71990 \pm 269.29530$ \\
                     Train on $2$nd second & $10.42494 \pm 9.35271$ &  $-2,558.32012 \pm 36.07170$ \\
                     Train on full dataset &  $7.10734 \pm 0.34540$ &   $-2,688.25501 \pm 4.04080$ \\
\bottomrule
\end{tabular}
\end{table}



\begin{table}
\centering
\caption{Ion Channel, all experiment: RMSE on test set and at observations in various prediction sets.}
\begin{tabular}{rccccccccc}
\toprule
                                Experiment &               RMSE test & \multicolumn{8}{c}{RMSE prediction} \\
                                           &                 &                       1 &                       2 &                       3 &                       4 &                       5 &                      10 &                      50 &                      90 \\
\midrule
      Koehs Result, Prediction after Train &           - &           - &           - &           - &           - &           - &           - &           - &           - \\
         Koehs Result, Prediction on Train &           - &           - &           - &           - &           - &           - &           - &           - &           - \\
\midrule
Train on $1$st sec, Prediction after Train & $\num{6.63e-13} \pm \num{1.27e-13}$ & $\num{2.91e-13} \pm \num{8.96e-15}$ & $\num{6.30e-14} \pm \num{8.96e-15}$ & $\num{3.75e-13} \pm \num{8.96e-15}$ & $\num{4.57e-13} \pm \num{8.96e-15}$ & $\num{2.25e-13} \pm \num{8.96e-15}$ & $\num{2.63e-13} \pm \num{8.96e-15}$ & $\num{6.69e-12} \pm \num{8.96e-15}$ & $\num{5.50e-12} \pm \num{5.33e-13}$ \\
   Train on $1$st sec, Prediction on Train & $\num{4.18e-13} \pm \num{1.47e-14}$ & $\num{2.71e-13} \pm \num{7.27e-14}$ & $\num{2.24e-13} \pm \num{7.27e-14}$ & $\num{1.97e-13} \pm \num{7.32e-14}$ & $\num{2.32e-13} \pm \num{6.50e-14}$ & $\num{2.45e-13} \pm \num{6.34e-14}$ & $\num{2.38e-13} \pm \num{5.92e-14}$ & $\num{7.97e-13} \pm \num{1.12e-13}$ & $\num{1.64e-12} \pm \num{9.84e-14}$ \\
                     Train on $1$st second & $\num{1.13e-12} \pm \num{4.41e-14}$ & $\num{1.09e-12} \pm \num{1.05e-13}$ & $\num{1.09e-12} \pm \num{1.02e-13}$ & $\num{1.14e-12} \pm \num{1.02e-13}$ & $\num{1.20e-12} \pm \num{1.02e-13}$ & $\num{1.27e-12} \pm \num{1.06e-13}$ & $\num{1.40e-12} \pm \num{1.28e-13}$ & $\num{1.51e-12} \pm \num{1.32e-13}$ & $\num{8.33e-13} \pm \num{4.18e-14}$ \\
                     Train on $2$nd second & $\num{1.15e-12} \pm \num{3.20e-13}$ & $\num{1.27e-12} \pm \num{1.92e-13}$ & $\num{1.31e-12} \pm \num{2.60e-13}$ & $\num{1.36e-12} \pm \num{3.37e-13}$ & $\num{1.41e-12} \pm \num{3.94e-13}$ & $\num{1.44e-12} \pm \num{4.47e-13}$ & $\num{1.46e-12} \pm \num{5.02e-13}$ & $\num{1.53e-12} \pm \num{4.84e-13}$ & $\num{1.79e-12} \pm \num{2.34e-13}$ \\
                     Train on full dataset & $\num{4.42e-13} \pm \num{3.32e-14}$ & $\num{2.07e-13} \pm \num{6.43e-15}$ & $\num{2.17e-13} \pm \num{3.64e-15}$ & $\num{2.29e-13} \pm \num{3.64e-15}$ & $\num{3.43e-13} \pm \num{1.06e-15}$ & $\num{4.87e-13} \pm \num{5.14e-15}$ & $\num{7.78e-13} \pm \num{1.73e-15}$ & $\num{1.31e-12} \pm \num{1.80e-13}$ & $\num{5.78e-13} \pm \num{1.46e-14}$ \\
\bottomrule
\end{tabular}
\end{table}



\begin{table}
\centering
\caption{Ion Channel, all experiments: Equilibrium distribution with mean and standard deviation.}
\begin{tabular}{rccc}
\toprule
                                Experiment & \multicolumn{3}{c}{Equilibrium Distribution} \\
                                           &             Bottom State &          Middle State &             Top State \\
\midrule
      Koehs Result, Prediction after Train &                $0.17961$ &             $0.14987$ &             $0.67052$ \\
         Koehs Result, Prediction on Train &                $0.17961$ &             $0.14987$ &             $0.67052$ \\
\midrule
   Train on $1$st sec, Prediction on Train &    $0.18153 \pm 0.00542$ &  $0.0895 \pm 0.00513$ & $0.72897 \pm 0.00166$ \\
Train on $1$st sec, Prediction after Train &    $0.18142 \pm 0.00497$ & $0.08966 \pm 0.00542$ & $0.72892 \pm 0.00167$ \\
                     Train on $1$st second &    $0.18173 \pm 0.00506$ & $0.08944 \pm 0.00549$ & $0.72883 \pm 0.00137$ \\
                                2nd_second &    $0.33133 \pm 0.26885$ & $0.10641 \pm 0.07112$ & $0.56226 \pm 0.22591$ \\
                     Train on full dataset &    $0.19251 \pm 0.00456$ & $0.08055 \pm 0.00861$ & $0.72694 \pm 0.00654$ \\
\bottomrule
\end{tabular}
\end{table}
\begin{figure}
\centering
\begin{align*}
\begin{pmatrix}
-30.16 & 18.58 & 11.58\\
23.35 & -67.68 & 44.33\\
2.86 & 10.15 & -13.01\\
\end{pmatrix}\\
& \begin{pmatrix}
0. & 57.235 & 3.501\\
116.908 & 0. & 212.786\\
0.721 & 25.986 & 0.\\
\end{pmatrix}
&\pm
\begin{pmatrix}
0. & 1.777 & 0.496\\
5.020 & 0. & 5.378\\
0.082 & 0.514 & 0.\\
\end{pmatrix}\\
& \begin{pmatrix}
0. & 91.619 & 86.396\\
1297.79 & 0. & 186.562\\
13.407 & 40.487 & 0.\\
\end{pmatrix}
&\pm
\begin{pmatrix}
0. & 17.085 & 68.074\\
1997.861 & 0. & 121.040\\
8.690 & 12.69 & 0.\\
\end{pmatrix}\\
& \begin{pmatrix}
0. & 125.686 & 2.647\\
303.854 & 0. & 520.106\\
0.787 & 56.761 & 0.\\
\end{pmatrix}
&\pm
\begin{pmatrix}
0. & 0.625 & 0.099\\
2.734 & 0. & 3.803\\
0.067 & 0.392 & 0.\\
\end{pmatrix}
\\ \end{align*}
\caption{Ion Channel, all experiment: Learned prior transition rates with mean and standard deviation. Order from top to bottom: Koehs result, our result trained on 1st second, our result trained on 2nd second and our result trained on full dataset.}
\end{figure}



\begin{table}
\centering
\caption{Ion Channel, all experiments: Absolute Values of Eigenvalues of Q-Matrix.}
\begin{tabular}{rccc}
\toprule
                                Experiment & \multicolumn{3}{c}{Absolute Eigenvalues} \\
                                           &          $\lambda_0$ &          $\lambda_1$ &            $\lambda_2$ \\
\midrule
      Koehs Result, Prediction after Train &                - &       - &         - \\
         Koehs Result, Prediction on Train &                - &       - &         - \\
\midrule
   Train on $1$st sec, Prediction on Train &        $0.0 \pm 0.0$ &    $49.515 \pm 1.84$ &   $367.622 \pm 23.816$ \\
Train on $1$st sec, Prediction after Train &        $0.0 \pm 0.0$ &   $49.552 \pm 1.704$ &     $367.33 \pm 23.37$ \\
                     Train on $1$st second &        $0.0 \pm 0.0$ &   $49.431 \pm 1.612$ &   $367.464 \pm 23.274$ \\
                                2nd_second &        $0.0 \pm 0.0$ & $130.475 \pm 53.688$ & $1586.11 \pm 2307.065$ \\
                     Train on full dataset &        $0.0 \pm 0.0$ &    $102.3 \pm 2.111$ &    $907.541 \pm 80.05$ \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}
\centering
\caption{Ion Channel, all experiments: Relaxation Times.}
\begin{tabular}{rccc}
\toprule
                                Experiment & \multicolumn{2}{c}{Ordered Relaxation Times} \\
                                           \\
\midrule
      Koehs Result, Prediction after Train &                    - &   - \\
         Koehs Result, Prediction on Train &                    - &   - \\
   Train on $1$st sec, Prediction on Train &          $0.003 \pm 0.0$ & $0.02 \pm 0.001$ \\
Train on $1$st sec, Prediction after Train &          $0.003 \pm 0.0$ & $0.02 \pm 0.001$ \\
                     Train on $1$st second &          $0.003 \pm 0.0$ & $0.02 \pm 0.001$ \\
                                2nd_second &        $0.002 \pm 0.001$ & $0.01 \pm 0.004$ \\
                     Train on full dataset &          $0.001 \pm 0.0$ &   $0.01 \pm 0.0$ \\
\bottomrule
\end{tabular}
\end{table}




\begin{figure}
\centering
\begin{align*}
& \begin{pmatrix}
0. & 0.019 & 0.03\\
0.077 & 0. & 0.014\\
0.113 & 0.039 & 0.\\
\end{pmatrix}
&\pm
\begin{pmatrix}
0. & 0.001 & 0.001\\
0.005 & 0. & 0.000\\
0.005 & 0.001 & 0.\\
\end{pmatrix}\\
& \begin{pmatrix}
0. & 0.008 & 0.014\\
0.033 & 0. & 0.006\\
0.05 & 0.018 & 0.\\
\end{pmatrix}
&\pm
\begin{pmatrix}
0. & 0.000 & 0.000\\
0.001 & 0. & 0.000\\
0.001 & 0.001 & 0.\\
\end{pmatrix}
\\ \end{align*}
\caption{Ion Channel, all experiments trained on first second and on complete dataset: Mean passage time in seconds from state in row to state in column. States are ordered from lowest to highest state.}
\end{figure}

